Deep Learning Serves Traffic Safety Analysis: A Forward-looking Review

This paper explores Deep Learning (DL) methods that are used or have the potential to be used for traffic video analysis, emphasizing driving safety for both Autonomous Vehicles (AVs) and human-operated vehicles. We present a typical processing pipeline, which can be used to understand and interpret traffic videos by extracting operational safety metrics and providing general hints and guidelines to improve traffic safety. This processing framework includes several steps, including video enhancement, video stabilization, semantic and incident segmentation, object detection and classification, trajectory extraction, speed estimation, event analysis, modeling and anomaly detection. Our main goal is to guide traffic analysts to develop their own custom-built processing frameworks by selecting the best choices for each step and offering new designs for the lacking modules by providing a comparative analysis of the most successful conventional and DL-based algorithms proposed for each step. We also review existing open-source tools and public datasets that can help train DL models. To be more specific, we review exemplary traffic problems and mentioned requires steps for each problem. Besides, we investigate connections to the closely related research areas of drivers' cognition evaluation, Crowd-sourcing-based monitoring systems, Edge Computing in roadside infrastructures, Automated Driving Systems (ADS)-equipped vehicles, and highlight the missing gaps. Finally, we review commercial implementations of traffic monitoring systems, their future outlook, and open problems and remaining challenges for widespread use of such systems.

==> DL-long.tex <==
\section{The Fundamental Knowledge of Deep Learning}     \label{sec:dl}

\arr{we don't need this section. I think we had a miscommunication. Reviewing basics of DLL can turn against our focus and will bore the reader. MLP, CNN, .... are very basic stuff and useful for vbeginners and should come in tutorials not in review papers. What I wanted to add was adding at the end of each section, some overall trends, etc. For instance, what are new and next generation methods under development for vehicle classification, and what they add to the current practice, etc....}
\xc{\textit{Xiwen:} I thought the reviewer\#3 wanted more introduction about DL..}

\xc{The fundamental knowledge of deep learning is reviewed by many references (such as \cite{lecun2015deep,goodfellow2016deep}). A network can be considered as a mapping function parameterized by $\Theta$: $x\xrightarrow{f(x;\Theta)}\hat{y}$, where $x$ denotes the input and $\hat{y}$ denotes the predicted output. The loss function $\mathcal{L}(y,\hat{y})$ shows the distance between the prediction and the ground truth. The most basic approach to update the weight is gradient descent that updates a parameter $\Theta_i$ by $\Theta_i^{t+1}\leftarrow \Theta_i^{t}-\eta\frac{\partial\mathcal{L}}{\partial\Theta_i^{t}}$, where $\eta$ is the learning rate, and it is proved that the optimal of a function with strong convexity and strong smoothness can always reach with an as long as the learning rate is small enough. In deep learning, the dimensions of the network are often extremely high, and computing the high-order derivative is expensive and even infeasible, so first-order optimization is used more frequently. There are two branches of these first-order optimizers, which are schedule-based and adaptive-based. Schedule-based optimizers (such as Stochastic Gradient Descent (SGD) \cite{robbins1951stochastic}, Stochastic Gradient Descent with Momentum (SGDM), and Nesterov accelerated gradient (NAG) \cite{nesterov1983method}) often define the schedule of the function of learning rate in advance. while adaptive-based optimizers (such as Adaptive Gradient (Adagrad) \cite{duchi2011adaptive}, Adadelta \cite{zeiler2012adadelta},  Root Mean Square Propagation (RMSProp) \cite{tieleman2012lecture}, and Adam \cite{kingma2014adam} ) update the learning rate based on current gradient or the learned weights. To the best knowledge of authors, Adam is the most popular optimizer used in recent works.
There are three typical types of architectures:
\begin{itemize}
\item \textbf{Multilayer Perceptron (MLP)}: It is also known as Full Connected Networks consisting of multiple layers with multiple neurons. Each neurons is a linear function cascaded with a non-linear activation function (it avoids to learn a linear combination) and can be presented as $h_i=\sigma (\mathrm{w}^T x +b)$. $\sigma$ denotes the activation function, such as sigmoid and rectified linear units (Relu) \cite{agarap2018deep}. The units between two layers and dense connection, meaning that each unit from the previous layer connects to every unit in the current layers, which requires a large number of parameters. MLP is rarely used to solve complex problems; however, a paper \cite{tolstikhin2021mlp} proposed by Google in 2021 claimed that only using MLP with some modification can also achieve the results of the state-of-art. It is observed that their architecture still does not essentially solve the parameter problem, and we noted this work used TPU clusters and pre-trained on JKF-300M (300 million images with 18 classes), which is generally unavailable and infeasible for common research groups and some practical applications. MLP often has no specific assumption or prior before solving a problem. CNNs and RNNs use heuristic knowledge from their domain as the inductive bias (locality and Sequentiality, respectively) to enforce the ability of the networks.
     \item \textbf{Convolutional Neural Networks (CNN)}:  A CNN often contains many convolutional layers, activation functions, and pooling layers. Inspired by the locality of image signals, the convolution operation offers some important properties to reduce the complexity of classical neural networks and learn features more efficiently: i) sparse interaction, ii) parameter sharing, and iii) equivariant representation \cite{goodfellow2016deep}. In a convolutional layer, there are many small kernels that can be considered a filter bank. Each kernel can learn a certain feature (such as a line or edge) by mapping a patch of the feature maps from previous layers to a unit of the feature maps in the current layer (by summing the weighted units by the kernel then through an activation function). The area of the patch is known as the receptive field. Although the connection between two layers is sparse, these units can connect each other after some deeper layers. This is known as sparse interaction. In MLP, each $\mathrm{w}$ is only used once in once forward propagation, while in CNN, the weights are tied, meaning that the weight of the kernel will apply in all input (i.e., A kernel will slide all area of its input signal). This is known as parameter sharing. Another important property is shift-invariant, meaning that if we shift the input signal with a small value, the output signal will have the same shift. This property allows CNNs to detect a certain pattern regardless of the location of an image. Besides, pooling layers (such as max pooling) are used to downsample the feature maps that can preserve most information of the feature maps (only change the feature maps, not the number of channels. $1\times 1$ is often used to change the number of channels). It should note that CNN cannot directly handle some inherent properties of images, such as rotation invariant and scaling invariant, which require further processing.
     \item \textbf{Recurrent Neural Networks (RNN)}: The feed-forward networks (MLP and CNN) only consider the input at current step. Compared with them, RNNs have the advantage of handling sequential data (such as speech and audio) by maintaining both current input and the historical information as a hidden state. Thus, a typical RNN can be presented as $h^t = f(h^{t-1},x^t;\Theta)$. $h^t$ denotes the hidden layer at time $t$. Its back-propagation is known as Back-propagation Through Time (BPTT), which requires unfolding the network to every timestep and then computing its corresponding gradient with respect to the weights. Unfortunately, in practice, the vanilla RNN is hard to train by BPTT, and often gradient explosion or vanishing occurs. Moreover, since these gradient issues, RNN generally loses the long-term dependencies. Further, Long Short-term Memory (LSTM) was proposed in \cite{hochreiter1997long} that can address gradient vanishing and long-term dependencies by introducing the forgetting mechanism. An LSTM unit consists of a cell, an input gate, an output gate, and a forget gate, which collaboratively allow the network to get the memory of the dependencies with arbitrary time intervals (actually, it is still powerless if the intervals are two large). More recently, the Gated Recurrent Unit was proposed in \cite{cho2014properties}, and can be treated as a simpler version of LSTM. It can achieve a better performance than LSTM in some small datasets with fewer parameters \cite{chung2014empirical}.
 \end{itemize}}
 
\xc{ We provide a comparison among these architectures in Table \ref{tab:compare_dl}. Specially, we also provide a fresh architecture called Transformer, which has strong ability in both CV and sequence tasks. We give more detail about it in \ref{sec:transformer}. Notice that this comparison is not strict, and in piratical, people often combine multiple types of these architectures with many customized modules.}
 
 % Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\centering
\caption{A comparison among the typical architectures.}
\label{tab:compare_dl}
\resizebox{\textwidth}{!}{%
\blt
\begin{tabular}{lllll} \toprule
\textbf{Architecture} & \textbf{MLP} & \textbf{CNN} & \textbf{RNN/LSTM} & \textbf{Transformer} \\ \midrule
Pros & Straightforward to design & \begin{tabular}[c]{@{}l@{}}Good to process high-dimensional   data\\      Learn features with locality;\\      Shift-invariant;\\      Few parameters;\\      Powerful on CV tasks\end{tabular} & \begin{tabular}[c]{@{}l@{}}Good to process the sequential data;\\      LSTM can learn long-term dependencies\end{tabular} & \begin{tabular}[c]{@{}l@{}}Allow to process sequence parallelly;\\      Good to process long sequence;\\      Self-attention mechanism;\\      Powerful on both CV and NLP tasks\end{tabular} \\  \midrule
Cons & \begin{tabular}[c]{@{}l@{}}Paramters are too many since   dense connection;\\      Limited ability\end{tabular} & \begin{tabular}[c]{@{}l@{}}Do not encode the position of   object;\\      Gradient vanishing in very deep layers \\      (solved by ResNet \cite{});\\      Not good to process long sequence data\end{tabular} & \begin{tabular}[c]{@{}l@{}}Hard to train since gradient issues;\\      The data only can be input serially; \\      powerless to extreme long-term dependencies\end{tabular} & \begin{tabular}[c]{@{}l@{}}Many parameters that require long   time to train; \\      Not consider locality; \\ Has not many advantages in short sequence\end{tabular} \\ \midrule
Inductive Bias & Weak & Locality/Spatial invariance & Sequentiality/Time invariance & Weak \\
\bottomrule
\end{tabular}%
}
\end{table*}
 
 
  \xc{Training a network sometimes is not straightforward and is impacted by many factors. For example, the training schedule should be well initialized with some hyper-parameters (such as mini-batch size and learning rate). A network is encouraged to be large at the beginning, then pruning its architecture. Moreover, some tricks can be helpful in boosting the performance of the networks. For example, word embedding uses low-dimensional space to present high-dimensional data, which allows words with similar meanings to be closer in the low-dimensional space. This often much outperforms one-hot encoding. An exemplary scenario would be personalized driving abnormal detection. Suppose there are 20 collected features for each driver. If there are 100 drivers, by one-hot encoding, the input dimensions of data should be $100+20=120$, which leads to the "curse of dimensionality ."This because, in fact, the difference among these drivers are definitely deserved to use 20 dimensions to represent, and maybe 10 dimensions are enough. We list some common tricks in Table \ref{tab:DL_tricks}. We do not claim these tricks can definitely lead to improvement since training a network sometimes is empirical.}
 
 % Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Some tricks that may help to train a network.}
\label{tab:DL_tricks}
\resizebox{\columnwidth}{!}{%
\blt
\begin{tabular}{ll}\toprule
\textbf{Name} & \textbf{Description} \\ \midrule
Data Normalization & Stabilize the training \\ \midrule
Xavier/Kaiming Inti. & Initialize based on the magnitudes    of signals \\ \midrule
\begin{tabular}[c]{@{}l@{}}Batch/Layer/Instance \\ Normalization\end{tabular} & \begin{tabular}[c]{@{}l@{}}Local response   normalization;\\      As a regularizer;\\      Avoid gradient vanishing\end{tabular} \\ \midrule
Dropout & A regularizer to  avoid overfitting \\ \midrule
L1/L2 regularization & Regularizers to  avoid overfitting \\ \midrule
Weight decay & \begin{tabular}[c]{@{}l@{}}Similar to L2   regularization\\      but different in some optmizers (e.g. Adam)\end{tabular} \\ \midrule
LeakyRelu & Avoid dead neurons (as for Relu) \\ \midrule
Word Embedding & Better manage high-space categorical data \\ \midrule
Soft Labeling & \begin{tabular}[c]{@{}l@{}}State the relations between   different classes;\\      Improve generalization\end{tabular} \\ \midrule
Data Augmentation & \begin{tabular}[c]{@{}l@{}}Improve the variety of   data;\\      Improve generalization\end{tabular} \\ \midrule
Residual Connection & \begin{tabular}[c]{@{}l@{}}Avoid gradient vanishing;\\      Allow to build a very deep networks\end{tabular} \\ \midrule
$1\times 1$ Conv & Change the number of channels \\ \midrule
Gradient Clipping & Avoid gradient explosion \\ \bottomrule
\end{tabular}%
}
\end{table}
 
 
 
     
     %Moreover, a pattern of an image is expected to be invariant to location \cite{lecun2015deep}.  
     
     
    %  can considered as a filters bank.  
     
     
     
    %  are inspired by the fact that 2D signal (such as images) has local connection, which means the features can be represented by much fewer parameters. 
     
     
    %  which can be represented by fe
     
    %  A CNN often contains many convolutional layers, activation function, and pooling layer.
    
    


% \subsection{Multilayer Perceptron (MLP) }
% Multilayer Perceptron also known Full Connected Networks consists of multiple layers with multiple neurons. Each neurons is a linear function cascaded with a non-linear activation function (it avoids to learn a linear combination). 


%\subsection{Convolutional Neural Networks (CNN)}


% \subsection{Recurrent Neural Networks (RNN)}

==> TableDataset-1.tex <==

\begin{table}[!h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
Category &
  Dataset &
  Size &
  Features \\ \hline
\multirow{\begin{tabular}[c]{@{}l@{}}Trajectory\\ analysis\end{tabular}} &
  MIT traffic dataset(2011)\cite{wang2011automatic} &
  \begin{tabular}[c]{@{}l@{}}around 162, 000 frames\\ from a 90 minutes long video sequence (30 fps)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Both pedestrian and vehicle movements\\ with occlusions and varying illumination conditions\end{tabular} \\ \cline{2-4} 
 &
  MIT trajectory dataset(2008)\cite{grimson2008trajectory} &
  577 radar tracks, 45 453 video tracks &
  Multiple single camera view \\ \cline{2-4} 
 &
  CVRR trajectory analysis datasets (2011) \cite{morris2011trajectory}  &
  \begin{tabular}[c]{@{}l@{}}4 scenes: a simulated intersection (19 activities),\\ a real highway (8 activities)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Units are pixels;\\ \\ only contain spatial information;\end{tabular} \\ \cline{2-4} 
 &
  i-Lids–advanced vehicle detection challenge\cite{ilidsadvanced_2007} &
  35000 images. 7 sequences with 25 fps. &
  \begin{tabular}[c]{@{}l@{}}Consider daytime;\\ various locations in the UK\end{tabular} \\ \cline{2-4} 
 &
  QMUL junction dataset(2012) \cite{hospedales2012video} &
  1 hour video &
  busy traffic at a junction \\ \hline
\multirow{\begin{tabular}[c]{@{}l@{}}Auto-driving\\ tasks\end{tabular}} &
  CamVid(2009) \cite{brostow2009semantic} &
  700 images, 32 classes, 10 min HD video with 30fps &
  \begin{tabular}[c]{@{}l@{}}support pixel-wise segmentation tasks;\\ provide 3D camera pose.\end{tabular} \\ \cline{2-4} 
 &
  Cityscapes (2016)\cite{cordts2016cityscapes} &
  \begin{tabular}[c]{@{}l@{}}5000 pixel-level annotated images\\  and 20000 coarse annotated images (weak-label)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}complex urban street scenes;\\  record from 50 cities;\end{tabular} \\ \cline{2-4} 
 &
  Mapillary Vistas Dataset(2017)\cite{neuhold2017mapillary} &
  \begin{tabular}[c]{@{}l@{}}25 000 high-resolution images; \\ 66 classes for objection\\ 37 instance-specific labels\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Various conditions regarding weather, \\ season and daytime\end{tabular} \\ \cline{2-4} 
 &
  SYNTHIA(2016) \cite{ros2016synthia} &
  \begin{tabular}[c]{@{}l@{}}13,400 frames of the city (real);\\ \\ four video sequences of  ~50,000 frames (simulated);\\ 13 classes\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Scene diversity;\\ multiple seasons;\\ lighting conditions and weather\end{tabular} \\ \cline{2-4} 
 &
  KITTI Vision Benchmark Suite (2012)\cite{Geiger2012CVPR}&
  7481 training images and 7518 test images; &
  \begin{tabular}[c]{@{}l@{}}Up to 15 cars and 30 pedestrians per image;\\ tasks of interest are stereo, optical flow, \\ visual odometry, 3D object detection, and 3D tracking.\end{tabular} \\ \cline{2-4} 
 &
  Berkeley Deep Drive (2018)\cite{yu2018bdd100k}  &
  over 100K videos &
  \begin{tabular}[c]{@{}l@{}}diversity of annotations ;\\ diversity of geography, environment, and weather.\end{tabular} \\ \cline{2-4} 
 &
  IDD (2019) \cite{varma2019idd}&
  10,004 images; 34 classes; 182 drive sequences &
  \begin{tabular}[c]{@{}l@{}}unstructured environments;\\ four-level label hierarchy; possibility for new tasks: \\ domain adaptation, \\ few-shot learning and behavior prediction.\end{tabular} \\ \hline
\multirow{\begin{tabular}[c]{@{}l@{}}Traffic sign\\ detection\end{tabular}} &
  TLR (2009)\cite{de2009real} &
  \begin{tabular}[c]{@{}l@{}}11 179 frames (8min 49sec, @25FPS);\\ 9 168 instances of traffic lights\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}hand-labeled;\\ tasks for traffic light detection and traffic sign detection\end{tabular} \\ \cline{2-4} 
 &
  LISA (2012)\cite{mogelmose2012vision}&
  \begin{tabular}[c]{@{}l@{}}6600 frames with ~7800 annotated objects;\\ 49 classes of signs\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Recorded in the US;\\ Images from various camera types\end{tabular} \\ \cline{2-4} 
 &
  GTSDB(2013)\cite{houben2013detection} &
  \begin{tabular}[c]{@{}l@{}}900 images \\ divided into 600 training images (846 traffic signs) \\ and 300 evaluation images (360 traffic signs)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}signs are divided into prohibitory, danger, mandatory, \\ and other signs\end{tabular} \\ \cline{2-4} 
 &
  BelgianTS(2014)\cite{timofte2014multi} &
  \begin{tabular}[c]{@{}l@{}}13,444 traffic sign annotations in 9,006 still images \\ corresponding to 4,565\\ physically distinct traffic signs.\end{tabular} &
  Available for 2D and 3D testing. \\ \cline{2-4} 
 &
  TT100K (2016)\cite{zhu2016traffic}&
  \begin{tabular}[c]{@{}l@{}}100000 images containing 30000 traffic-sign instances;\\  128 sign classes\end{tabular} &
  Diversity of annotation \\ \cline{2-4} 
 &
  BSTL (2017)\cite{behrendt2017deep}&
  \begin{tabular}[c]{@{}l@{}}13427 images (5093training+8334test~15fps);\\ 24000 annotated traffic lights\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Cover a decent variety of road scenes and\\  typical difficulties\end{tabular} \\ \hline
\multirow{\begin{tabular}[c]{@{}l@{}}Naturalistic\\ Study\end{tabular}} &
  The 100-Car Naturalistic Driving Study(2006)\cite{dingus2006100} &
  \begin{tabular}[c]{@{}l@{}}~2,000,000 vehicle miles;\\ ~43,000 hours of data\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Contains extreme cases of driving behavior;\\ Event-based database\end{tabular} \\ \cline{2-4} 
 &
  SHRP 2 NDS dataset(2012)\cite{the_shrp_2_2012}  &
  more than 2 PB of continuous naturalistic driving data &
  \begin{tabular}[c]{@{}l@{}}Multi-view video outputs;\\ collected during a 3-y period from \\ more than 3,500 participants, aged 16–98\end{tabular} \\ \hline
\multirow{Plate detection} &
  ReId (2017)\cite{ReId} &
  9.5hours from 8 locations &
  \begin{tabular}[c]{@{}l@{}}varied daytimes;\\ multi-plates on a frame\\ cameras placed on bridges above highways;\\ relatively small objects\end{tabular} \\ \cline{2-4} 
 &
  UCSD car dataset(2007) \cite{UCSDCARS} &
  \begin{tabular}[c]{@{}l@{}}10 hours video;\\ 878 cars tracked from the moment;\\ 291 still cars recorded in parking lot\end{tabular} &
  label with make, model, license plate location, plate texts \\ \cline{2-4} 
 &
  UFPR-ALPR Dataset(2018)\cite{laroca2018robust_UFPR} &
  \begin{tabular}[c]{@{}l@{}}4,500 fully annotated images from 150 vehicles;\\ 30 fps\\ >30,000 license characters;\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}different license color;\\ both vehicle and camera are moving\end{tabular} \\ \cline{2-4} 
 &
  SSIG Dataset(2016)\cite{gonccalves2016benchmark_SSIG} &
  \begin{tabular}[c]{@{}l@{}}2000 Brazilian license plates; \\ 14,000 alphanumeric symbols\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}static camera view;\\ character are segmented\end{tabular} \\ \hline
\multirow{UAV} &
  MOR-UAV(2020)\cite{MOR-UAV} &
  \begin{tabular}[c]{@{}l@{}}89,783 moving object instances;\\  10,948 various scenarios;\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}tasks for moving and non-moving objects;\\ varied conditions of the environment;\\ labeled by aixs-aligned bounding boxes\end{tabular} \\ \cline{2-4} 
 &
  Stanford Drone Dataset(2016)\cite{robicquet2016learning} &
  \begin{tabular}[c]{@{}l@{}}>100 top-view scenes;\\ 20,000 targets\\ annotated trajectories and id\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}real-world scenario-based;\\ varied types of targets\end{tabular} \\ \cline{2-4} 
 &
  The highD dataset(2018)\cite{krajewski2018highd} &
  \begin{tabular}[c]{@{}l@{}}16.5hous of measurements for 110,000 vehicles from 6\\ locations.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}real-world scenario-based;\\ focus on highways\\ contain naturalistic behavior of road users\end{tabular} \\ \cline{2-4} 
 &
  The inD dataset(2019)\cite{bock2019ind} &
  \begin{tabular}[c]{@{}l@{}}contains more than 11500 road users;\\ 10 hours measurement\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Succeessor of highD,\\ focus on intersections\end{tabular} \\ \hline
  \multirow{}{}{\begin{tabular}[c]{@{}l@{}}Video-based \\ Traffic events\\ (Accident)\end{tabular}} &
  UCF-Crimes(2018) \cite{sultani2018real} &
  1900 sequences, 128hours &
  \begin{tabular}[c]{@{}l@{}}Includes realistic anomalies such as fighting, road accident.\\ No spatial annotation\end{tabular} \\ \cline{2-4} 
 &
  DAD(2016) \cite{chan2016anticipating} &
  1730 sequences, 2.4 hours &
  \begin{tabular}[c]{@{}l@{}}Spatio-temporal annotation\\ Video captured by dashcam for driving behavior\end{tabular} \\ \cline{2-4} 
 &
  CADP(2018)\cite{shah2018cadp} &
  1416 sequences, 5.2 hours &
  \begin{tabular}[c]{@{}l@{}}Include multi-accident sequences\\ Captured by CCTVInclude varied environment\end{tabular} \\
  \cline{2-4}
  &
  NVIDIA AI CITY challenge\cite{ai_city_challenge} &
  \begin{tabular}[c]{@{}l@{}}Track 1: 31 videos (about 9 hours in total)\\ Track 2: 56,277 images,\\ 36,935 come from 333 object identities\\ Track 3: 215.03 minutes videos \\ 300K bounding boxes\\ Track 4: 200 15mins videos 30fps\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Track 1: vehicle counting\\ Track 2: vehicle Re-id\\ Track 3: vehicle tracking\\ Track 4: Abnormal detection\\ Anomalies can be due to \\ car crashes or stalled vehicles\end{tabular} \\ \hline
  

\end{tabular}%
}
\caption{Some popular traffic-related datasets}
\label{tab:trafficdataset}
\end{table}


==> backup.tex <==
\section{Deep Learning for video processing} \label{sec:video-proc}

Deep learning methods are heavily used for video processing for their outstanding power in solving different problems such as object detection, object recognition, event recognition, and other video understanding tasks in general. DL methods can be considered the brainpower of most AI platforms developed for traffic safety analysis.   

\subsection{DL-based Classification Methods in Traffic Analysis} 
%\xc{Xiwen: I think we can compress the classification section. since 1) There are very limited works using deep learning to do traffic-related classification problem (except fine-grained classification), 2) the detection methods must include classification function, and in order to compress the content, We can consider to compress this section and only focused on classification methods for fine-grained vehicle classification. }
%\arr{Good point: I agree with you, and it is better to keep the first para about the use of classification in traffic analysis. And change the text from para 2..., you can start saying that "Since the use of classification methods for most traffic-related problems is straightforward and noting the fact that there exist comprehensive reviews on classification methods, we skip the review of classification methods and refer the interested reader to [REFs]. Here, we only review fine-grained classification methods that are custom built or customized for traffic-related problems. Also, note that classification can be an integral part of some other methods, including instance segmentation, object detection, speed estimation, etc."   However, use "ifx myver..." command to keep the previous text. Finally, use blue color so I remember to review the new text.}

\ifx \myver \oldVer
Classification is one of the most fundamental tasks in computer vision. The use of classification in this context can be implemented for object classification (e.g., classifying objects between vehicles, pedestrians, motorcycles, traffic signs, etc.), traffic light and railroad crossing barrier status check, and scene detection (e.g., buildings, roads, road lanes, roadside infrastructures, etc.). It can be developed at different levels, such as the basic level for classifying different object types and fine-grained classification into sub-categories (such as differentiating traffic signs or identifying vehicle classes among sedans, SUVs, trucks, etc.) based on the semantic content of the input.


%Various network architectures are developed for these tasks that later been used as backbone networks for other tasks. This means classification can be regarded as a benchmark task for verifying the feasibility of new network architecture or a module developed to boost the performance of the existing network. Network architectures for different application scenarios are also a focal point, such as a lightweight network for mobile and embedded platforms. The first Deep Convolutional Neural Networks (CNNs) was LeNet~\cite{lecun1998gradient} that achieved a state-of-art performance on hand-written digits recognition. However, LeNet has a limited performance on large scale data. After ImageNet~\cite{russakovsky2015imagenet} became the new benchmark on image classification task, Deep CNN architectures targeting the large scale data learning were supposed to be developed. In 2012, AlexNet~\cite{krizhevsky2012imagenet} firstly brought the classification error rate from $26\%$ in $15\%$. After two year, VGGnet proposed a deeper network that further improve the classification accuracy. But when the network goes deeper, there raise another problem, that the simply stacking layers on plain architecture is obviously not a suitable solution to boost the performance. ResNet~\cite{he2016deep} was proposed for addressing the gradient propagation and degradation problem. ResNet enables people to train a much deeper network by applying residual connection on the CNNs. Another question existed in CNNs is that the convolutional layers typically have fixed receptive field. GoogLeNet~\cite{szegedy2015going} proposed a multi-scale feature fusion architecture that concatenated features extracted by conv layers with different filter size.  To let CNNs running on mobile and embedded systems, Depth-wise separation convolution (DWConv) was proposed in~\cite{chollet2017xception}. DWConv achieved similar performance as naive conv layer with much less computational and parameters. MobileNet~\cite{howard2017mobilenets} and ShuffleNet~\cite{zhang2018shufflenet} are two light-weight network architectures specific for mobile and embedded devices. Another problem in CNNs is that the Conv layer takes all feature channels equally. To let the CNNs focus on informative channels, attention mechanism was introduced in SENet~\cite{hu2018squeeze}. SENet set up channel attention modules to self-guide the networks to filter the less important features, that remarkably improved the performance of existed CNNs. The example of fine-grained vehicle model/make classifcation shown in Fig.\ref{fig:VehicleFineGrained} 


Due to the generality and flexibility of DL methods, most existing DL methods can be used for traffic safety analysis, like other applications. 
It is noteworthy that various DL network architectures are developed primarily for classification tasks and then further extended for other tasks. Therefore, standard classification problems can be used as a benchmark testing method to evaluate the performance of different network architectures. 
There are popular DL networks whose performance is further boosted by several architectural modifications. 
DL algorithms are nowadays available for different operating systems running on most computer architectures accelerated by GPUs/TPUs, Message Passing Interface (MPI)-based parallel programming, and high-performance computing (HPC). 
Other modifications are implemented to accommodate emerging processing platforms. For instance, lightweight networks are proposed for mobile, FPGA-based, and embedded computation platforms. 

The first Deep Convolutional Neural Networks (D-CNNs) was LeNet~\cite{lecun1998gradient} that achieved state-of-the-art performance on hand-written digit recognition. However, LeNet has a limited performance on large-scale data. 
In 2012, AlexNet~\cite{krizhevsky2012imagenet} realized a breakthrough by dramatically reducing the classification error rate from $26\%$ to $15\%$.
Another breakthrough was the implementation of ImageNet~\cite{russakovsky2015imagenet}, which soon became the new benchmark for image classification tasks. Afterward, a countless number of various deep CNN architectures were developed to tackle large-scale datasets. 
Another notable architecture was VGGnet\cite{simonyan2014very}, which utilized a deeper network architecture to further improve the classification accuracy. But when the network goes deeper, different problems such as computational complexity, error propagation in gradient-based back-propagation for network training, and the need for larger datasets arise by stacking many layers, and the performance of the network saturates with minimal improvement for additional layers.  ResNet~\cite{he2016deep} was proposed in 2016 to address such issues by enabling people to train a much deeper network by applying residual connections to the CNNs. 

Another issue with standard CNNs is the restrictive use of fixed receptive fields in convolutional layers. GoogLeNet~\cite{szegedy2015going} proposed a multi-scale feature fusion architecture that concatenates features extracted by convolution layers with different filter sizes. 
Another remarkable milestone was developing wider than deeper networks. For instance, Wide Residual Networks (WRN)~\cite{zagoruyko2016wide} is proposed to used wider bottlenecks to enhance the performance of ResNet. 

Another research direction is enabling CNNs to execute on mobile and embedded systems. For instance, Depth-Wise Separation Convolution (DWConv) was proposed in~\cite{chollet2017xception}, which achieved similar performance as naive convolution layers with much less computational complexity and fewer parameters. MobileNet~\cite{howard2017mobilenets} and ShuffleNet~\cite{zhang2018shufflenet} are two light-weight network architectures specific for mobile and embedded devices. 

An important issue with the CNNs is that the Convolution layers take all feature channels equally. To make the CNN focus on informative channels, an attention mechanism was introduced in SENet~\cite{hu2018squeeze}. SENet set up channel attention modules to self-guide the networks to filter the less important features that remarkably improved the performance of existed CNNs. Other recent works implement different channel attention mechanisms to improve the representational capacity of convolutional networks \cite{li2019meda}.
The example of fine-grained vehicle model/make classification using CNN-based methods is shown in Fig.\ref{fig:VehicleFineGrained}. 
% Various datasets have been proposed for different classification tasks, as shown in Table.\ref{tab:Classifaction Datasets}.





\begin{figure}[h]
\begin{center}
\centerline{\includegraphics[width=1\columnwidth]{figures/FineGrainedCars.jpg}}
\caption{The example of fine-grained vehicle make/model classification.}%Source from\cite{yang2015large}} 
\label{fig:VehicleFineGrained}
\end{center}
\end{figure}




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\else
%\xc{New version:}
Classification is one of the most fundamental tasks in computer vision. The use of classification in this context can be implemented for object classification  (e.g., classifying objects between vehicles, pedestrians, motorcycles, traffic signs, etc.), traffic light and railroad crossing barrier status check, and scene detection (e.g., buildings, roads, road lanes, roadside infrastructures, etc.). Often, it is the backbone or the feature extractor part of the detection networks (e.g., SSD\cite{liu2016ssd}) and segmentation networks (e.g., Mask R-CNN\cite{he2017mask}). It can be developed at different levels, such as the basic level for classifying different object types and fine-grained classification into sub-categories (such as differentiating traffic signs or identifying vehicle classes among sedans, SUVs, trucks, etc.) based on the semantic content of the input. The well-known baseline classification methods include AlexNet(2012) \cite{krizhevsky2012imagenet}, VggNet(2014) \cite{simonyan2014very}, GoogleNet(2015) \cite{szegedy2015going}, ResNet(2016) \cite{he2016deep}, MobileNets(2017) \cite{howard2017mobilenets}, DenseNet(2017)\cite{huang2017densely}, EfficientNet(2019), \cite{tan2019efficientnet} etc. 
\ar{It is noteworthy that ResNet is %[amongst] 
the most highly cited paper in all areas in Google Scholar Metrics 2020, which further proves its extraordinary achievement.} 

\ar{Classification is often considered an upstream task. Therefore, frameworks of the downstream tasks, such as detection, tracking, and segmentation, often use the pre-trained versions of these baselines DL architectures as their backbone to extract the hidden representations. Note that these baseline methods mainly utilized CNN architectures until recently, when a framework named \textit{Transformer} has offered a new breed of deep learning methods with even higher performances, as discussed in Section \ref{sec:transformer}.}


Since the use of classification methods for most traffic-related problems is straightforward and noting the fact that there exist comprehensive reviews on classification methods, we skip the review of classification methods and refer the interested reader to \cite{shen2019survey,schmarje2020survey,zhao2017survey,wang2019development}. Here, we only review fine-grained classification methods that are custom-built or customized for traffic-related problems, as presented in Table \ref{tab:fine-grained} and Fig.\ref{fig:VehicleFineGrained_perf}.



\fi

%Also, note that classification can be an integral part of some other methods, including instance segmentation (e.g.\cite{zhang2020traffic}), object detection (e.g. \cite{zhou2016dave,yu2017model,sang2018improved,nayak2019vision}), speed estimation, etc. 





\begin{comment}

\begin{table*}[h]
\centering
\caption{Examples of fine-grained vehicle classification.}
\label{tab:fine-grained}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline\rowcolor{gray}
\textbf{Method} &
  \textbf{Paper:[Ref] Authors (year)} &
  \textbf{Performance Accuracy [Dataset]} \\ \hline
3D box+CNN &
  \cite{sochor2016boxcars}Sochor et al.(2016) &
  83.20\% \\ \hline
3D box+Vgg-16 &
  \cite{sochor2018boxcars}Sochor et al.(2018) &
  92.27\% on  BoxCars116k(self) \\ \hline
DenseNet-161 &
  \cite{ma2019fine}Ma et al.(2020) &
  \begin{tabular}[c]{@{}l@{}}93.81 \% on Stanford Cars\cite{krause20133d}\\      97.89 \% on    COMPCARS\cite{yang2015large}\end{tabular} \\ \hline
DenseNet-161 &
  \cite{li2019dual}Li et al.(2019) &
  93.51\% on Stanford Cars\cite{krause20133d} \\ \hline
part-based +DenseNet-264 &
  \cite{xiang2019global}Xiang et al.(2019) &
  \begin{tabular}[c]{@{}l@{}}94.3\% on Stanford Cars\cite{krause20133d}\\      99.6\% on COMPCARS\cite{yang2015large}\end{tabular} \\ \hline
Part-based+RCNN+SVM &
  \cite{huang2016fine}Huang et al.(2016) &
  87.3\% \\ \hline
Faster R-CNN+Feature Fusion &
  \cite{zhu2019fine}Zhu et al.(2019) &
  Top 1: 79.1\%, Top 5: 94.1\% on COMPCARS\cite{yang2015large} \\ \hline
CNN+Feature Fusion &
  \cite{yu2018ff}Yu et al.(2018) &
  98.89\% on COMPCARS\cite{yang2015large} \\ \hline
ResNet-50 + Attention &
  \cite{yu2020cam}Yu et al.(2020) &
  \begin{tabular}[c]{@{}l@{}}93.1\% on Stanford Cars\cite{krause20133d}\\      95.3\% on COMPCARS\cite{yang2015large}\end{tabular} \\ \hline
Attention &
  \cite{ke2020fine}Ke et al.(2020) &
  \begin{tabular}[c]{@{}l@{}}94.5\% mAP on Stanford Cars\cite{krause20133d}\\      95.8\% FZU dataset (self)\end{tabular} \\ \hline
multi-task CNN &
  \cite{hu2017location}Hu et al.(2017) &
  Top 1: 91\%, Top 5: 97.7\% on COMPCARS\cite{yang2015large} \\ \hline
CNN+filter bank &
  \cite{wang2018learning}Wang et al.(2018) &
  93.8\% on Stanford Cars\cite{krause20133d} \\ \hline
Fine-tuning Vgg-16 &
  \cite{zhang2018fine}Zhang et al.(2018) &
  98.71\% on COMPCARS\cite{yang2015large} \\ \hline
\end{tabular}%
}
\end{table*}
\end{comment}




\begin{table*}[h]
\centering
\caption{Examples of fine-grained vehicle classification.}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{lll}
\toprule
\textbf{Method} &
  \textbf{Paper:[Ref] Authors (year)} &
  \textbf{Performance Accuracy [Dataset]} \\ \midrule
3D box+CNN &
  \cite{sochor2016boxcars}Sochor et al.(2016) &
  83.20\%  on  BoxCars116k(self)\\ \midrule
3D box+Vgg-16 &
  \cite{sochor2018boxcars}Sochor et al.(2018) &
  92.27\% on  BoxCars116k(self) \\ \midrule
DenseNet-161 &
  \cite{ma2019fine}Ma et al.(2020) &
  \begin{tabular}[c]{@{}l@{}}93.81 \% on Stanford Cars\cite{krause20133d}\\      97.89 \% on    COMPCARS\cite{yang2015large}\end{tabular} \\ \midrule
DenseNet-161 &
  \cite{li2019dual}Li et al.(2019) &
  93.51\% on Stanford Cars\cite{krause20133d} \\ \midrule
part-based +DenseNet-264 &
  \cite{xiang2019global}Xiang et al.(2019) &
  \begin{tabular}[c]{@{}l@{}}94.3\% on Stanford Cars\cite{krause20133d}\\      99.6\% on COMPCARS\cite{yang2015large}\end{tabular} \\ \midrule
Part-based+RCNN+SVM &
  \cite{huang2016fine}Huang et al.(2016) &
  87.3\% \\ \midrule
Faster R-CNN+Feature Fusion &
  \cite{zhu2019fine}Zhu et al.(2019) &
  Top 1: 79.1\%, Top 5: 94.1\% on COMPCARS\cite{yang2015large} \\ \midrule
CNN+Feature Fusion &
  \cite{yu2018ff}Yu et al.(2018) &
  98.89\% on COMPCARS\cite{yang2015large} \\ \midrule
ResNet-50 + Attention &
  \cite{yu2020cam}Yu et al.(2020) &
  \begin{tabular}[c]{@{}l@{}}93.1\% on Stanford Cars\cite{krause20133d}\\      95.3\% on COMPCARS\cite{yang2015large}\end{tabular} \\ \midrule
Attention &
  \cite{ke2020fine}Ke et al.(2020) &
  \begin{tabular}[c]{@{}l@{}}94.5\% mAP on Stanford Cars\cite{krause20133d}\\      95.8\% FZU dataset (self)\end{tabular} \\ \midrule
multi-task CNN &
  \cite{hu2017location}Hu et al.(2017) &
  Top 1: 91\%, Top 5: 97.7\% on COMPCARS\cite{yang2015large} \\ \midrule
CNN+filter bank &
  \cite{wang2018learning}Wang et al.(2018) &
  93.8\% on Stanford Cars\cite{krause20133d} \\ \midrule
Fine-tuning Vgg-16 &
  \cite{zhang2018fine}Zhang et al.(2018) &
  98.71\% on COMPCARS\cite{yang2015large} \\ \bottomrule
\end{tabular}%
}
\label{tab:fine-grained}
\end{table*}


\begin{figure}[h]
\begin{center}
\centerline{\includegraphics[width=1\columnwidth]{figures/fine_class.jpg}}
\caption{The performance of some fine-grained models on Stanford Cars and COMPCARS.}%Source from\cite{yang2015large}} 
\label{fig:VehicleFineGrained_perf}
\end{center}
\end{figure}





\begin{figure*}[h]
\begin{center}
\centerline{\includegraphics[width=1\textwidth]{figures/detectionfig_2.png}}
\caption{ (a),(b) are the examples of vehicle detection by two alternative methods YOLOv5\cite{glenn_jocher_2021_4679653} and Faster R-CNN\cite{ren2015faster}. They output the location and category of each object with detection confidence. Cars are shown by orange bounding boxes, trucks are shown by lime bounding boxes, buses are shown by green bounding boxes, and persons are shown by red bounding boxes. As shown in (a),(b), YOLOv5 performs worse on small vehicle detection while Faster R-CNN has missed objects in the near zone. (c) is the is PII removed data. %\xc{SSD performs bad at this image, so I removed it.} 
} 
\label{fig:detection}
\end{center}
\end{figure*}
\subsection{DL-based Object Detection Methods in Traffic Analysis}


Object detection is another key stage in DL-based processing pipelines for driving safety analysis. Object detection simply means locating different objects in images and video frames, potentially with complex backgrounds, by drawing bounding boxes around the objects of interest.It can coexist or be integrated with object classification and labeling. An illustrative example of vehicle detection using 2 benchmark methods is shown in Fig. \ref{fig:detection}(a)(b). 

Notable examples of object detection in the context of driving safety analysis include detecting surrounding vehicles, humans, traffic signs, and obstacles. It also can be part of more complicated tasks such as traffic distribution and composition analysis, improper lane crossing events, trajectory extraction, speed estimation, moving object tracking, path planning, and detecting vehicles on road shoulders, etc., as presented in Table \ref{tab:problem}.
%\arr{We plan to add this Table to section IV. Sample Problems.} 


Another use case of object detection is removing Personal Identifiable Information (PII), such as masking human face and license plate numbers before publishing traffic video, as shown in Fig. \ref{fig:detection}(c).

%\begin{figure}[h]
%\begin{center}
%\centerline{\includegraphics[width=0.9\columnwidth]{figures/maskedfigure.png}}
%\caption{An example frame with PII removal. The plate masking is barely visible here, so you can present part of the images (like cutting each image into left and right part and show only the right part, also, you can check if yellow color gives a better visibility here.) } 
%\label{fig:PII}
%\end{center}
%\end{figure}


%An important challenge specific to the driving safety analysis is that most object detection algorithms are customized to use horizontal view or inclined view (e.g., MS-COCO\cite{lin2014microsoft}), \ar{or top-view images (e.g., using aerial images captured by drone in \cite{qu2020dilated})} for object detection; while the majority of data for safety metrics comes from tilted cameras in roadside infrastructure with \ar{inclined view?}. % is multi-angle and multi-scale.


Although there exist some datasets for traffic analysis from the roadside cameras \cite{wang2011automatic,morris2011trajectory,hospedales2012video}, still there is a critical need for larger datasets that cover different zones, urban, suburban, and rural setups, residential and high-risk zones, railroads, and environmental conditions.
%The same concept applies to traffic analysis datasets, and there is a critical need for publicly available roadside video datasets.} \arr{verify if there exist some already available, and if yes mention it here}.

Some notable ongoing research problems include solving the trade-off between the algorithm's accuracy and speed, realizing small object detection, distributed and federated learning, model sharing among roadside servers, and  implementing lightweight models and embedded devices appropriate for autonomous vehicles, etc. 



Compared to the conventional object detection algorithms such as Viola-Jones detector\cite{viola2001rapid}, the Histogram of Oriented Gradients (HOG detector)\cite{dalal2005histograms}, and Deformable Part-based Models (DPM)\cite{felzenszwalb2009object} ), CNN-based methods substantially improve the recognition success rate. 

From the implementation point of view, the DL-based algorithms can be divided into one-stage and two-stage methods. The two-stage detectors first generate Regions of Interests (RoIs) and then send the region proposals down the pipeline for object classification and bounding-box regression. R-CNN series\cite{girshick2014rich,girshick2015fast,ren2015faster,dai2016r,pang2019libra} comprises the most popular two-stage algorithm family. 
\ar{The architectures of R-CNN series are shown in Fig. \ref{fig:R-CNN family}.
Specifically,  R-CNN\cite{girshick2014rich} adopts \textit{selective search}\cite{uijlings2013selective} to generate region proposals, and then feed resized (by cropping or warping) proposals into CNN-based backbone to extract features. Finally, SVM performs classification for objects' categories and locations. SPPNet\cite{he2015spatial} introduced \textit{spatial pyramid pooling} (SPP) layers, which solved the fixed-size input issue. Integrated by R-CNN and SPPNet, Fast R-CNN \cite{girshick2015fast} realized \textit{RoI pooling} to output fixed size features and adopted multi-task loss to allow single-stage training. Since Fast R-CNN were still bottlenecked by the \textit{selective search} heavy computation, Faster R-CNN \cite{ren2015faster} introduced \textit{region proposal network} (RPN), an end-to-end trainable network to generate quality region proposals. Mask R-CNN adds a parallel branch to predict the object mask.}

One-stage detectors directly treat object detection tasks as a regression and classification problem. These methods are divided into anchor-free and anchor-based methods. In anchor-based methods, a set of bounding boxes with different predefined sizes are required to capture the scale and aspect ratio of the objects. Some famous implementations include \textit{You Look only Once} (YOLO) family (e.g., YOLOv2 \cite{redmon2017yolo9000}, YOLOv3\cite{redmon2018yolov3}, and YOLOv4\cite{bochkovskiy2020yolov4}, and YOLOv5 \cite{glenn_jocher_2021_4679653}\footnote{Note that the authors of YOLOv5 are different from the previous versions}, as well as the Single Shot multi-box Detector (SSD) series\cite{liu2016ssd}). 
\ar{The basic idea of YOLO is demonstrated in Fig. \ref{fig:YOLO}. The network treats the detection as a regression problem and learns the location and class of each bounding box separately. Specifically, an image is split into $S\times S$ patches. In each patch, the network can predict the coordination of $B$ bounding boxes with their confidence levels as well as the class of each patch. After aggregation, the bounding box of an object is localized with its category. Then, non-maximal suppression is applied to filter out the extra bounding boxes for the same object.}


Recently, anchor-free methods are getting more attention to avoid defining anchor-related hyperparameters and to ease complicated computations. The main ideas include implementation by dense prediction (e.g.,  DenseBox\cite{huang2015densebox}, Fully Convolutional One-Stage (FCOS) object detectors \cite{tian2019fcos}, RetinaNet\cite{lin2017focal}) as well as implementation by keypoints and center points (e.g., CornerNet\cite{law2018cornernet,law2019cornernet}, CenterNet\cite{zhou2019objects, duan2019centernet},ExtremeNet\cite{zhou2019bottom}). 

Generally speaking, two-stage methods can achieve higher accuracy but at lower speeds than the one-stage methods. Some recent one-stage methods (including YOLO V4\cite{bochkovskiy2020yolov4} and SSD\cite{liu2016ssd}) solve the trade-off between the accuracy and speed by realizing a more efficient network structure. A summary of these algorithms' performance is presented in Fig.\ref{fig:detection_per}.


\begin{figure}[h]
\begin{center}
\centerline{\includegraphics[width=1\columnwidth]{figures/object_detect.jpg}}
\caption{Some object detection models perform on MS COCO test-dev.} 
\label{fig:detection_per}
\end{center}
\end{figure}


\begin{comment}


\begin{table*}[]
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline\rowcolor{gray}
\multicolumn{2}{|l|}{\textbf{Stage}} &
  \textbf{Features} &
  \textbf{Methods}\\ \hline
\multicolumn{2}{|l|}{Two-stage} &
 
  \begin{tabular}[c]{@{}l@{}}First, generate region proposal,\\ then do object classification and \\ bounding-box regression\end{tabular}  &  R-CNN family\cite{girshick2014rich,girshick2015fast,ren2015faster,dai2016r,pang2019libra} \\ \hline
\multirow{}{}{One-stage} &
  Anchor-based & \begin{tabular}[c]{@{}l@{}}No need region proposal.\\ Predefined boxes to \\ capture the scale and aspect ratio of the objects.\end{tabular}&
   \begin{tabular}[c]{@{}l@{}}YOLOv2 \cite{redmon2017yolo9000}, YOLOv3\cite{redmon2018yolov3},\\  YOLOv4\cite{bochkovskiy2020yolov4}, \xc{YOLOv5\cite{glenn_jocher_2021_4679653}}, SSD\cite{liu2016ssd}\end{tabular} 
   \\ \cline{2-4} 
 &
  Anchor-free & \begin{tabular}[c]{@{}l@{}}No need region proposal.\\ Implemented by dense prediction or \\ keypoints and centerpoints\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}YOLO\cite{redmon2016you},DenseBox\cite{huang2015densebox},FCOS\cite{tian2019fcos},\\ RetinaNet\cite{lin2017focal},CornerNet\cite{law2018cornernet,law2019cornernet}, \\ CenterNet\cite{zhou2019objects, duan2019centernet}, ExtremeNet\cite{zhou2019bottom}\end{tabular} 
   \\ \hline
\end{tabular}%
}
\caption{A summary of recent DL-based methods for object detection. \arr{candidate to remove if limited in space.}}  %\arr{Switch the 2nd and 3rd columns so "Features go 2nd", then include each method like DenseBox[101] as a separate row. Add another column "Traffic use case" and include papers that use any of these methods for traffic and driving video analysis. These refs do not need to be new ones necessarily; and it is ok to reuse the same references in different Tables like Table 4 and 5. Also, if you didn't find a traffic-related use case for some of the methods, it is fine to leave it blank.}\xc{Xiwen: My think was we can directly remove this table, since it only summarized the different DL methods, and the next table already covered these methods for traffic-related tasks.  And according to the next table, most works are based on YOLO or RCNN, which means there are many methods that we need to leave them blank.  }}
\label{tab:object detection}
\end{table*}

\end{comment}



%\arr{again better to provide examples of how people used these methods for traffic analysis. You can make a table and consider existing and potential applications! Like a table with header: "method[REF]  - one-stage/two-stage - anchor-free/anchor-based - application  accuracy"  and for applications list plate detection, vehicle detection, etc.  Do the same for other sections like video stabilization, classification, .... }

%\xc{There are several tasks for understanding the road users parameters, such as vehicle detection, plate detection, and traffic sign detection. We note that the algorithms we mentioned above often evaluate their performance on the traffic related objects; however, we still want to remark some works that used the outstanding algorithms we discuss before, which is shown on Table.\ref{tab:objectdetection}. We note that some works (such as \cite{6778050,8019461,kim2017deep,selmi2017deep,masood2017license}) tend to fine-tune the CNN framework according to the task requirement, and the recent mainstream traffic works begin to widely deploy R-CNN series, YOLO series, and SSD. It means these algorithms exactly can stand the test of practice, but not means the other algorithms are not favorable. It also may because the complexity of the task is relatively low or the recent detectors are hard to deploy to the real scenarios.}

The applications of object detection methods in traffic video analysis mostly relate to understanding the objects surrounding the road users, such as vehicles, plates, and traffic signs. Most research works in this area adopt one of the aforementioned algorithms for object detection, as summarized in Table \ref{tab:objectdetection}. The metrics used for object detection, recognition, and image segmentation are outlined in Table \ref{tab:somemetrics}.  
We note that some works (such as \cite{6778050,8019461,kim2017deep,selmi2017deep,masood2017license}) tend to fine-tune the CNN framework according to the task requirement, and the recent mainstream traffic works begin to deploy the R-CNN series, YOLO series, and SSD widely. It means these algorithms can stand the test of practice, but it does not mean that the other algorithms are not favorable. It also can be due to the relatively low complexity of this task, or due to the difficulty of deploying recent detectors in real-world scenarios.

%\fbox{Xiwen from here: Pedestrian detection}

\ar{Pedestrians are often the most vulnerable entities on the road, hence pedestrian detection is usually considered a top-priority component of safety assessment and control systems.
Pedestrian detection, especially in crowded areas, would be more complex than similar object detection tasks. Indeed, early CNN-based frameworks underperformed on the task due to the uncertain dense distribution and high dynamics of pedestrians. Some common issues, including the multi-scale problem (different receptive fields with low-information and noisier observations for small-scale pedestrians) and occlusion by crowding (parts of pedestrians are invisible), may challenge these models and decline their accuracy \cite{xiao2021deep}. Some solutions, such as \cite{cai2016unified,li2017scale} addresses the multi-scaling issue by modifying the scale of the region proposals.  Specifically, MS-CNN\cite{cai2016unified} has multiple layers to output features with different receptive fields at the region-proposal sub-network. SAF R-CNN \cite{li2017scale} uses multiple sub-networks to learn the large-scale features and small-scale features, respectively. 
Likewise, \cite{lin2018graininess} uses an attention mechanism by applying a fine-grained attention mask to focus on differently scaled pedestrians. SSA-CA \cite{zhou2019ssa} performs detection after semantic segmentation.}

\ar{Straightforward methods (such as \cite{tian2015deep,xie2021psc}) are proposed to solve the occlusion by enhancing the model to learn patterns with different occlusions. High-level semantic features are employed in \cite{wang2018pcn,liu2019high} to help the occlusion detection. The other explicit solutions \cite{chi2020pedhunter} use data augmentation by introducing extra annotation of the visible parts in the training phase, which substantially enhances the detection ability even under high occlusions. From the author's perspective, the work in \cite{luo2020whether} is very creative, which uses a cycle-consistent adversarial network (Cycle-GAN) \cite{zhu2017unpaired} to translate front view images into bird view images, then solve the detection problem by decomposing it into three subtasks of pedestrian localization, scale prediction, and classification. %addressing three cascade sub-tasks of "where", "what", and "weather" \arr{is the object? is this whether or weather?}\xc{This paper decompose the detection problem into pedestrian localization, scale prediction and classification three sub-tasks}. 
It achieves an outstanding performance of 6.37 miss rate (MR) on Caltech (reasonable) and 9.3 MR on CityPersons (reasonable) datasets.}

\ar{We listed some recent works for pedestrian detection in Table \ref{tab:ped_dect}.  These methods for pedestrian detection are often evaluated on Caltech \cite{dollar2011pedestrian} and CityPersons \cite{dollar2011pedestrian} datasets, which both include person-to-person occlusion caused by crowding and other objects. It it notable that these two datasets are designed specifically for pedestrian detection. A more complicated scenario of detecting vehicles and pedestrians simultaneously, is often validated using auto-driving datasets, such as KITTI \cite{Geiger2012CVPR} (see Table \ref{tab:trafficdataset-continue}).}



\ar{It is noteworthy that some handcrafted features, such as optical flow features, are complementary to deep convolutional features, which can further boost the models' ability \cite{hu2017pushing}. Another interesting problem is pedestrian detection from multi-spectral images (such as RGB true-color + thermal camera feeds, as shown in Fig. \ref{fig:multi_spec}. This approach can be advantageous because infrared images provide more informative and robust features under low illuminations and extreme weather conditions. These works often require \textit{feature fusion} %, meaning how to efficiently integrate features from two spectral images or the extracted features 
to boost the overall performance. Feature fusion can be implemented in different stages, ranging from low-level (near the input layer) to high-level (near the output layer). The authors of \cite{liu2016multispectral} have shown that fusion at the middle-level (the authors name it \textit{halfway fusion}) often achieves the best results. More recently, attention mechanisms, including channel attention and semantic attention, are applied for feature fusion \cite{zhang2019cross} to allow the network automatically learn the importance of different features. Alternatively, an illumination-aware weighting mechanism is used in \cite{li2019illumination} to learn the variation of illumination and adaptively mix the features of the visible (RGB) and thermal images. Some minor issues such as modality imbalance and weak alignment between different channels should be taken care of when fusing multiple camera feeds  \cite{zhou2020improving,zhang2019weakly}. 
A summary of recent implementations is presented in Table. \ref{tab:ped_dect}. KAIST \cite{hwang2015multispectral} and CVC-14 \cite{gonzalez2016pedestrian} datasets are often used as the benchmark validation dataset for these works. More datasets for pedestrian detection are provided in Table. \ref{tab:trafficdataset-continue}.}



\begin{figure}[h]
\begin{center}
\centerline{\includegraphics[width=1\columnwidth]{figures/multi_spec.jpg}}
\caption{\ar{A dual feel camera feed (visible and thermal image pair) for multi-spectral pedestrian detection. Images are from \cite{hwang2015multispectral}.}} 
\label{fig:multi_spec}
\end{center}
\end{figure}





\input{TableOD}

\input{tablePED}

%\cite{yang2015towards}Yang, et al.(2015) MSER+SVM+CNN  98.24GTSDB 98.77CTSD
%These detectors(YOLOv2\cite{redmon2017yolo9000},YOLOv3\cite{redmon2018yolov3}, YOLOv4\cite{bochkovskiy2020yolov4},SSD series\cite{liu2016ssd}) are organized as anchor-based methods, meaning before detection, there a set of bounding box with certain different sizes required to be predefined to capture the scale and aspect ratio of the objects. Recently, anchor-free methods are getting more attention, since they can avoid anchor-related hyperparameters setting and complicated computation. The main ideas include implementation by dense prediction(such as DenseBox\cite{huang2015densebox}, FCOS\cite{tian2019fcos},RetinaNet\cite{lin2017focal}) and implementation by keypoint/centerpoint(such as CornerNet\cite{law2018cornernet,law2019cornernet}, CenterNet\cite{zhou2019objects, duan2019centernet},ExtremeNet\cite{zhou2019bottom}). Generally, two-stage methods can achieve high accuracy but low speed, while one-stage can achieve low  accuracy but high speed; however, recent some state-of-the-arts can solve the trade-off question well (such as YOLO V4\cite{bochkovskiy2020yolov4},SSD\cite{liu2016ssd}).

\begin{figure*}[]
\begin{center}
\centerline{\includegraphics[width=0.8\textwidth]{figures/RCNN_family.png}}
\caption{Network architecture for R-CNN family of localization and segmentation.\xc{miss description (solved)}} 
\label{fig:R-CNN family}
\end{center}
\end{figure*}

\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=1\columnwidth]{figures/YOLO.png}}
\caption{\ar{The demonstration of the basic idea of YOLO.}}
\label{fig:YOLO}
\end{center}
\end{figure}


\subsection{Visual Tracking}\label{sec:tracking}

%\fbox{Ready to review. Also mentioned some pedestrian here} 

Visual tracking refers to capturing the movement of specific objects by processing video frames. Traffic video processing by autonomous vehicles or traffic monitoring systems is perhaps the most popular application of visual tracking. With the advent of AVs and technology-assisted driving systems, this research area has become a hot topic. 
%To evaluate human-driven car safety, visual tracking enables to capture the high-speed vehicles' movement, which allows the following judgment can be executed. 
The mainstream algorithms can roughly be categorized into Correlation Filter-based Trackers (CFT) and non-CFT methods \cite{fiaz2019handcrafted}. The two challenging issues are the natural difficulty of reliable visual tracking and the lack of well-annotated %high-quality 
datasets, especially for driving safety analysis.


Visual tracking methods can be categorized into discriminative methods \cite{hare2015struck,wang2010discriminative,kalal2010pn,wang2014object} and generative methods \cite{kwon2011tracking,sevilla2012distribution,liu2014visual,belagiannis2012segmentation,kwak2011learning} from the modeling standpoint. Generative tracking methods comprise the following sequential steps: (i) extract the target features to learn the appearance model, which represents the target, (ii) search through the image area to find areas that best match the model, using pattern matching. The target information carried by generative models is often richer than that of the discriminative methods. Also, generative models make it is easier to meet the evaluation criteria and the real-time requirements of target tracking when processing a massive amount of data. The key components of generative methods include target representation and target modeling. The limitations of this approach include (i) background information of the image is not fully utilized, and (ii) the appearance of the target in different video frames may include substantial randomness and diversity, which affects the stability of the model.

Discriminative methods turn the tracking problem into a classification problem, and rely on training a classifier to distinguish between the target and the background. The target area is considered the positive sample in the current frame, and the background area is the negative sample. 
Discriminative methods turn the tracking problem into a classification problem, which can simultaneously utilize the information from the target and background. ML methods can be employed to train a binary classifier to distinguish between the target (considered as the positive sample) and the background (considered as the negative samples), and can be updated online as more video frames are accumulated. The trained classifier is used to find the optimal area in the next frame. Discriminative methods are often more robust than generative models when facing appearance and environmental Changes.

%The machine learning method is used to train the classifier online to distinguish the target and the background, and the trained classifier is used to find the optimal area in the next frame. Discriminative methods are often more robust than generative models \ar{[especially]} \ar{in terms of distinguishing the background and information}. \arr{clarify: do you mean discriminative models are in general better for target tracking due to explicitly distinguishing the foreground and background parts of the image, or you mean that they are only better in this sense although they may not be better trackers than the generative ones in general? I guess you mean the second}. 







Correlation Filter (CF) methods and DL methods are often considered discriminant methods. In recent years, tracking methods based on correlation filtering \cite{bolme2010visual,bolme2009average,henriques2012exploiting,henriques2014high,kiani2017learning,li2014scale} have gained a lot of attention from computer vision researchers because of their fast speed and reasonable performance. 

The correlation filter is initialized by the given target in the first frame of the input. 
A classifier is trained by regressing the input features to the target Gaussian distribution. The response peak in the predicted distribution is found in the follow-up tracking step to locate the target's position. 
Correlation filtering methods, when combined with deep features and CNN architectures (e.g., R-CNN series \cite{bewley2016simple,yu2016poi,wojke2017simple}, SSD-based methods \cite{zhao2018multi}) exhibit outstanding performances and hence have gradually become a dominant approach in this field. 

In addition to CF-based trackers, some other DL frameworks, even without using correlation filters, can also achieve an excellent performance. 
More elegant methods, including  \cite{lu2017online,fang2018recurrent,maksai2018eliminating,zhu2018online,ma2018trajectory,sadeghian2017tracking} tried to directly employ sequential learning models such as Long Short Term Memory (LSTM) or Recurrent Neural Networks (RNN) in their network structures after CNN-based feature extractors to capture the temporal information of video frames that represent object motions. 

\ar{Siamese Network structure (shown in Fig.\ref{fig:SiameseNet}) offers a paradigm shift for visual tracking.} %\xc{Xiwen: Just highlight the description of Fig .\ref{fig:SiameseNet} since its label was duplicated. } 
The core idea of Siamese networks \cite{kim2016similarity,wang2016joint,leal2016learning,son2017multi,zhou2018online,wang2019fast,li2019siamrpn++} is training twin networks to identify the similarity between two different images, such as the same object in consecutive video frames. 
These methods address both the similarity knowledge learning and the real-time operation requirements with acceptable tracking accuracy.  

\begin{figure}[h]
\begin{center}
\centerline{\includegraphics[width=0.9\columnwidth]{figures/SiameseNet.png}}
\caption{\ar{The architecture of basic Siamese neural network for similarity training.}}% \xc{label was duplicated}}% Source from \cite{kim2016similarity}.}
\label{fig:SiameseNet}
\end{center}
\end{figure}



Many contemporary traffic monitoring systems still tend to use conventional tracking methods such as filtering and convolution methods due to their efficiency, low complexity, and stability. For examples, methods based on Kalman filtering \cite{dinh2017development,kaur2016vehicle,o2010rear,teoh2012reliability,khalkhali2020vehicle}, Gaussian Mixture Models (GMM) \cite{chen2012vehicle,dinh2017development}, Hidden Markov Models (HMM) \cite{jazayeri2011vehicle}, and SIFT-based methods\cite{luvizon2016video,yang2016research} are used in traffic monitoring systems. However, using DL-based methods is gaining traction in recent years to perform traffic monitoring tasks due to the emergence of powerful and low-cost processing platforms, making DL methods more affordable and near real-time. 


Hybrid methods that enable tracking by detection are another possibility. For instance, a DL method can be used for fast and accurate object detection, followed by a second estimator based on conventional methods, Kalman filtering, and Kanade–Lucas–Tomasi (KLT) feature tracker for tracking purposes. \ar{This approach simplifies the processing job for object detectors designed for specific tasks, such as multi-spectral pedestrian detection. }

A summary of some important implementations is presented in Table \ref{tab:trackingontraffic}. \ar{Note that datasets KITTI, and MOT 15 Challenges \cite{leal2015motchallenge} include pedestrians, in addition to vehicles. Several studies, including \cite{scheidegger2018mono,zou2019multi,fernandez2019real}, are specifically designed to improve the safety of humans.}




%Since the efficiency and stability of the conventional methods.even recently, many works for traffic monitoring still tend to deploy these methods as their top priority. For examples, kalman filter based works\cite{dinh2017development,kaur2016vehicle,o2010rear,teoh2012reliability,khalkhali2020vehicle}, GMM methods\cite{chen2012vehicle,dinh2017development}, HMM methods\cite{jazayeri2011vehicle}, and SIFT-based methods\cite{luvizon2016video,yang2016research}. We still find some works tried to use deep learning to solve the task. The deep learning methods tend to tracking by detecting, meaning that the frameworks often have a fast detector head, then some frameworks use the outputs from the detector to do a second estimate by conventional methods such as Kalman filter or KLT. A summary of these works is shown on Table.\ref{tab:trackingontraffic}


\begin{comment}


\begin{table*}
\centering
\caption{Some traffic-related visual tracking method that use deep learning. The default dataset is generated by the author of each work. The default performance metric is accuracy unless specified otherwise.}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|} 
\hline\rowcolor{gray}
\textbf{Paper: [Ref] Authors (year)} & \textbf{Methods}                        & \textbf{Performance}                                                                                                             \\ 
\hline
\cite{qiu2018kestrel}Qiu, et al.(2018)     & YOLO+KLT                       & 76.4\% Recall 88.2\% Precision                                                                                               \\ 
\hline
\cite{lopez2019boosting}L{\'o}pez-Sastre, et al.(2019)    & Faster R-CNN                   & \begin{tabular}[c]{@{}l@{}}30.5AP on subset:M-30 66.2\%AP on subset:M-30-HD~\\38.1\%AP on subset:Urban1 of GRAM-RTM\end{tabular}  \\ 

\hline
\cite{scheidegger2018mono}Scheidegger, et al.(2018)     & CNN+PMBM filter\cite{garcia2018poisson}                & 80.04\% MOTA on KITTI                                                                                                     \\ 
\hline
\cite{zou2019multi}Zou, et al.(2019)     & Siamese network+SPP+MDP        & \begin{tabular}[c]{@{}l@{}}75.29\% MOTA campus~\\76.06\% MOTAurban~\\78.14\% MOTA highway~\\on KITTI\end{tabular}                \\ 
\hline
\cite{li2019spatio}Li, et al.(2019)     & FPN+tracking loss              & 83.2\% IDF1 on nivida AI city                                                                                                 \\ 
\hline
\cite{nikodem2020multi}Nikodem, et al.(2020)     & hourglass                      & \begin{tabular}[c]{@{}l@{}}MOTA 97+\%\\MCTA 91+\%\end{tabular}                                                              \\ 
\hline
\cite{zhao2018autonomous}zhao, et al.(2018)     & SSD+dual Kalman filters        & Shown in the form of figures                                                                                            \\ 
\hline
\cite{wang2019orientation}Wang, et al.(2019)     & YOLOv3+SIFT                    & 81.3\% MOTA                                                                                                                  \\ 
\hline
\cite{usmankhujaev2020real}Usmankhujaev, et al.(2020)    & yoloV3+kalman filter           & \begin{tabular}[c]{@{}l@{}}100\% Daytime~Wrong cases detection\\89.83\% Daytime(flipped) Wrong cases detection~\\86.11\% Nighttime(flipped) Wrong cases detection\end{tabular}                 \\ 
\hline
\cite{kwan2018compressive}Kwan, et al.(2018)    & ResNet                         & For compressive measurements                                                                                            \\ 
\hline
\cite{fernandez2019real}Fern{\'a}ndez-Sanjurjo,et al.(2019)    & CNN detector+DCF+Kalman filter & 86.96\% MOTA on MOT 15\cite{leal2015motchallenge}                                                                                                    \\
\hline
\end{tabular}
}
\label{tab:trackingontraffic}
\end{table*}
\end{comment}

\begin{table*}
\centering
\caption{Some traffic-related visual tracking method that use deep learning. The default dataset is generated by the author of each work. The default performance metric is accuracy unless specified otherwise.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lll} 
\toprule
\textbf{Paper: [Ref] Authors (year)} & \textbf{Methods}                        & \textbf{Performance}                                                                                                             \\ 
\midrule
\cite{qiu2018kestrel}Qiu, et al.(2018)     & YOLO+KLT                       & 76.4\% Recall 88.2\% Precision                                                                                               \\ 
\midrule
\cite{lopez2019boosting}L{\'o}pez-Sastre, et al.(2019)    & Faster R-CNN                   & \begin{tabular}[c]{@{}l@{}}30.5AP on subset:M-30 66.2\%AP on subset:M-30-HD~\\38.1\%AP on subset:Urban1 of GRAM-RTM\end{tabular}  \\ 

\midrule
\cite{scheidegger2018mono}Scheidegger, et al.(2018)     & CNN+PMBM filter\cite{garcia2018poisson}                & 80.04\% MOTA on KITTI                                                                                                     \\ 
\midrule
\cite{zou2019multi}Zou, et al.(2019)     & Siamese network+SPP+MDP        & \begin{tabular}[c]{@{}l@{}}75.29\% MOTA campus~\\76.06\% MOTAurban~\\78.14\% MOTA highway~\\on KITTI\end{tabular}                \\ 
\midrule
\cite{li2019spatio}Li, et al.(2019)     & FPN+tracking loss              & 83.2\% IDF1 on nivida AI city                                                                                                 \\ 
\midrule
\cite{nikodem2020multi}Nikodem, et al.(2020)     & hourglass                      & \begin{tabular}[c]{@{}l@{}}MOTA 97+\%\\MCTA 91+\%\end{tabular}                                                              \\ 
\midrule
\cite{zhao2018autonomous}zhao, et al.(2018)     & SSD+dual Kalman filters        & Shown in the form of figures                                                                                            \\ 
\midrule
\cite{wang2019orientation}Wang, et al.(2019)     & YOLOv3+SIFT                    & 81.3\% MOTA                                                                                                                  \\ 
\midrule
\cite{usmankhujaev2020real}Usmankhujaev, et al.(2020)    & yoloV3+kalman filter           & \begin{tabular}[c]{@{}l@{}}100\% Daytime~Wrong cases detection\\89.83\% Daytime(flipped) Wrong cases detection~\\86.11\% Nighttime(flipped) Wrong cases detection\end{tabular}                 \\ 
\midrule
\cite{kwan2018compressive}Kwan, et al.(2018)    & ResNet                         & For compressive measurements                                                                                            \\ 
\midrule
\cite{fernandez2019real}Fern{\'a}ndez-Sanjurjo,et al.(2019)    & CNN detector+DCF+Kalman filter & 86.96\% MOTA on MOT 15\cite{leal2015motchallenge}                                                                                                    \\
\bottomrule
\end{tabular}
}
\label{tab:trackingontraffic}
\end{table*}

%How to ensure tracking speed while using deep features to improve tracking is a problem that needs to be solved. 







%\subsection{Dataset and Benchmarks}
%\begin{itemize}
 %   \item KITTI Tracking dataset\cite{Geiger2012CVPR}
 %   \item VOT\cite{VOT_TPAMI}
%    \item OBT\cite{}
 %   \item UAV123\cite{mueller2016benchmark}
%\end{itemize}

\subsection{Semantic Segmentation}\label{sec:Semantic Seg}



Semantic segmentation, where objects of different types are separated, can be considered the heart of many video processing tasks. For instance, vehicle detection, vehicle tracking, and environment perception in a crowded environment with interlaced and overlapping objects can be powered by semantic segmentation when regular segmentation methods fail to separate objects from complex backgrounds. \ar{An example of semantic segmentation is shown in Fig. \ref{fig:diffSeg}(b).} The purpose of semantic segmentation is to label each pixel of an image to represent different categories (e.g., cars, pedestrians, roadside infrastructures, traffic signs, etc.). For instance, semantic segmentation can be employed by an autonomous vehicle for background modeling, identifying road boundaries and free spaces, and detecting lane markings and traffic signs. Semantic segmentation can also be used by an external traffic monitoring system for analyzing the behaviors of human-driven and self-driving vehicles in specific zones and times. To avoid reliance on massive data collection and expensive annotations, semi-supervised and weakly-supervised learning methods \cite{wei2018revisiting,hong2015decoupled,souly2017semi,hung2018adversarial} are developed for low-cost implementation with reasonable performance. 

\begin{figure}[h]
\begin{center}
\centerline{\includegraphics[width=0.99\columnwidth]{figures/diff_typy_seg_new.jpg}}  %diff_typy_seg.png
\caption{A example of different types of segmentation. Source from \cite{kirillov2019panoptic}.} %\xc{miss description. label was duplicated. (solved) }}
%\xc{Do we need to mention 'panoptic segmentation', since it is shown in the figure}} %lets skip
\label{fig:diffSeg}  %\xc{orignal is SiameseNet}
\end{center}
\end{figure}

Early works tended to deploy existing classification algorithms at the patch level for semantic segmentation. Since 2014, Fully Convolutional Network (FCN)\cite{long2015fully} was introduced that allows spatially dense prediction tasks by translating famous DL architectures such as AlexNet, VGG net, and GoogLeNet into fully convolutional network architectures.  
Afterward, many upgraded architectures such as U-net\cite{UNET} and SegNet\cite{badrinarayanan2017segnet} were proposed, which build upon the concept of FCN and utilize auto-encoder architectures for semantic segmentation with small training datasets using data augmentation methods. This architecture is further updated to multi-stage auto-encoder networks in \cite{cheng2019spgnet}.
In some work\cite{yu2015multi,chen2017deeplab,paszke2016enet,chen2017rethinking}, atrous/dilated convolution architectures are used to keep spatial resolution and expand the receptive fields. The authors of \cite{peng2017large} expanded the receptive fields by employing large kernel with its proposed global convolution.

In \cite{liu2015parsenet,pinheiro2016learning,lin2017refinenet}, a feature fusion method is deployed that allows the framework to learn global features merged with more local features. For these methods, Conditional Random Fields can be used to enhance the output. Other works \cite{visin2016reseg,li2016lstm} are based on a Recurrent Neural Network (RNN) structure that can better tackle sequence-related tasks. Additional models including\cite{zhang2019dual} based on graph convolutional network, \cite{zhao2017pyramid} based on pyramid pooling model, and \cite{yuan2020object} based on learning relations between the object region and pixels have competitive performance. Furthermore,  \cite{qi2017pointnet,qi2017pointnet++,huang2016point} focused on semantic segmentation with 3D point cloud data, which have great potentials for autonomous driving and traffic safety analysis. More specifically, the methods \cite{qi2017pointnet,qi2017pointnet++} are evaluated by indoor scene dataset, while \cite{huang2016point} is evaluated by urban scene captured by scanners, something potentially more relevant for traffic analysis. The performance of some models is shown in Fig.\ref{fig:semantic_perf}.


The applications of semantic segmentation frequently appear in the world of AVs. Some examples include (i) scene understanding, which involves understanding the traffic environment with road users, (ii) free space estimation to determine the available spaces on the road that a vehicle is allowed to use with no collisions, and (iii) Stixel representation, which assigns each pixel with a 3D depth information. A summary of related works is presented in Table \ref{tab:semanticwork}. 

\begin{figure}[h]
\begin{center}
\centerline{\includegraphics[width=1\columnwidth]{figures/semantic.jpg}}
\caption{Semantic segmentation models perform on Cityscapes.}
\label{fig:semantic_perf}
\end{center}
\end{figure}


%To understand the traffic environment scene, ERFNET\cite{romera2017erfnet} proposed a autoencoder-based framework with a novel layer that leverages skip connections and convolutions with 1D kernels, which can boost the inference speed with the a similar accuracy to the 2D kernels. ESnet\cite{lyu2019esnet} accelerate the segmentation process by incorporating high-resolution of global edge information with low-resolution of classification level semantic information. Moreover, \cite{deng2017cnn,saez2018cnn} made the progress on segmentation for scenes captured by fisheye camera. \cite{deng2017cnn} propose Overlapping Pyramid Pooling (OPP) module that incorporate the local, global and pyramid local region context information. \cite{saez2018cnn} applies ERFnet to process the data from fisheye camera and present a new fisheye image dataset for semantic segmentation from the existing CityScapes dataset\cite{}.  



%-free space estimation(obstacle): Free space is defined as the available space on the ground surface where navigation of vehicle is guaranteed without collision.
%\cite{kendall2015bayesian,ohgushi2020road,hua2019small,levi2015stixelnet,deepika2017obstacle}

%-Stixel representation: 
%The Stixel World  is a segmentation of an image into superpixels, where each superpixel is a thin stick-like segment with a class label and a 3D planar depth model.
%\cite{cordts2017stixel,schneider2016semantic,erbs2012stixmentation}



\begin{comment}


\begin{table*}
\centering
\resizebox{\textwidth}{!}{
\caption{Some semantic segmentation works in the traffic field.}
\begin{tabular}{|l|l|l|l|} 
\hline\rowcolor{gray}
\textbf{Task}                  & \textbf{Paper: [Ref] Authors (year)}                                                           & \textbf{Methods}                                                                                                                                                & \textbf{Performance}                                                                                                                                                           \\ 
\hline
Scene understanding   & \begin{tabular}[c]{@{}l@{}}\cite{romera2017erfnet}Romera, et al(2017)\\ \cite{lyu2019esnet}Lyu et al.(2019)\\  \cite{deng2017cnn}Deng, et al.(2017) \\ \cite{saez2018cnn}Sáez, et al.(2018)\\ \cite{kendall2015bayesian}Kendall, et al.\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Autoencoder\\ Edge Detection Network+Fusion\\ CNN+pyramid pooling module\\ Autoencoder\\ Bayesian Autoencoder \end{tabular} & \begin{tabular}[c]{@{}l@{}}pixel accuracy$>$95\% Cityscapes\\63.2\% mIoU Cityscapes\\54.5\% mIoU Cityscapes\\59.3\% mIoU Cityscapes\\63.1\% mIoU CamVid\end{tabular}            \\ 
\hline
Free space estimation & \begin{tabular}[c]{@{}l@{}} \cite{ohgushi2020road}Ohgushi, et al.(2020)\\ \cite{hua2019small}Hua, et al.(2019)\\\\ \cite{levi2015stixelnet}Levi, et al.(2015)\\ \\ \cite{deepika2017obstacle}Deepika, et al.(2017)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Autoencoder\\ Autoencoder+fusion+optical flow\\ \\ CNN\\ \\ SegNet \end{tabular}                                          & \begin{tabular}[c]{@{}l@{}}21.9\% mIoU\\Path planning accuracy\\0.15m Indoor and 0.27m Outdoor\\0.87 AUC~\\89.12\% maxF SEGMENTATION on KITTI\\0.9667 IoU\end{tabular}  \\ 
\hline
Stixel representation & \begin{tabular}[c]{@{}l@{}}\cite{schneider2016semantic}Schneider,  et al.(2016)\\\cite{cordts2017stixel}Cordts,  et al. (2017)\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}FCN+SGM\\ FCN+SGM+graphical model \end{tabular}                                                                             & \begin{tabular}[c]{@{}l@{}}7.8 Disparity Error on KITTI 15.2\% on Ladicky\\83.1\% exact Disparity accuracy\end{tabular}                                                   \\
\hline
\end{tabular}}
\caption{Some semantic segmentation works in the traffic field.}
\label{tab:semanticwork}
\end{table*}
\end{comment}








































































\begin{table*}
\centering
\caption{Some semantic segmentation works in the traffic field.}
\resizebox{\textwidth}{!}{
\begin{tabular}{llll} 
\toprule
\textbf{Task}                  & \textbf{Paper: [Ref] Authors (year)}                                                           & \textbf{Methods}                                                                                                                                                & \textbf{Performance}                                                                                                                                                           \\ 
\midrule
Scene understanding   & \begin{tabular}[c]{@{}l@{}}\cite{romera2017erfnet}Romera, et al(2017)\\ \cite{lyu2019esnet}Lyu et al.(2019)\\  \cite{deng2017cnn}Deng, et al.(2017) \\ \cite{saez2018cnn}Sáez, et al.(2018)\\ \cite{kendall2015bayesian}Kendall, et al.\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Autoencoder\\ Edge Detection Network+Fusion\\ CNN+pyramid pooling module\\ Autoencoder\\ Bayesian Autoencoder \end{tabular} & \begin{tabular}[c]{@{}l@{}}pixel accuracy$>$95\% Cityscapes\\63.2\% mIoU Cityscapes\\54.5\% mIoU Cityscapes\\59.3\% mIoU Cityscapes\\63.1\% mIoU CamVid\end{tabular}            \\ 
\midrule
Free space estimation & \begin{tabular}[c]{@{}l@{}} \cite{ohgushi2020road}Ohgushi, et al.(2020)\\ \cite{hua2019small}Hua, et al.(2019)\\\\ \cite{levi2015stixelnet}Levi, et al.(2015)\\ \\ \cite{deepika2017obstacle}Deepika, et al.(2017)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Autoencoder\\ Autoencoder+fusion+optical flow\\ \\ CNN\\ \\ SegNet \end{tabular}                                          & \begin{tabular}[c]{@{}l@{}}21.9\% mIoU\\Path planning accuracy\\0.15m Indoor and 0.27m Outdoor\\0.87 AUC~\\89.12\% maxF SEGMENTATION on KITTI\\0.9667 IoU\end{tabular}  \\ 
\midrule
Stixel representation & \begin{tabular}[c]{@{}l@{}}\cite{schneider2016semantic}Schneider,  et al.(2016)\\\cite{cordts2017stixel}Cordts,  et al. (2017)\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}FCN+SGM\\ FCN+SGM+graphical model \end{tabular}                                                                             & \begin{tabular}[c]{@{}l@{}}7.8 Disparity Error on KITTI 15.2\% on Ladicky\\83.1\% exact Disparity accuracy\end{tabular}                                                   \\
\bottomrule
\end{tabular}}

\label{tab:semanticwork}
\end{table*}


%romera2017erfnet pixel accuracy$>$95 Cityscapes
%,lyu2019esnet 63.2 mIoU Cityscapes 
%,deng2017cnn   54.5 mIoU Cityscapes
%,saez2018cnn   59.3  mIoU Cityscapes
%kendall2015bayesian 63.1 mIoU  CamVid

%,ohgushi2020road 21.9 mIoU 
%,hua2019small . Path planning accuracy 0.15m Indoor 0.27m Outdoor
%,levi2015stixelnet  0.87 OBTICLE DETECTION  89.12\% maxF SEGMENTATION   KITTI
%,deepika2017obstacle 0.9667 IoU
 
%cordts2017stixel 83.1 exact Disparity accuracy data generated from Cityscapes
%,schneider2016semantic  the subset of Kitti [2] annotated\cite{ladicky2014pulling}.
%,erbs2012stixmentation  88.64 Stixel-wise percentage accuracy
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

\begin{comment}


\begin{table*}[htbp]
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{|l|l|} 
\hline\rowcolor{gray}
\textbf{Metric}                                   & \textbf{Definition}                                                                                                                                                                                                                                                                                                                                        \\ 
\hline
Accuracy                                 & $\frac{\text{Correct predictions}}{\text{Total predictions}}$                                                                                                                                                                                                                                                                                                   \\ 
\hline
Recall (R)                               & $\frac{TP}{TP+FN}$ ~~~ (*)                                                                                                                                                                                                                                                                                                                                \\ 
\hline
Precision (P)                            & $\frac{TP}{TP+FP}$                                                                                                                                                                                                                                                                                                                                \\ 
\hline
F1 score                                 & $2\times\frac{P\times R}{P+ R}$                                                                                                                                                                                                                                                                                                                   \\ 
\hline
Pixel Accuracy (PA)                      & $\frac{TP+TN}{TP+TN+FP+FN}$                                                                                                                                                                                                                                                                                                                       \\ 
\hline
Normalized error (mean)                  & \begin{tabular}[c]{@{}l@{}} Normalized error=$\frac{|d-d_{gt}|}{d_{gt}}$. \\ $d$ is the calculated distance and \\ $d_{gt}$ is the ground truth of distance. \end{tabular}                                                                                                                                                                         \\ 
\hline
Average Precision (AP)                   & $AP=\int_0^1 P(R)dR$ P-R CURVE (for one class)                                                                                                                                                                                                                                                                                                    \\ 
\hline
mean Average Precision (mAP)             & $mean(AP_i)$                                                                                                                                                                                                                                                                                                                                      \\ 
\hline
Intersection over Union (IoU)            & \begin{tabular}[c]{@{}l@{}}$\frac{B_p\cap B_{gt}}{B_p\cup B_{gt}}$\\ $B_{gt}$: ground truth bounding box\\ $B_{p}$: predicted bounding box \end{tabular}                                                                                                                                                                                          \\ 
\hline
Disparity accuracy\cite{menze2015object}                      &  $disparity_{inlier}\%$. The disparity $\leq$ 3px/5\% is true                                                                                                                                                                                                                                                                                                                                         \\ 
\hline
Stixel-wise percentage accuracy          & Similar to PA                                                                                                                                                                                                                                                                                                                                     \\ 
\hline
Identification F1-Score ($ID:F1$)           & $ID:F1=\frac{2ID:TP}{2ID:TP+ID:FP+ID:FN}$                                                                                                                                                                                                                                                                                                              \\ 
\hline
multiple object tracking accuracy (MOTA) & \begin{tabular}[c]{@{}l@{}}$MOTA=1-\frac{FN+FP+\Phi}{T}$\\ $\Phi$ denotes the number of fragmentations \end{tabular}                                                                                                                                                                                                                              \\ 
\hline
Multi-camera Tracking Accuracy (MCTA)    & \begin{tabular}[c]{@{}l@{}}$MCTA= \underbrace{\frac{2PR}{P+R}}_{F_1} \underbrace{(1-\frac{M^w}{T^w})}_{\text{within camera}} \underbrace{(1-\frac{M^h}{T^h})}_{\text{handover}}$\\ $M^w$: within-camera identity mismatches \\ $T^w$: true within-camera detections\\ $M^h$: handover mismatches\\ $T^h$: true handover detections \end{tabular}  \\ 
\hline
RMSE                                     & $RMSE=\sqrt{\sum_{i=1}^N(p_i-a_i)^2/N}$                                                                                                                                                                                                                                                                                                           \\
\hline
\end{tabular}
}
\caption{Some metrics to evaluate traffic works. \\ *: TP:True Positive, TN: True Negative, FP:False Positive, FN:False Negative.}
\label{tab:somemetrics}
\end{table*}

\end{comment}

\begin{table*}[htbp]
\centering
\caption{\ar{Evaluation metrics for different vision-based traffic analysis tasks (detection, classification, etc.)}}% for traffic works, including TP:True Positive, TN: True Negative, FP:False Positive, FN:False Negative. \xc{add Miss Rate}}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{ll} 
\toprule
\textbf{Metric}                                   & \textbf{Definition}                                                                                                                                                                                                                                                                                                                                        \\ 
\midrule
Accuracy                                 & $\frac{\text{Correct predictions}}{\text{Total predictions}}$                                                                                                                                                                                                                                                                                                   \\ 
\midrule
Recall (R)                               & $\frac{TP}{TP+FN}$ ~~~ (*)                                                                                                                                                                                                                                                                                                                                \\ 
\midrule
Precision (P)                            & $\frac{TP}{TP+FP}$                                                                                                                                                                                                                                                                                                                                \\ 
\midrule
F1 score                                 & $2\times\frac{P\times R}{P+ R}$                                                                                                                                                                                                                                                                                                                   \\ 
\midrule
Pixel Accuracy (PA)                      & $\frac{TP+TN}{TP+TN+FP+FN}$                                                                                                                                                                                                                                                                                                                       \\ 
\midrule
\ar{Miss Rate (MR)}                              & \ar{$\frac{FN}{TP+FN}$}                                                                                                                                                                                                                                                                                                                                \\  \midrule
Normalized error (mean)                  & \begin{tabular}[c]{@{}l@{}} Normalized error=$\frac{|d-d_{gt}|}{d_{gt}}$. \\ $d$ is the calculated distance and \\ $d_{gt}$ is the ground truth of distance. \end{tabular}                                                                                                                                                                         \\ 
\midrule
Average Precision (AP)                   & $AP=\int_0^1 P(R)dR$ P-R CURVE (for one class)                                                                                                                                                                                                                                                                                                    \\ 
\midrule
mean Average Precision (mAP)             & $mean(AP_i)$                                                                                                                                                                                                                                                                                                                                      \\ 
\midrule
Intersection over Union (IoU)            & \begin{tabular}[c]{@{}l@{}}$\frac{B_p\cap B_{gt}}{B_p\cup B_{gt}}$\\ $B_{gt}$: ground truth bounding box\\ $B_{p}$: predicted bounding box \end{tabular}                                                                                                                                                                                          \\ 
\midrule
Disparity accuracy\cite{menze2015object}                      &  $disparity_{inlier}\%$. The disparity $\leq$ 3px/5\% is true                                                                                                                                                                                                                                                                                                                                         \\ 
\midrule
Stixel-wise percentage accuracy          & Similar to PA                                                                                                                                                                                                                                                                                                                                     \\ 
\midrule
Identification F1-Score ($ID:F1$)           & $ID:F1=\frac{2ID:TP}{2ID:TP+ID:FP+ID:FN}$                                                                                                                                                                                                                                                                                                              \\ 
\midrule
multiple object tracking accuracy (MOTA) & \begin{tabular}[c]{@{}l@{}}$MOTA=1-\frac{FN+FP+\Phi}{T}$\\ $\Phi$ denotes the number of fragmentations \end{tabular}                                                                                                                                                                                                                              \\ 
\midrule
Multi-camera Tracking Accuracy (MCTA)    & \begin{tabular}[c]{@{}l@{}}$MCTA= \underbrace{\frac{2PR}{P+R}}_{F_1} \underbrace{(1-\frac{M^w}{T^w})}_{\text{within camera}} \underbrace{(1-\frac{M^h}{T^h})}_{\text{handover}}$\\ $M^w$: within-camera identity mismatches \\ $T^w$: true within-camera detections\\ $M^h$: handover mismatches\\ $T^h$: true handover detections \end{tabular}  \\ 
\midrule
RMSE                                     & %$RMSE=\sqrt{\sum_{i=1}^N(p_i-a_i)^2/N}$
$RMSE=\sqrt{\sum_{i=1}^N(y_i-\hat{y}_i)^2/N}$                                                                                                                                                                                                                                                                                                           \\
\bottomrule
\end{tabular}
}

\label{tab:somemetrics}
\end{table*}

%A disparity estimation with an absolute deviation of less than or
%equal to 3 px and a relative deviation less than 5% compared to
%ground truth is considered as an inlier



%\subsection{Dataset and Benchmarks}
%Semantic Boundaries Dataset\cite{hariharan2011semantic},  MIT Scene paring data(ADE20K)\cite{zhou2019semantic}



\subsection{Instance Segmentation}\label{sec:Instance Segmentation Problem definition}
Instance segmentation, which deals with detecting and delineating distinct objects of interest in images and video frames, can be considered as one of the most difficult tasks in computer vision \ar{(Fig. \ref{fig:diffSeg}(c))}. It goes one step beyond semantic segmentation and not only labels the pixels based on their object categories, but also distinguishes between different object instances of the same type. This is of crucial importance for traffic imagery analysis in dense zones, where different objects (e.g., vehicles, pedestrians) have to be identified and located in video frames for optimal decision making by AVs, or to extract safety metrics by monitoring systems. 
In contrast to semantic segmentation, instance segmentation only needs to find the edge contour of the object of interest with no need for bounding boxes, hence it can realize a more accurate object detection when assessing the behaviors of vehicles.
%\arr{do you mean: without the need for using bounding boxes? otherwise mention why "the effect of bounding boxes" is something negative.}\xc{Here means use a bounding box to evaluate an object must contain other edge information that not belongs to the object, and directly use contour to evaluate the object can obtain more information and would be more accurate.}. 
Building a reliable and real-time method, for instance, segmentation, especially for crowded zones and under highly distorted traffic videos (e.g., in rainy and cloudy weather conditions), can be challenging. 


Instance segmentation can be divided into one-stage and two-stage methods. Two-stage methods often require generating region or object proposals followed by a classification-based segmentation performed over the features extracted from the selected regions or bounding boxes around object proposals. To generate region proposal, \cite{hariharan2014simultaneous,dai2016MNC,he2017mask} predict a bounding box for each instance, while \cite{pinheiro2015learning,pinheiro2016learning,dai2016instance,li2017fully}  develop pixel-wise coarse segmentation masks. 

Since instance segmentation partitions the image by masking the detected objects and associating each pixel with a distinct object, some two-stage detectors such as Faster R-CNN \cite{ren2015faster}) can execute instance segmentation task after some post-processing, e.g., by adding a branch for mask predictions. 


One-stage instance segmentation methods do not utilize a separate stage for generating region proposals; rather, they apply the segmentation directly to the original images. Some methods \cite{bolya2019yolact,bolya2019yolact++,wang2019solo,wang2020solov2} inspired by one-stage detectors (such as YOLO\cite{redmon2017yolo9000}) directly predict bounding boxes. However, these anchor-based methods heavily rely on predefined anchors, which may be affected by many factors such as the predefined anchor boxes' aspect ratio and scales. Another approach is developing anchor-free methods using dense prediction or centerpoint/keypoints. For instance, \cite{chen2020blendmask,lee2020centermask,xie2020polarmask} relied on FCOS\cite{tian2019fcos} as their dense prediction detector, while ExtremeNet\cite{zhou2019bottom} is a keypoint-based detector that can roughly perform the segmentation task. The difference between the accuracy of one-stage and two-stage methods is not as great as one may expect. Indeed, recent one-stage methods such as CenterMask\cite{lee2020centermask} can perform real-time inference with accuracy as high as two-stage methods, or even better. The performance of some instance segmentation models is shown in Fig.\ref{fig:instance_perf}.

\begin{figure}[h]
\begin{center}
\centerline{\includegraphics[width=1\columnwidth]{figures/instance.jpg}}
\caption{Instance segmentation models perform on MS COCO test-dev }
\label{fig:instance_perf}
\end{center}
\end{figure}


In the context of traffic analysis, instance segmentation can be used not only to identify and locate vehicles but also to obtain detailed information about the vehicle, such as a vehicle's class, number of axles, 3D bounding box, dimension, etc. It can be used as part of the processing to identify road lanes, traffic volume, etc. For instance, one may consider each lane as an instance. Some famous methods that utilize instance segmentation for traffic image analysis are presented in Table \ref{tab:instancework}.


%In traffic safety works, instance segmentation is used to 
%-obtain comprehensive vehicle information, such as type, number of axles, 3D bounding box, speed, length, current driving lane, and traffic volume.\cite{zhang2015monocular,mou2018vehicle,zhang2020traffic,huang2018measuring}
%- Lane detection\cite{neven2018towards,roberts2018dataset,roberts2018dataset}
%- 3D reconstruction\cite{schurischuster2020time,hadi2020semantic}



%zhang2015monocular  59.0 object recall and 83.1\% of the randomly sampled foreground pixel pairs ordered KITTI
%mou2018vehicle   95.87 F1 score  ISPRS
%,zhang2020traffic vehicle types and number of axles are more than 97\% and 88\%
%,huang2018measuring normalized error = $\frac{d-d_1}{d}$ d is the calculated distance and dt is the ground truth of distance. 1.333 front 4.698 side-way KITTI

%neven2018towards  96.4 acc is the average correct number
%of points per image $sum_{im}\frac{C_{im}}{S_{im}}$ tuSimple lane dataset  
%,roberts2018dataset IoU Mapillary 82.9  CityScapes 85.2 KITTI 83.8  aUthor's dataset 95
%,roberts2018dataset

%schurischuster2020time worng
%,hadi2020semantic AP@50\% 8.862 CityScaoes 43.949 IDD\cite{varma2019idd} 5.643 WildDash\cite{zendel2018wilddash}


%  The popular one-stage anchor-free detectors involve YOLO\cite{},RetinaNet\cite{lin2017focal}, and FCOS\cite{tian2019fcos}). 
%Similarly, more-than-one methods often contain these two steps: Region Proposal(also known as detect Interests of Region), and then segmentation. The main ideas of region proposal contain bounding-box-based(\textbf{SDS}\cite{hariharan2014simultaneous}, \textbf{MNC}\cite{dai2016MNC}, \textbf{Mask R-CNN}\cite{he2017mask}), segmentation-mask-based (\textbf{DeepMask}\cite{pinheiro2015learning}, \textbf{SharpMask}\cite{pinheiro2016learning}, and \textbf{FCIS}\cite{li2017fully}). 


%As we discussed in Section.\ref{sec:Instance Segmentation Problem definition}, Instance segmentation involves the object detection task, meaning some deep-learning-based object detection models (such as R-CNN\cite{girshick2014rich}, Fast R-CNN\cite{girshick2015fast}, Faster R-CNN\cite{ren2015faster}) can be applied or improved in Instance segmentation models. Proposal methods MCG\cite{arbelaez2014multiscale}(for SDS), ...(from MCN paper)   



%One-stage methods are also known as proposal-free methods, meaning these methods are not required to produce a region proposal before segmentation. Ideally, proposal-free should be faster but less accurate than proposal-based methods.


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}


\begin{comment}

\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{

\begin{tabular}{|l|l|l|l|} 
\hline\rowcolor{gray}
\textbf{Task }                                                                               & \textbf{[REF] authors (Year)}                                                     & \textbf{Methods}                                                                                  &\textbf{Performance}                                                                                                                                                                                                                   \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Obtain comprehensive\\ vehicle information \end{tabular} & \begin{tabular}[c]{@{}l@{}}\cite{zhang2015monocular}Zhang, et al.(2015)\\~\\ \cite{mou2018vehicle}Mou, et al.(2018)\\ \cite{zhang2020traffic}Zhang, et al.(2020)\\ \cite{huang2018measuring}Huang, et al.(2018) \end{tabular} & \begin{tabular}[c]{@{}l@{}}CNN+MRF\\ ~\\ ResFCN\\ Mask R-CNN\\ Mask R-CNN \end{tabular} & \begin{tabular}[c]{@{}l@{}}59.0\% object recall,\\83.1\% of the randomly sampled foreground pixel pairs ordered on KITTI~\\95.87\% F1 score on ISPRS\\97\% vehicle types accuracy\\1.333 front 4.698 side-way KITTI\end{tabular}  \\ 
\hline
Lane detection                                                                      & \begin{tabular}[c]{@{}l@{}} \cite{neven2018towards}Neven, et al.(2018)\\\cite{roberts2018dataset}Roberts, et al.(2018)\\ ~ \end{tabular}        & \begin{tabular}[c]{@{}l@{}}multi-task CNN\\ SegNet \\~\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}96.4\% accruacy\\IoU Mapillary 82.9\% CityScapes 85.2\%\\KITTI 83.8\% author's dataset 95\%\end{tabular}                                                                                                   \\ 
\hline
3D reconstruction                                                                   & \cite{hadi2020semantic}Hadi, et al.(2020)                                                         & Mask R-CNN                                                                               & \begin{tabular}[c]{@{}l@{}}AP@50\% 8.862\% CityScapes 43.949\%\\IDD\cite{varma2019idd} 5.643\% WildDash\cite{zendel2018wilddash}\end{tabular}                                                                                                                                    \\
\hline
\end{tabular}
}
\caption{Some instance segmentation methods used for traffic imagery analysis. If the dataset is not indicated, it means that a proprietary dataset generated by the authors is used.}
\label{tab:instancework}
\end{table*}

\end{comment}
\begin{table*}[h]
\centering
\caption{Some instance segmentation methods used for traffic imagery analysis. If the dataset is not indicated, it means that a proprietary dataset generated by the authors is used.}
\resizebox{\textwidth}{!}{

\begin{tabular}{llll} 
\toprule
\textbf{Task }                                                                               & \textbf{[REF] authors (Year)}                                                     & \textbf{Methods}                                                                                  &\textbf{Performance}                                                                                                                                                                                                                   \\ 
\midrule
\begin{tabular}[c]{@{}l@{}}Obtain comprehensive\\ vehicle information \end{tabular} & \begin{tabular}[c]{@{}l@{}}\cite{zhang2015monocular}Zhang, et al.(2015)\\~\\ \cite{mou2018vehicle}Mou, et al.(2018)\\ \cite{zhang2020traffic}Zhang, et al.(2020)\\ \cite{huang2018measuring}Huang, et al.(2018) \end{tabular} & \begin{tabular}[c]{@{}l@{}}CNN+MRF\\ ~\\ ResFCN\\ Mask R-CNN\\ Mask R-CNN \end{tabular} & \begin{tabular}[c]{@{}l@{}}59.0\% object recall,\\83.1\% of the randomly sampled foreground pixel pairs ordered on KITTI~\\95.87\% F1 score on ISPRS\\97\% vehicle types accuracy\\1.333 front 4.698 side-way KITTI\end{tabular}  \\ 
\midrule
Lane detection                                                                      & \begin{tabular}[c]{@{}l@{}} \cite{neven2018towards}Neven, et al.(2018)\\\cite{roberts2018dataset}Roberts, et al.(2018)\\ ~ \end{tabular}        & \begin{tabular}[c]{@{}l@{}}multi-task CNN\\ SegNet \\~\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}96.4\% accruacy\\IoU Mapillary 82.9\% CityScapes 85.2\%\\KITTI 83.8\% author's dataset 95\%\end{tabular}                                                                                                   \\ 
\midrule
3D reconstruction                                                                   & \cite{hadi2020semantic}Hadi, et al.(2020)                                                         & Mask R-CNN                                                                               & \begin{tabular}[c]{@{}l@{}}AP@50\% 8.862\% CityScapes 43.949\%\\IDD\cite{varma2019idd} 5.643\% WildDash\cite{zendel2018wilddash}\end{tabular}                                                                                                                                    \\
\bottomrule
\end{tabular}
}

\label{tab:instancework}
\end{table*}





%\subsection{Person re-identification (Re-ID)}
%Person re-identification (Re-ID) aims to process video captured by multiple non-overlapping cameras that can address person detection, person tracking, but most of them focus on object person retrieval. The challenges involve different viewpoints processing, low-image resolution, strange pose, illumination changes, etc.  Some of the algorithms tried to learn feature representation. \cite{wu2016personnet,zheng2017unlabeled，zhong2017re，sun2017svdnet，ye2018robust}  

%In practical, 






%\arr{put a section for event recognition and how we can use deep learning to perform even recognition in this context. for example, cross passing a lane without turning on the signal is an event considered violation of traffic rule. Events are variants of  time-series analysis. For example, here you need to perform object detection and recognition, but then process different incidents in time domain....it can be related to human action recognition. Another example, passing a red light: with object detection we can detect the vehicle and traffic light but it a violation of rules only of passing coincides with a red traffic light, etc.. }
%$MCTA= \underbrace{\frac{2PR}{P+R}}_{F_1} \underbrace{(1-\frac{M^w}{T^w})}_{\text{within camera}} \underbrace{(1-\frac{M^h}{T^h})}_{\text{handover}}$


\subsection{Video-based Event Recognition } \label{sec:event_detect}
\fbox{Ready to review} 
\fbox{Added automated video-based road safety papers}
%Event-based video analysis provides endless possibilities to explore the interactions among objects in varied scenes during a short period. Compared with the conventional analysis approaches (extract object information then manually feed to other statistical models), this kind of methods allow the safety analysis system to evaluate the behaviours of involved vehicles directly. Generally, event recognition requires extract features first then do classification. The low-level visual features can be organized as static frame features and motion spatio-temporal features. Static frame features are the appearance characteristics that can be obtained from a single frame. These features can be learned by Scale-Invariant Feature Transform (SIFT)\cite{lowe2004distinctive}, Speeded Up Robust Features (SURF)\cite{bay2006surf}, the Local Binary Patterns (LBP)\cite{ojala2002multiresolution,tang2013combining}, and GIST (a very low-dimensional scene representation)\cite{friedman1979framing,oliva2001modeling}. In fact, motion spatio-temporal features play a more important role when event detecting,since most events strongly depend on temporal patterns. The approaches to learn these features involve Motion SIFT (MoSIFT)\cite{chen2009mosift}, spatio-temporal interest points (STIP)\cite{laptev2005space}, and Dense trajectories\cite{wang2011action,wang2013action}. The high-level visual features are often related to interpret the specific visual concepts (in traffic field, such as vehicle moving, braking, traffic light flash). Some of the early works\cite{yang2012complex,yu2012multimedia,guo2012detecting,habibian2014videostory,habibian2013recommendations,lan2014multimedia,lan2014resource,liu2013video,mazloom2013searching} tried to capture these features from keyframes with a set of low-level features, while some works\cite{sun2013active,ma2013complex} treat these features according to their time evolvement (such as using HMM model).    


%Event detection also benefit much from the deep learning methods, and frequently, the solutions deploy RNN/LSTM to preserve the temporal features and deploy CNN to extract spatial features. 


%Event detection also benefit much from the deep learning methods, especially from CNNs, since their outstanding performance on visual feature extract. Like discuss early, some deep learning approaches solve the problem in the perspective of static frame. \cite{ye2015eventnet} proposed a pretrained CNN model under event-level, while \cite{mettes2016imagenet} deployed a framework pretraind on ImageNet, which is under concept-level. Moreover, \cite{gan2015devnet,wang2015video} extract the frame-based features according to the keyframes and contextual features, respectively. Fusion-based methods can better understand video events in different scenarios. \cite{7823615} proposed fusion classifier that can learn the weights for each SVM feature classier, and \cite{7364255} proposed a fusion structure fed with the features of semantic cues, object, and scene. In contrast to static frame-based approaches, motion-based methods can obtain richer spatio-temporal information. The general solution is to deploy RNN/LSTM\cite{feng2016deep,jiang2016automatic,feng2020spatio,wang2018abnormal,yu2016robust,jiang2016automatic,liu2019lstm} to preserve the temporal features and deploy CNN to extract spatial features. 
%\cite{,yu2016robust,jiang2016automatic,liu2019lstm}




Video-based event recognition extends the role of DL methods from object detection and identification paradigms into a more intricate problem of understanding events. It provides endless possibilities to explore the interactions among objects in an interactive environment rather than focusing on disjoint object-based tasks. Indeed, without event detection and analysis, the majority of video information remains unexploited and underutilized. Note that many safety metrics relate to the interactions of vehicles with one another and with the environment. For instance, traffic sign interpretation can be recast as an image-based object classification problem, while more intricate violations of traffic safety such as unsafe lane changing behavior without signaling require modeling interactions between vehicles and their surrounding environments. 
Such challenging problems are still in their infancy stages and apparently require heavy investment by the research community. In essence, the event recognition problem is also related to another well-investigated problem of video-based human action recognition, and similar tools and algorithms can be adopted here.

An alternative method of event analysis is using conventional analysis approaches by extracting object-based information and manually feeding them into statistical and reasoning models such as Hidden Markov Models (HMM) for safety analysis. However, with the recent advances in developing powerful DL methods, they enable a more automated and direct way of evaluating the behaviors of involved vehicles. The most naive way of event recognition can be realized by extracting static features from video frames using methods like SIFT \cite{lowe2004distinctive}, SURF \cite{bay2006surf}, the Local Binary Patterns (LBP) \cite{ojala2002multiresolution,tang2013combining}, HOG detector \cite{dalal2005histograms}, Binary Robust Invariant Scalable Keypoints (BRISK) \cite{leutenegger2011brisk}, Features from Accelerated Segment Test (FAST) \cite{rosten2006machine,viswanathan2009features} and GIST (a very low-dimensional scene representation) \cite{friedman1979framing,oliva2001modeling}, and then performing object detection followed by a time-series analysis for even recognition. 
Some other methods combine the feature extraction and time-series analysis stage into directly extracting temporal features using methods like motion spatio-temporal features (Motion SIFT (MoSIFT) \cite{chen2009mosift}, Spatio-Temporal Interest Points (STIP) \cite{laptev2005space}, and Dense trajectories \cite{wang2011action,wang2013action}), then perform the classification task. 

More contemporary event detection algorithms benefit from DL methods to automate this process, and a dominant method is directly applying a 3D convolutional network to process non-anomalous frames \cite{hasan2016learning}. Another approach is deploying CNN to extract spatial features and then performing sequential analysis using methods such as  RNN/LSTM \cite{feng2016deep,jiang2016automatic,wang2018abnormal,chong2017abnormal,medel2016anomaly,liu2019lstm,feng2020spatio} to preserve the temporal features. 


Most of these methods use supervised learning methods to detect a set of predefined events. Therefore, developing generic methods for understanding safety risks from driving profiles and tackling unseen types of safety violations has a long way ahead.

Event recognition is of particular importance for traffic safety analysis since it can be used for detecting abnormal events and traffic violations and their associations with crash rates \cite{giannakeris2018speed}, car behavior analysis \cite{zhou2016spatial,franklin2020traffic}, and pedestrians' crossing identification \cite{xu2015learning,medel2016anomaly,xu2017detecting}. 
Recently, some works\cite{anno2019gan,ravanbakhsh2019training,nguyen2020anomaly} try to predict anomaly actions using Generative Adversarial Networks (GAN). The core idea is predicting the future video frames for a normal user with rational behavior from the history of normal sequences to identify severe abnormalities by comparing the observed video frame against the anticipated one.

For vehicle-level analysis, when the goal is detecting plain and simple events, conventional methods achieve a reasonable performance. For instance, \cite{akoz2014traffic} uses HMM to detect traffic abnormality, and \cite{kaviani2015automatic} deployed a topic model to recognize crashes from surveillance videos. However, using DL methods can be used to analyze more complex events and achieve higher performance records. 
Some generic platforms like Rekall \cite{fu2019rekall}, provide a query-based approach to translate the challenging task of event recognition into a sequence of object detection and classification problems. 




We summarize important DL-based event recognition methods in Table \ref{tab:abnormaldetect}, and present some popular datasets for event recognition tasks in Table \ref{tab:trafficdataset}. One observation is that unsupervised, semi-supervised, and self-supervised models are becoming more prevalent in recent works \cite{giannakeris2018speed,yao2019unsupervised,nguyen2020anomaly} to mitigate the costly and tedious job of video annotation and simplifies volume video processing. 


%\xc{Besides these pure data-driven methods that often focus on detection, we also note there are some frameworks of automated video-based road safety analysis that use ML/DL to extract the information of the road users from videos and then perform the analysis by the domain knowledge from traffic safety (such as surrogate safety measures). For example, the authors in \cite{st2015large} collected large-scale data in about 40 roundabout weaving zones. The authors track the vehicle by KLT. Then after processing data, they extract the surrogate measures of each vehicle, such as speed, individual interaction measurements, and TTC, and plan to perform some correlation analysis with complementary data (such as design geometry and environment attributes). A summary of the recent frameworks is presented in Table \ref{tab:automated_video}. We note that most of these frameworks use the conventional tracking algorithms, which is consistent with the discussion in Section \ref{sec:tracking} that these methods still have reasonable performance. The suggestion would be some recent tracking algorithms that can already provide fast and accurate detection and tracking, such as the YOLOv5 and DeepSort \cite{wojke2017simple} combo. }
\ar{These pure data-driven methods often focus on detection problems. Alternatively, other automated video-based road safety analysis frameworks exist that use ML/DL methods to extract information about the road users from RSU videos and perform safety analysis using domain knowledge. An important class of such studies is extracting surrogate safety measures. For example, the authors of \cite{st2015large} collected large-scale data in about 40 roundabout weaving zones. They track the vehicles using KLT-based \xc{Yes. Kanade–Lucas–Tomasi (KLT)-based tracker \cite{saunier2006feature}}\arr{spell out if it is the first occurrence. Do you mean Kanade–Lucas–Tomasi (KLT) feature-based dense tracking} method, then extract a set of surrogate measures, such as speed, individual interaction measurements, and TTC, for each vehicle. Performing correlation analysis between the surrogate measures and complementary data (such as design geometry and environment attributes) reveals insightful relations about traffic safety. A summary of such frameworks is presented in Table \ref{tab:automated_video}. We note that most of these frameworks use conventional tracking algorithms, which yield reasonable performance, as discussed in Section \ref{sec:tracking}. \arr{Do you mean this:} However, more advanced joint detection and tracking algorithms can be developed.\xc{here I want to mention some DL method as detector for the hybrid method (discussed at the end of Section \ref{sec:tracking}), which uses DL detector for fast and accurate
object detection, followed by a second estimator based on conventional methods } For instance, one may combine YOLOv5 and DeepSort for precise vehicle tracking \cite{wojke2017simple}. \xc{\cite{wojke2017simple} this citation is for DeepSort}} 







\begin{comment}


\begin{table*}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|} 
\hline\rowcolor{gray}
\textbf{Paper: [Ref] Authors (year)} & \textbf{Methods}                                                                  & \textbf{Performance}                                         \\ 
\hline
\cite{nguyen2020anomaly}Nguyen, et al.(2020)     & GAN                                                                      & F1 score 0.9412 AI City Challenge 2019              \\ 
\hline
\cite{yao2019unsupervised}Yao, et al.(2019)     & \begin{tabular}[c]{@{}l@{}}Auto Encoder-Decoder\\ with GRU \end{tabular} & 60.1\% AUC on A3D Dataset                             \\ 
\hline
\cite{tian2019automatic}Tian, et al.(2019)     & YOLO-CA                                                                  & 90.02\% AP CAD-CVIS                                   \\ 
\hline
\cite{kim2020pre}Kim, et al.(2020)     & 3D conv                                                                  & 82\%                                               \\ 
\hline
\cite{ijjina2019computer}Ijjina, et al.(2019)     & 3D conv                                                                  & 71\%                                                  \\ 
\hline
\cite{shah2018cadp}Shah, et al.(2018)      & \begin{tabular}[c]{@{}l@{}}DSA-RNN\cite{chan2016anticipating}\\ Faster R-CNN \end{tabular}          & 47.25\% on CADP                                       \\ 
\hline
\cite{srinivasan2020novel}Srinivasan, et al.(2020)      & Detection Transformer\cite{carion2020end}                                                    & 78.2\% on CADP                                        \\ 
\hline
\cite{suzuki2018anticipating}Suzuki, et al.(2018)     & QRNN+DeCAF\cite{donahue2014decaf}                                                                & 99.1\% mAP                                            \\ 
\hline
\cite{giannakeris2018speed}Giannakeris, et al.(2018)     & Faster RCNN                                                              & F1-score 0.33 RMSE 227 on NVIDIA CITY Track 2       \\ 
\hline
\cite{arceda2018fast}Arceda, et al.(2018)    & YOLO+ViF\cite{hassner2012violent}+SVM                                                             & 89\%                                                  \\ 
\hline
\cite{biradar2019challenges}Biradar, et al.(2019)   & YOLOv2+ CNN                                                              & F1-score 0.3838 RMSE 93.61 on NVDIA CITY Track 3    \\ 
\hline
\cite{xu2018dual}Xu, et al.(2018)    & Mask-RCNN+ ResCNN                                                        & F1-score 0.8649 RMSE 3.6152 on NVIDIA CITY Track 2  \\ 
\hline
\cite{doshi2020fast}Doshi, et al.(2020)    & YOLO+KNN+K-means                                                         & F1-score 0.5926 RMSE 8.2386 on NVIDIA CITY track 4  \\ 
\hline
\cite{zhou2016spatial}Zhou, et al.(2016)    & 3D Conv                                                                   & 95.2\% on U-turn dataset                              \\ 
\hline
\cite{franklin2020traffic}Franklin, et al.(2020)    & YOLOv3                                                                   & 100\% and 95.34\% for input video 1 and video 2         \\
\hline
\end{tabular}
}

\caption{Some recent DL works for video-based traffic abnormal event detection. Unless otherwise specified, the non-indicated numbers is the accuracy.}
\label{tab:abnormaldetect}
\end{table*}
\end{comment}

%. Semi-supervised learning primarily uses unlabeled data with some supervision with a small amount of labeled data for specifying example classes known apriori
\begin{table*}[]
\centering
\caption{Some recent DL works for video-based traffic abnormal event detection. Unless otherwise specified, the non-indicated numbers is the accuracy.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lll} 
\toprule
\textbf{Paper: [Ref] Authors (year)} & \textbf{Methods}                                                                  & \textbf{Performance}                                         \\ 
\midrule
\cite{nguyen2020anomaly}Nguyen, et al.(2020)     & GAN                                                                      & F1 score 0.9412 AI City Challenge 2019              \\ 
\midrule
\cite{yao2019unsupervised}Yao, et al.(2019)     & \begin{tabular}[c]{@{}l@{}}Auto Encoder-Decoder\\ with GRU \end{tabular} & 60.1\% AUC on A3D Dataset                             \\ 
\midrule
\cite{tian2019automatic}Tian, et al.(2019)     & YOLO-CA                                                                  & 90.02\% AP CAD-CVIS                                   \\ 
\midrule
\cite{kim2020pre}Kim, et al.(2020)     & 3D conv                                                                  & 82\%                                               \\ 
\midrule
\cite{ijjina2019computer}Ijjina, et al.(2019)     & 3D conv                                                                  & 71\%                                                  \\ 
\midrule
\cite{shah2018cadp}Shah, et al.(2018)      & \begin{tabular}[c]{@{}l@{}}DSA-RNN\cite{chan2016anticipating}\\ Faster R-CNN \end{tabular}          & 47.25\% on CADP                                       \\ 
\midrule
\cite{srinivasan2020novel}Srinivasan, et al.(2020)      & Detection Transformer\cite{carion2020end}                                                    & 78.2\% on CADP                                        \\ 
\midrule
\cite{suzuki2018anticipating}Suzuki, et al.(2018)     & QRNN+DeCAF\cite{donahue2014decaf}                                                                & 99.1\% mAP                                            \\ 
\midrule
\cite{giannakeris2018speed}Giannakeris, et al.(2018)     & Faster RCNN                                                              & F1-score 0.33 RMSE 227 on NVIDIA CITY Track 2       \\ 
\midrule
\cite{arceda2018fast}Arceda, et al.(2018)    & YOLO+ViF\cite{hassner2012violent}+SVM                                                             & 89\%                                                  \\ 
\midrule
\cite{biradar2019challenges}Biradar, et al.(2019)   & YOLOv2+ CNN                                                              & F1-score 0.3838 RMSE 93.61 on NVDIA CITY Track 3    \\ 
\midrule
\cite{xu2018dual}Xu, et al.(2018)    & Mask-RCNN+ ResCNN                                                        & F1-score 0.8649 RMSE 3.6152 on NVIDIA CITY Track 2  \\ 
\midrule
\cite{doshi2020fast}Doshi, et al.(2020)    & YOLO+KNN+K-means                                                         & F1-score 0.5926 RMSE 8.2386 on NVIDIA CITY track 4  \\ 
\midrule
\cite{zhou2016spatial}Zhou, et al.(2016)    & 3D Conv                                                                   & 95.2\% on U-turn dataset                              \\ 
\midrule
\cite{franklin2020traffic}Franklin, et al.(2020)    & YOLOv3                                                                   & 100\% and 95.34\% for input video 1 and video 2         \\
\bottomrule
\end{tabular}
}


\label{tab:abnormaldetect}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{\ar{Automated video-based road safety analysis frameworks.}}
\label{tab:automated_video}
\resizebox{\textwidth}{!}{%
\blr
\begin{tabular}{llll}\toprule
\textbf{[REF]   authors (Year)}                                 & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Video Processing\\      Method\end{tabular}}}                                                               & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Analysis \\      Method\end{tabular}}}                               & \textbf{Description}                                                                                               \\ \midrule
\cite{st2015large} St-Aubin et al. (2015)                      & KLT                                                                                                                                                            &     -                                                                                                                       & Dataset Collection                                                                                                 \\ \midrule
\cite{zangenehpour2016signalized}   Zangenehpour et al. (2016) & \begin{tabular}[c]{@{}l@{}}KLT for tracking;\\      Bayesian classification for seg.\cite{zangenehpour2015automated};\end{tabular}                              & \begin{tabular}[c]{@{}l@{}}Regression Analysis;\\      Rank correlation analysis;\end{tabular}                              & Cyclist and motor-vehicle interactions                                                                             \\ \midrule
\cite{lu2016video} Lu et al. (2016)                            & KLT                                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}Sensitivity analysis;\\      Golden section search\end{tabular}                                 & Calibrate car-following parameters in VISSIM simulation                                                           \\ \midrule
\cite{mohamed2018impact} Mohamed et al.   (2018)               & \begin{tabular}[c]{@{}l@{}}KLT;\\      Kinematic method\\       Motion pattern matching (MPM) by   \\      the longest common sub-sequence (LCSS)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Distribution/frequency  analysis;\\      Clustering\end{tabular}                                & \begin{tabular}[c]{@{}l@{}}Study on  impact of motion prediction methods\\       on safety indicators\end{tabular} \\ \midrule
\cite{xu2018automated} Xu et al. (2018)                        & \begin{tabular}[c]{@{}l@{}}YOLOv2;\\      NMS\end{tabular}                                                                                                     &    -                                                                                                                        & Database building for pedestrian   analysis                                                                         \\ \midrule
\cite{battiato2018board} Battiato et al.   (2018)              & \begin{tabular}[c]{@{}l@{}}Kernel-based object tracking   \cite{comaniciu2003kernel};\\      HOG\end{tabular}                                                  & Bayesian classification                                                                                                     & Risk analysis from on-board video data                                                                             \\ \midrule
\cite{xie2019mining} Xie et al. (2019)                         & \begin{tabular}[c]{@{}l@{}}KLT;\\      rPCA;\\      Dirichlet process Gaussian mixture model (DPGMM)\end{tabular}                                              & HMM                                                                                                                        & model the rear-end conflicts                                                                                       \\ \midrule
\cite{chen2020conflict} Chen et al.   (2020)                   & \begin{tabular}[c]{@{}l@{}}HOG;\\      SVM;\\      Kalman Filter;\\      Adaptive Gaussian Mixture model\end{tabular}                                          & Distribution analysis                                                                                                      & \begin{tabular}[c]{@{}l@{}}Safety space analysis;\\       Data collected by UAV\end{tabular}                       \\ \midrule
\cite{yang2021proactive} Yang et al.   (2021)                  & \begin{tabular}[c]{@{}l@{}}KLT;\\      Kalman Filter\end{tabular}                                                                                              & Functional Data Analysis                                                                                                   & \begin{tabular}[c]{@{}l@{}}Anomalies detection;\\       Data collected by UAV\end{tabular}                         \\ \midrule
\cite{noh2022analyzing} Noh et al. (2022)                      & \begin{tabular}[c]{@{}l@{}}Mask R-CNN;\\      DeepSort\end{tabular}                                                                                            & LSTM                                                                                                                       & Pedestrian-vehicle collision risk   prediction                                                                      \\ \midrule
\cite{chen2022network} Chen et al. (2022)                      & \begin{tabular}[c]{@{}l@{}}YOLOv5;\\      DeepSort\end{tabular}                                                                                                & \begin{tabular}[c]{@{}l@{}}Regression Analysis;\\      Rank correlation analysis;\\      Coalition game theory\end{tabular} & Traffic risk analysis   \\ \bottomrule                                                                                          
\end{tabular}%
}
\end{table*}





%ltsm: feng2016deep
 
%DATASETsss:
%-Dashcam Accident Dataset (DAD)
%CADP\cite{shah2018cadp}
% NVIDIA AI CITY CHALLENGE\cite{ai_city_challenge}
%{Video recognition architectures are favorably designed by extending image classification networks with a temporal dimension. Some work intend to directly borrow the 2D structure in form of 3D\cite{taylor2010convolutional,tran2015learning,xie2017rethinking,carreira2017quo,peng2016multi,hara2018can,qiu2017learning}. Some works\cite{donahue2015long,li2018recurrent,li2018videolstm,sun2017lattice} fine-tune the 2D CNN structure with RNN/LSTM to preserve the temporal features. Some works\cite{carreira2017quo,feichtenhofer2016convolutional,simonyan2014two} tend to process the framework by deploying optical flow to capture the motion information. SlowFast ....}




\subsection{Sensor Information Processing} \label{sec:sensor}
It is notable that there are several studies and datasets devoted to sensor information analysis. Different types of commonly used sensors were provided previously in section \ref{sec:hardware}. Of particular and increasing interest is the point cloud mapping collected from LiDARs, not just because they offer more accurate distance measurement, but also they are considered as separate and independent sensing of the environment to that of videos to ensure accurate perception thus road safety. 3D point cloud mapping from LiDAR is different from grid-based 2D images, thus different treatment strategies are pursued. LiDAR point cloud semantic segmentation works use deep neural networks, initially treating point cloud as construct graph \cite{simonovsky2017dynamic}, followed by the development of multi-layer perceptrons to learn from raw cloud data directly \cite{qi2017pointnet,qi2017pointnet++}. More recently, the spherical projection has been employed to map LiDAR sequential scans to depth images, and improved segmentation \cite{wu2018squeezeseg,wu2019squeezesegv2,milioto2019rangenet++,xiang2019novel}. Since the focus of this paper is video-processing for traffic safety analysis, we refer the interested readers to \cite{nellore2016survey,bernas2018survey,won2020intelligent,ahangar2021survey}.
%\xc{I think this comment should be moved to section.\ref{sec:Semantic Seg}}.


\subsection{Network-level Analysis} \label{sec:network}


Traffic flow problems can be formulated as a network of mobile nodes, and studies on individual crash analysis can be extended to the more complex setup of network-level analysis. 

There exist a few research paradigms that consider network-level analysis. One bold example is the transportation network design and related family of problems. 
Transportation network design belongs to the category of operations research and can be divided into the Road Network Design Problem (RNDP) and Service Network Design Problem (SNDP) according to their features and functions\cite{farahani2013review}. The works \cite{yang1998models,szeto2015sustainable,hosseininasab2015integration} of RNDP aim to optimize the performance of urban networks according to some criteria such as topology, capacities, and flow accessibility. The works \cite{fan2006optimal,yan2013robust,cancela2015mathematical,liu2016capacitated,di2018transportation} of SNDP aim to address the planning of operations for freight transportation carriers, such as station locations, route planning, and operation frequency. 

Traffic prediction studies often employ statistical techniques (such as Kalman filtering \cite{guo2014adaptive}, hidden Markov model \cite{qi2014hidden}, Bayesian interference \cite{wang2014new}) and DL  (such as LSTSM, CNN) methods \cite{ma2015long,cui2018deep,du2018hybrid,wang2019traffic} to infer the network state and produce optimal strategies for different conditions. 

Network-level analysis can be used for traffic safety analysis as well. Some key objectives would include finding correlations between traffic flow, safety metrics geo-maps, and crash rates. For example, one may expect a direct relation between the traffic composition (density and variety of vehicles) and the number of crashes at different parts of highways. One may also expect relations between the traffic flow and crash rates of nearby intersections or segments. Network-level analysis can shed light on these highly unexplored research areas.

There exist four general approaches for network-level analysis \cite{mannering2020big} including traditional statistical models (e.g., \cite{part2010highway}), endogeneity/heterogeneity models (e.g., \cite{bhat2014count,mannering2016unobserved}), data-driven methods \cite{arbabzadeh2017data,cheng2018big}, and causal inference models. Furthermore, we note that some models\cite{lord2010extension,aguero2008analysis} exploit previously collected crash data with road information (such as average daily traffic (ADT), lane width, speed limited, shoulder width) to estimate crash frequencies at intersections or segments. Some models \cite{karlaftis2002effects,othman2009identifying} explore risk probabilities by processing geometric features. Recently, new models\cite{yu2013multi,ahmed2013data,xu2014using,yu2020convolutional,sun2015dynamic,sameen2017severity} 
take advantage of advanced sensors techniques and high-performance computation frameworks to infer real-time crash risks and take proactive strategies. Safety analysis frameworks can perform integrative analysis by incorporating different static and dynamic data modalities (i.e., imagery and sensor inputs) from different points of view to comprehend the network status and derive realistic distributions for safety factors. An immediate benefit of such networks would be assessing the contribution of different factors on safety distributions and providing advisory to improve roadways and infrastructure design as well as developing safety enforcement and public education campaigns. 

 \begin{figure*}[h]
\begin{center}
\centerline{\includegraphics[width=0.8\textwidth]{figures/futuremodel.png}}
\caption{VANETs framework.}%. Source from\cite{cheng2018big}. } 
\label{fig:VANETs}
\end{center}
\end{figure*}

%\arr{Lets go with the following short statements and avoid touching networking and data aggregation details. }

A key challenge is developing strategies and scheduling policies for data aggregation to provide required modalities for network-level safety analysis at the minimum cost possible. Also, data aggregation is constrained by the utilized networking infrastructure and communication protocols between the vehicles and roadside infrastructure. Study of such networks are out of the scope of this work, and we refer the interested users to \cite{al2017internet,allal2012geocast,boussoufa2018geographic,dhankhar2014vanets,allal2013geocast,cheng2018big,martinez2011survey,luo2004survey,al2017internet} 




Recently, the ideas of using data augmentation and physics-informed neural networks (PINN) are proposed to mimic the dynamics of complex systems while mitigating the need for manual annotation of massive datasets. We believe that the power of PINN and data augmentation is not yet fully utilized in this context. There is a great potential to develop surrogate models for traffic flow and risk analysis. The authors also believe that elegantly designed graph neural networks can play an essential role in modeling network-level events and trends.  

%\textbf{Data Aggregation} : Data aggregation approaches aim to improvement of energy efficiency and eliminate the redundancy caused by the high density of the data sensed by the nodes in the sensor networks. A large city traffic monitoring camera networks, petabytes data was generated per day. The data collected by adjacent cameras usually display high spatial and temporal correlation and similarity. Efficient and stable data aggregation strategies are supposed to be developed to reduce the data overhead, energy usage, and maintenance cost. 















\begin{comment}
\textbf{Communication [keep the title, but most likely we would exclude, or we Can refer to some recent surveys regardoing this aspect]:} 

The early surveys reviewed inter-vehicle communication (IVC) involving protocols built upon the MAC layer\cite{luo2004survey} to transport layer, security analysis\cite{sichitiu2008inter}, IVC-based services\cite{willke2009survey}. The recent surveys paid more attention to vehicular ad hoc networks (VANETs) (shown in Fig.\ref{fig:VANETs}). \cite{martinez2011survey} compared VANETs simulators according to their different factors. \cite{zhang2011survey,al2012survey,manvi2017survey,sakiz2017survey} discussed security problems in the perspective of trust models, security attack and defence, authentication schemes, and attack detection, respectively. \cite{jarupan2011survey} contrasted cross-layer design approaches. \cite{allal2012geocast,boussoufa2018geographic,dhankhar2014vanets,allal2013geocast} explored the routing protocols for VANETs. \cite{cheng2018big} reviewed the big-data-driven technologies.


Here, we still want to mention some popular IoT communication protocols that have the potential to allow the information exchange among vehicles, devices, infrastructure or internet. \cite{al2017internet} compared 6LoWPAN, ZigBee, BlueTooth, RFID, NFC, SigFox, Cellular, and Z-Wave, which is shown in Table.\ref{tab: protocol}.
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[!h]

\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
Protocols & 6LoWPAN      & ZigBee       & BlueTooth LE & RFID   & NFC          & SigFox       & Cellular                                                  & Z-wave       \\ \hline
Security  & AES  & AES  & AES & RC4    & AES  & AES& RC4                                                       & AES \\ \hline
Power     & Low          & Low          & Low          & Middle & Middle       & Middle       & High                                                      & Low          \\ \hline
Speed     & Low          & Low          & Low          & Middle & Low          & Low          & \begin{tabular}[c]{@{}l@{}}Middle\\ to High*\end{tabular} & Low          \\ \hline
Range     & Low          & Low          & Low          & Low    & Low          & Middle       & Middle                                                    & Low          \\ \hline
\end{tabular}%
}
\caption{Comparison between communication protocols.AES are safer but slower than RC4. *High speed because of the recent development of 5G.}
\label{tab: protocol}
\end{table*}
\end{comment}




%https://openaccess.thecvf.com/content/CVPR2021/papers/Feichtenhofer_A_Large-Scale_Study_on_Unsupervised_Spatiotemporal_Representation_Learning_CVPR_2021_paper.pdf

%https://arxiv.org/pdf/2205.09113.pdf

%https://openaccess.thecvf.com/content_ICCVW_2019/html/HVU/Han_Video_Representation_Learning_by_Dense_Predictive_Coding_ICCVW_2019_paper.html

%https://openaccess.thecvf.com/content_cvpr_2017/html/Fernando_Self-Supervised_Video_Representation_CVPR_2017_paper.html




==> draft.tex <==
vehicle detection:
pure CNN: 
\cite{sang2018improved}:YOLOv2,vehicle detection
\cite{espinosa2017vehicle} Faster R-cnn,vehicle detection
\cite{wang2019comparative} Faster R-cnn,R-FCN,SSD,YOLOv3,RetinaNet
\cite{kim2019multi} YOLOv3, vehicle detection
\cite{wang2017evolving} Faster RCNN, vehicle detection
\cite{soin2017moving} RCNN, vehicle detection
\cite{zhang2019vehicle} SSD, vehicle detection
\cite{zhang2017application} Faster R-cnn, vehicle detection, traffic monitoring
\cite{peppa2018urban} Faster RCNN
ssd: chen2020inception cao2020front
plate detection:
pure CNN:\cite{kim2017deep}\cite{selmi2017deep}\cite{masood2017license}
\cite{hsu2017robust} YOLO/YOLOv2
\cite{kessentini2019two} YOLOv2
\cite{lee2016real} Faster RCNN
\cite{khazaee2020real} YOLOv3
\cite{xie2018new} YOLO
\cite{chen2019automatic} YOLO
ssd
ren2020implementation,hu2020mobilenet,danilenko2020license

traffic sign:
pure CNN: \cite{zhu2016traffic,wu2013traffic,shustanov2017cnn}
\cite{qian2016road} Fast R-cnn
\cite{shao2019improved} Faster RCNN
\cite{zhang2020cascaded} r-cnn
\cite{zuo2017traffic} Faster rcnn
\cite{zhang2017real} YOLOv2 \cite{Tai_2020} v3
\cite{wu2019traffic} Faster rcnn
\cite{peng2016traffic} Faster rcnn

gao2019traffic ssd
you2020traffic SSD


zhang2019vehicle e UA-DETRAC s 77.94 mAP  UA-DETRAC
,chen2020inception 86.2 KITTI 87.4 UA-DETRAC
,cao2020front 92.18 kitti

6778050,  99.7\%
8019461:repeated 

espinosa2017vehicle: 0.7 author dataset
,wang2019comparative
,wang2017evolving,  84.43     DETRAC dataset others
soin2017moving, 100 author dataset
zhang2017application, 96.5 uav 
,peppa2018urban, 97 R-CNN 98.2 SSD  author dataset

lee2016real: 99.94

 \cite{hsu2017robust,kessentini2019two,khazaee2020real,xie2018new,chen2019automatic}
hsu2017robust:
kessentini2019two: a full LP recognition rate of 97.67\% in the GAP-LP dataset, and of 91.46\% in Radar dataset
khazaee2020real:0.979 0.972 on dateset gnerated by the authors 
xie2018new: 98.32 UCSD PKU
chen2019automatic:98.22 AOLP



ren2020implementation,hu2020mobilenet,danilenko2020license
ren2020implementation： 0.92
hu2020mobilenet 90.12 
danilenko2020license 94+ 


kim2017deep, 98.39\% and a recall of 96.83\% on Caltech
selmi2017deep 94.8 Caltech
,masood2017license 99.09\%  US 99.64\% EU

qian2016road  85.58\%.
,shao2019improved 69.56\% gtsdb+ctsd
,zhang2020cascaded The accuracy and recall rate of our method are 98.7\% and 90.5\% in GTSDB, 99.7\% and 83.62\% in CCTSDB and 98.9\% and 85.6\% in Lisa dataset respectively.
,zuo2017traffic 0.3449 traffic sign detection competition in 2016 by CCF
and UISEE company.
,wu2019traffic mAP  91.75\%  GTSDB
,peng2016traffic mAP ~90 GTSDB

zhang2017real 96.69 @0.017   CCTSDB and GTSDB
,Tai_2020  99.1 mAP  


gao2019traffic, The precision and recall on the test data set are 91.0\%, and 88.06\%  GTSDB
you2020traffic 0.75 0.82recall  TT100K traffic sign datase

zhu2016traffic  a recall 0.91 and accuracy 0.88 TT100K
,wu2013traffic,  AUC of 99.73\% in the category “danger”, and an AUC of 97.62\% in the category “mandatory  GTSDB
shustanov2017cnn 99.94 GTSRB


\subsection{Speed Estimation}
Speed Estimation aims to estimate the movement speed of an object by exploiting the interaction between the object and the environment in a video clip. The speed of the vehicle is one of most significant factor of driving safety. If the video is in the perspective of external observers, the speed of vehicles can be estimated based on visual tracker by:
\begin{align}
    V_t = \sqrt{\delta x^2_t+\delta y^2_t}
\end{align}
where,$x_t$ and $y_t$ are the instantaneous displacement of two dimensions. Consider the minimum time interval (depends on the video source quality and algorithm speed) is existed between two tracking, $\delta x_t$ and $\delta y_t$ can be written as:
\begin{align}
    \delta x_t& = x_t-x_{t-\delta t}\\
    \delta y_t& = y_t-y_{t-\delta t}\\
\end{align}
where, $\delta t$ is the minimum measurable time interval of a tracker.
If want to estimate the speed based on the drivers' view, the question would be relatively difficult. The solutions involve employ Binocular camera to collect data and deploy SLAM technique.



Accuracy  $\frac{Correct predictions}{Total predictions}$
Recall  $\frac{True Positive}{True Positive+False Negative}$
Precision $\frac{True positive}{True positive+False Positive}$
F1 score $2\times\frac{Precision\times Recall}{Precision+ Recall}$
**(Area Under ROC Curve) $AUC=\frac{\sum_{i\in Positive}rank_i-\frac{M(1+M)}{2}}{MN}$
sort the score (low to high) The rank of highest score is $n$
Pixel Accuracy (PA) $\frac{TP+TN}{TP+TN+FP+FN}$


Disparity accuracy 
stixel-wise percentage accuracy .similar to PA

Normalized error (mean)\cite{huang2018measuring} $normalized error=\frac{|d-d_{gt}|}{d_{gt}}$.  $d$ is the calculated distance and $d_{gt}$ is the ground truth of distance.


Average Precision (AP)  $AP=\int_0^1 P(R)dR$ P-R CURVE (for one class)
mean Average Precision (mAP) $mean(AP_i)$
Intersection over Union (IoU) $\frac{B_p\cap B_{gt}}{B_p\cup B_{gt}}$
$B_{gt}$: ground truth bounding box
$B_{p}$: predicted bounding box






2~\cite{xu2015learning}, unsupervised representation learning, trained SVM
119~\cite{medel2016anomaly}, self-supervised 
%216
205~\cite{xu2017detecting}, unsupervised representation learning
108~\cite{liu2018future}, supervised adversarial learning 

Accident detection: %211 \cite{} : 

gan-based: nguyen2020anomaly  F1 score 0.9412   AI City Challenge 2019 semi-supervised

yao2019unsupervised  60.1 AUC  A3D Dataset 

tian2019automatic 90.02 average precision (AP) CAD-CVIS
%rajesh2020deep successfully 
kim2020pre 0.82 3D conv GTA 

ijjina2019computer Detection Ratio 71 superivsed Youtube+GTA
 shah2018cadp    47.25 CADP
  srinivasan2020novel   78.2 CADP\cite{shah2018cadp}
suzuki2018anticipating 99.1 mean average precision (mAP)


52~\cite{giannakeris2018speed}, unsupervised clustering  NVDIA CITY. nF1-score of 0.33 and our detection time RMSE was 227 (also for spped evaluate)

arceda2018fast 89 

biradar2019challenges achieved 0.3838 F1-score and 93.61 RMSE respectively  Track 3  NVIDIA AI city challenge

xu2018dual  0.8649 3.6152 Track 2 NVIDIA AI CITY CHALLENGE
doshi2020fast 0.5926 8.2386   Track 4 NVIDIA AI CITY CHALLENGE UNSPER

car behaviour 

220~\cite{zhou2016spatial}, supervise 95.2 U-turn dataset\cite{benezeth2009abnormal}
franklin2020traffic  100 and 95.34 input video 1 video 2

traffic incident




%pedestrians 
%34
%2~\cite{xu2015learning}, unsupervised representation learning, trained SVM
%119~\cite{medel2016anomaly}, self-supervised 
%216
%205~\cite{xu2017detecting}, unsupervised representation learning
%108~\cite{liu2018future}, supervised adversarial learning 

12/11 9:33pm
metrif
IDF1



-multiple object tracking accuracy MOTA, $MOTA=1-\frac{FN+FP+\Phi}{T}$,$\Phi$ denotes the number of fragmentations 

-Identification F1-Score $IDF1=\frac{2IDTP}{2IDTP+IDFP+IDFN}$

Multi-camera Tracking Accuracy
$MCTA= \underbrace{\frac{2PR}{P+R}}_{F_1} \underbrace{(1-\frac{M^w}{T^w})}_{\text{within camera}} \underbrace{(1-\frac{M^h}{T^h})}_{\text{handover}}$
$M^w$: within-camera identity mismatches 
$T^w$:  true within-camera detections
$M^h$:  handover mismatches
$T^h$:  true handover detections

dinh2017development: Kalman filter, GMM
ngel2016low: the Approximated Median Filter
 liu2011multi:a Multi-Modal Particle Filter(MMPF)
jazayeri2011vehicle HMM
xia2013automatic   CAMShift
kaur2016vehicle kalman flter
o2010rear kalman flter
   graph-based

teoh2012reliability Kalman-filter

khalkhali2020vehicle Kalman-filter

luvizon2016video  SIFT+KLT speed

mei2011robust sparse representation

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Works               & Performance                  & Methods                                 \\ \hline
qiu2018kestrel      & 75.9 Recall 88.6 Accuracy    & YOLO+KLT                                \\ \hline
lopez2019boosting &
  \begin{tabular}[c]{@{}l@{}}0.305AP subset:M-30 0.662AP subset:M-30-HD \\ 0.381AP subset:Urban1 of  GRAM-RTM\end{tabular} &
  Faster R-CNN \\ \hline
xu2017car           & 98.43                        & Faster R-CNN                            \\ \hline
scheidegger2018mono & 80.04 MOTA on KITTI          & CNN+PMBM filter\cite{garcia2018poisson} \\ \hline
zou2019multi &
  \begin{tabular}[c]{@{}l@{}}75.29MOTA campus \\ 76.06MOTAurban \\ 78.14MOTA highway \\ on KITTI\end{tabular} &
  Siamese network+SPP+MDP \\ \hline
li2019spatio        & 83.2IDF1 nivida AI city      & FPN+tracking loss                       \\ \hline
nikodem2020multi &
  \begin{tabular}[c]{@{}l@{}}single-camera tracking accuracy 97+\\ multi-camera tracking accuracy 91+\end{tabular} &
  hourglass \\ \hline
zhao2018autonomous  & Shown in the form of figures & SSD+dual Kalman filters                 \\ \hline
wang2019orientation & 81.3                         & YOLOv3+SIFT                             \\ \hline
usmankhujaev2020real &
  \begin{tabular}[c]{@{}l@{}}100 Daytime \\ 89.83 Daytime(flipped) \\ 86.11 Nighttime(flipped)\end{tabular} &
  yoloV3+kalman filter \\ \hline
kwan2018compressiv  & For compressive measurements & ResNet                                  \\ \hline
fernandez2019real &
  86.96 MOTA on MOT 15\cite{leal2015motchallenge} &
  CNN detector+DCF+Kalman filter \\ \hline
\end{tabular}%
}
\caption{Some traffic-related works using deep learning. The default dataset is generated by the author of each work. The default metric is accuracy.}
\label{tab:trackingontraffic}
\end{table}

-traffic monitoring:
tracking by detecting

DL detect+ extact spatio-temporal features:
                    \cite{fernandez2019real}ehicles are identified through a deep learning based detector. Second, tracking is performed with a combination of a Discriminative Correlation Filter and a Kalman Filter.
                 86.96  CNN detector+DCF+Kalman filter MOT 15\cite{}
                    

-qiu2018kestrel      YOLO+KLT     75.9 RECALL 88.6P TKI and Desktop   


-lopez2019boosting Faster R-CNN   0.305AP subset:M-30 0.662 subset:M-30-HD 0.381 subset:Urban1          GRAM-RTM
-xu2017car    Faster R-CNN 98.43     

-scheidegger2018mono         CNN+Poisson multi-Bernoulli mixture tracking filter(PMBM)\cite{garcia2018poisson} 80.04 mota kitti
   
-zou2019multi Siamese network+SPP+Markov Decision Process(MDP)
multiple-object tracking accuracy (MOTA) 75.29 campus 76.06 urban 78.14 highway on KITTI

-li2019spatio FPN+tracking loss 83.2IDF1 nivida AI city

-nikodem2020multi  hourglass single-camera tracing accuracy of at least 97 multi-camera east 91

-zhao2018autonomous  SSD+dual Kalman filters Performance shown in form of figures

- wang2019orientation  YOLOv3+SIFT 81.3
- usmankhujaev2020real yoloV3+kalman filter 100 Daytime 89.83 Daytime(flipped) Nighttime(flipped) 86.11

DL: 
-kwan2018compressiv  ResNet compressive measurements
%\cite{wang2018learning}

%but deep learning is relatively time-consumi


$RMSE=\sqrt{\sum_{i=1}^N(p_i-a_i)^2/N}$
$p_i$ and $a_i$ represent the predicted and actual outcome.


NVIDIA AI CITY challenge\cite{ai_city_challenge}
Track 1: 31 video clips (about 9 hours in total) captured from 20 unique camera views



Vehicle Counting 9 hours of videos captured from 20 different vantage points
covering various lighting and weather conditions most 10fps

Track 2:Re-ID
56,277 images, of which 36,935 come from 333 object identities 

track 3:Vehicle Tracking

215.03 minutes of videos collected from 46 cameras spanning 16 intersections
 300K bounding boxes for 880 distinct annotated vehicle identities.
 
track 4: Traffic Anomaly Detection 
200 15mins videos 30fps
Anomalies can be due to car crashes or stalled vehicles


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|}
\hline
Task & Models \\ \hline
scene understanding &
  \begin{tabular}[c]{@{}l@{}}\cite{romera2017erfnet} pixel accuracy>95 Cityscapes\\ \cite{lyu2019esnet} 63.2 mIoU Cityscapes\\ \cite{deng2017cnn} 54.5 mIoU Cityscapes\\ \cite{saez2018cnn} 59.3  mIoU Cityscapes\\ \cite{kendall2015bayesian} 63.1 mIoU  CamVid\end{tabular} \\ \hline
Free space estimation &
  \begin{tabular}[c]{@{}l@{}}\cite{ohgushi2020road} 21.9 mIoU\\ \cite{hua2019small} Path planning accuracy\\  0.15m Indoor and 0.27m Outdoor\\ \cite{levi2015stixelnet} 0.87 AUC \\ 89.12\% maxF SEGMENTATION on KITTI\\ \cite{deepika2017obstacle} 0.9667 IoU\end{tabular} \\ \hline
Stixel representation &
  \begin{tabular}[c]{@{}l@{}}\cite{cordts2017stixel} 83.1 exact Disparity accuracy \\ \cite{schneider2016semantic} 7.8 Disparity accuracy\\ \cite{erbs2012stixmentation}88.64 Stixel-wise percentage accuracy\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Some semantic segmentation works In the traffic field. If the dataset is not indicated, it means the current work uses the dataset generated by its authors}
\label{tab:semanticwork}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Task &
  Works &
  Methods \\ \hline
scene understanding &
  \begin{tabular}[c]{@{}l@{}}\cite{romera2017erfnet} pixel accuracy$>$95 Cityscapes\\ \cite{lyu2019esnet} 63.2 mIoU Cityscapes\\ \cite{deng2017cnn} 54.5 mIoU Cityscapes\\ \cite{saez2018cnn} 59.3  mIoU Cityscapes\\ \cite{kendall2015bayesian} 63.1 mIoU  CamVid\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Autoencoder\\ Edge Detection Network+Fusion\\ CNN+pyramid pooling module\\ Autoencoder\\ Bayesian Autoencoder\end{tabular} \\ \hline
Free space estimation &
  \begin{tabular}[c]{@{}l@{}}\cite{ohgushi2020road} 21.9 mIoU\\ \cite{hua2019small} Path planning accuracy\\  0.15m Indoor and 0.27m Outdoor\\ \cite{levi2015stixelnet} 0.87 AUC \\ 89.12\% maxF SEGMENTATION on KITTI\\ \cite{deepika2017obstacle} 0.9667 IoU\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Autoencoder\\ Autoencoder+fusion+optical flow\\ \\ CNN\\ \\ SegNet\end{tabular} \\ \hline
Stixel representation &
  \begin{tabular}[c]{@{}l@{}}\cite{schneider2016semantic} \\ 7.8 Disparity Error on KITTI 15.2 on Ladicky\cite{ladicky2014pulling}\\ \cite{cordts2017stixel} 83.1 exact Disparity accuracy\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}FCN+SGM\\ \\ FCN+SGM+graphical model\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Some semantic segmentation works In the traffic field.}
\label{tab:semanticwork}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Task &
  Works &
  Methods \\ \hline
\begin{tabular}[c]{@{}l@{}}obtain comprehensive\\  vehicle information\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\cite{zhang2015monocular} 59.0 object recall,\\ 83.1\% of the randomly sampled foreground pixel pairs ordered on KITTI \\ \cite{mou2018vehicle} 95.87 F1 score on ISPRS\\ \cite{zhang2020traffic} 97\%  vehicle types accuracy\\ \cite{huang2018measuring} 1.333 front 4.698 side-way KITTI\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}CNN+MRF\\ 11\\ ResFCN\\ Mask R-CNN\\ Mask R-CNN\end{tabular} \\ \hline
Lane detection &
  \begin{tabular}[c]{@{}l@{}}\cite{neven2018towards} 96.4\% accruacy\\ \cite{roberts2018dataset}IoU Mapillary 82.9  CityScapes 85.2\\  KITTI 83.8 author's dataset 95\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}multi-task CNN\\ SegNet\end{tabular} \\ \hline
3D reconstruction &
  \begin{tabular}[c]{@{}l@{}}\cite{hadi2020semantic} AP@50\% 8.862 CityScapes 43.949\\ IDD\cite{varma2019idd} 5.643WildDash\cite{zendel2018wilddash}\end{tabular} &
  Mask R-CNN \\ \hline
\end{tabular}%
}
\caption{Some instance segmentation works In the traffic field. If the dataset is not indicated, it means the current work uses the dataset generated by its authors}
\label{tab:instancework}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Works                  & Performance                                        & Methods                                   \\ \hline
\cite{nguyen2020anomaly}      & F1 score 0.9412   AI City Challenge 2019           & GAN                                       \\ \hline
\cite{yao2019unsupervised}    & 60.1 AUC on A3D Dataset & \begin{tabular}[c]{@{}l@{}}Auto Encoder-Decoder\\ with GRU\end{tabular}                   \\ \hline
\cite{tian2019automatic}      & 90.02 AP  CAD-CVIS                                 & YOLO-CA                                   \\ \hline
\cite{kim2020pre}            & 0.82                                               & 3D conv                                   \\ \hline
\cite{ijjina2019computer}     & 71                                                 & 3D conv                                   \\ \hline
\cite{shah2018cadp}           & 47.25 on CADP           & \begin{tabular}[c]{@{}l@{}}DSA-RNN\cite{chan2016anticipating}\\ Faster R-CNN\end{tabular} \\ \hline
\cite{srinivasan2020novel}    & 78.2 on CADP                                       & Detection Transformer\cite{carion2020end} \\ \hline
\cite{suzuki2018anticipating} & 99.1 mAP                & QRNN\cite{bradbury2016quasi}+DeCAF\cite{donahue2014decaf}                                 \\ \hline
\cite{giannakeris2018speed}   & F1-score 0.33 RMSE 227   on NVIDIA CITY Track 2    & Faster RCNN                               \\ \hline
\cite{arceda2018fast}         & 89                                                 & YOLO+ViF\cite{hassner2012violent}+SVM     \\ \hline
\cite{biradar2019challenges}  & F1-score 0.3838 RMSE 93.61 on NVDIA CITY Track 3   & YOLOv2+ CNN                               \\ \hline
\cite{xu2018dual}             & F1-score 0.8649 RMSE 3.6152 on NVIDIA CITY Track 2 & Mask-RCNN+ ResCNN                         \\ \hline
\cite{doshi2020fast}          & F1-score 0.5926 RMSE 8.2386 on NVIDIA CITY track 4 & YOLO+KNN+K-means                          \\ \hline
\cite{zhou2016spatial} & 95.2 on U-turn dataset \cite{benezeth2009abnormal} & 3D CNN                                    \\ \hline
\cite{franklin2020traffic}    & 100 and 95.34 for input video 1 and video 2            & YOLOv3                                  \\ \hline
\end{tabular}%
}
\caption{Some recent deep learning works for video-based traffic abnormal detection. Unless otherwise specified, the non-indicated numbers is the accuracy}
\label{tab:abnormaldetect}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Works               & Performance                  & Methods                                 \\ \hline
\cite{qiu2018kestrel}      & 75.9 Recall 88.6 Accuracy    & YOLO+KLT                                \\ \hline
\cite{lopez2019boosting} &
  \begin{tabular}[c]{@{}l@{}}0.305AP subset:M-30 0.662AP subset:M-30-HD \\ 0.381AP subset:Urban1 of  GRAM-RTM\end{tabular} &
  Faster R-CNN \\ \hline
\cite{xu2017car}           & 98.43                        & Faster R-CNN                            \\ \hline
\cite{scheidegger2018mono} & 80.04 MOTA on KITTI          & CNN+PMBM filter\cite{garcia2018poisson} \\ \hline
\cite{zou2019multi} &
  \begin{tabular}[c]{@{}l@{}}75.29MOTA campus \\ 76.06MOTAurban \\ 78.14MOTA highway \\ on KITTI\end{tabular} &
  Siamese network+SPP+MDP \\ \hline
\cite{li2019spatio}        & 83.2IDF1 nivida AI city      & FPN+tracking loss                       \\ \hline
\cite{nikodem2020multi} &
  \begin{tabular}[c]{@{}l@{}}MOTA 97+\\ MCTA 91+\end{tabular} &
  hourglass \\ \hline
\cite{zhao2018autonomous}  & Shown in the form of figures & SSD+dual Kalman filters                 \\ \hline
\cite{wang2019orientation} & 81.3                         & YOLOv3+SIFT                             \\ \hline
\cite{usmankhujaev2020real} &
  \begin{tabular}[c]{@{}l@{}}100 Daytime \\ 89.83 Daytime(flipped) \\ 86.11 Nighttime(flipped)\end{tabular} &
  yoloV3+kalman filter \\ \hline
\cite{kwan2018compressive}  & For compressive measurements & ResNet                                  \\ \hline
\cite{fernandez2019real} &
  86.96 MOTA on MOT 15\cite{leal2015motchallenge} &
  CNN detector+DCF+Kalman filter \\ \hline
\end{tabular}%
}
\caption{Some traffic-related tracking works using deep learning. The default dataset is generated by the author of each work. The default metric is accuracy.}
\label{tab:trackingontraffic}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Task &
  Methods &
  Methods \\ \hline
\multirow{}{}{Vehicle Detection} &
  R-CNN family &
  \begin{tabular}[c]{@{}l@{}}\cite{espinosa2017vehicle} 70\\ \cite{wang2019comparative} \\ \cite{wang2017evolving}84.43 DETRAC dataset\\ \cite{soin2017moving}  100\\ \cite{zhang2017application} 96.5\\ \cite{peppa2018urban} 97\end{tabular} \\ \cline{2-3} 
 &
  YOLO family &
  \begin{tabular}[c]{@{}l@{}}\cite{sang2018improved} 99.51  BIT-Vehicle\\ \cite{kim2019multi}85.29 UA-DETRAC\end{tabular} \\ \cline{2-3} 
 &
  SSD &
  \begin{tabular}[c]{@{}l@{}}\cite{zhang2019vehicle} 77.94 mAP  UA-DETRAC\\ \cite{chen2020inception} 86.2 KITTI 87.4UVD\\ \cite{cao2020front} 92.18 KITTI\\ \cite{peppa2018urban} 98.2\end{tabular} \\ \cline{2-3} 
 &
  Others &
  \cite{6778050} 99.7 \\ \hline
\multirow{}{}{Plate Detection} &
  R-CNN family &
  \cite{lee2016real} 99.94 \\ \cline{2-3} 
 &
  YOLO family &
  \begin{tabular}[c]{@{}l@{}}\cite{hsu2017robust} \\ \cite{kessentini2019two} 97.67\% on GAP-LP dataset  91.46 on Radar\\ \cite{khazaee2020real} 97.9\\ \cite{xie2018new} 98.32 UCSD PKU\\ \cite{chen2019automatic} 98.22 AOLP\end{tabular} \\ \cline{2-3} 
 &
  SSD &
  \begin{tabular}[c]{@{}l@{}}\cite{ren2020implementation} 92\\ \cite{hu2020mobilenet} 90.12\\ \cite{danilenko2020license} 94+\end{tabular} \\ \cline{2-3} 
 &
  Others &
  \begin{tabular}[c]{@{}l@{}}\cite{kim2017deep} 98.39 on Caltech\\ \cite{selmi2017deep} 94.8 on Caltech\\ \cite{masood2017license} 99.09 US 99.64 EU\end{tabular} \\ \hline
\multirow{}{}{\begin{tabular}[c]{@{}l@{}}Traffic Sign \\ Detection\end{tabular}} &
  R-CNN family &
  \begin{tabular}[c]{@{}l@{}}\cite{qian2016road} 85.58\\ \cite{shao2019improved} 69.56 gtsdb+ctsd\\ \cite{zhang2020cascaded} 98.7 GTSDB\\ \cite{zuo2017traffic} 0.3449 on CCF2016\\ \cite{wu2019traffic} mAP  91.75  GTSDB\\ \cite{peng2016traffic} mAP ~90 GTSDB\end{tabular} \\ \cline{2-3} 
 &
  YOLO family &
  \begin{tabular}[c]{@{}l@{}}\cite{zhang2017real} 96.69 on CCTSDB and GTSDB\\ \cite{Tai_2020} 99.1 mAP\end{tabular} \\ \cline{2-3} 
 &
  SSD &
  \begin{tabular}[c]{@{}l@{}}\cite{gao2019traffic} 91.0 GTSDB\\ \cite{you2020traffic}0.75 TT100K\end{tabular} \\ \cline{2-3} 
 &
  Others &
  \begin{tabular}[c]{@{}l@{}}\cite{zhu2016traffic}91 TT100K\\ \cite{wu2013traffic}AUC 99.73 “danger” , 97.62 "mandatory" on GTSDB\\ \cite{shustanov2017cnn} 99.94 GTSDB\end{tabular} \\ \hline
\end{tabular}%
}
\caption{some object detection tasks of traffic works. If the dataset is not indicated, it means the current work uses the dataset generated by its authors}
\label{tab:objectdetection}
\end{table}


LP: AOLP\cite{hsu2012application}
caltech\cite{}

\begin{table}[]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|}
\hline
Accuracy &
  $\frac{Correct predictions}{Total predictions}$ \\ \hline
Recall (R) &
  $\frac{TP}{TP+FN}$ \\ \hline
Precision (P) &
  $\frac{TP}{TP+FP}$ \\ \hline
F1 score &
  $2\times\frac{P\times R}{P+ R}$ \\ \hline
Pixel Accuracy (PA) &
  $\frac{TP+TN}{TP+TN+FP+FN}$ \\ \hline
Normalized error (mean)\cite{huang2018measuring} &
  \begin{tabular}[c]{@{}l@{}}$normalized error=\frac{|d-d_{gt}|}{d_{gt}}$. \\ $d$ is the calculated distance and \\ $d_{gt}$ is the ground truth of distance.\end{tabular} \\ \hline
Average Precision (AP) &
  $AP=\int_0^1 P(R)dR$ P-R CURVE (for one class) \\ \hline
mean Average Precision (mAP) &
  $mean(AP_i)$ \\ \hline
Intersection over Union (IoU) &
  \begin{tabular}[c]{@{}l@{}}$\frac{B_p\cap B_{gt}}{B_p\cup B_{gt}}$\\ $B_{gt}$: ground truth bounding box\\ $B_{p}$: predicted bounding box\end{tabular} \\ \hline
Disparity accuracy &
   \\ \hline
Stixel-wise percentage accuracy &
  Similar to PA \\ \hline
Identification F1-Score (IDF1) &
  $IDF1=\frac{2IDTP}{2IDTP+IDFP+IDFN}$ \\ \hline
multiple object tracking accuracy (MOTA) &
  \begin{tabular}[c]{@{}l@{}}$MOTA=1-\frac{FN+FP+\Phi}{T}$\\ $\Phi$ denotes the number of fragmentations\end{tabular} \\ \hline
Multi-camera Tracking Accuracy (MCTA) &
  \begin{tabular}[c]{@{}l@{}}$MCTA= \underbrace{\frac{2PR}{P+R}}_{F_1} \underbrace{(1-\frac{M^w}{T^w})}_{\text{within camera}} \underbrace{(1-\frac{M^h}{T^h})}_{\text{handover}}$\\ $M^w$: within-camera identity mismatches \\ $T^w$:  true within-camera detections\\ $M^h$:  handover mismatches\\ $T^h$:  true handover detections\end{tabular} \\ \hline

RMSE & $RMSE=\sqrt{\sum_{i=1}^N(p_i-a_i)^2/N}$ \\ \hline
\end{tabular}%
}
\caption{Some metrics to evaluate traffic works.TP:True Positive TN: True Negative FP:False Positive FN:False Negative}
\label{tab:somemetrics }
\end{table}
UCF-Crimes\cite{sultani2018real}: 1900 sequences 128hours. 151 events
13 realistic anomalies such as fighting, road accident, burglary, robbery, etc
No spatial annotation

DAD\cite{chan2016anticipating}: 1730 sequences 2.4 hours 620 events
spatio-temporal annotation 
dashcam accident videos.

CADP\cite{shah2018cadp}: 1416 sequences 5.2 hours 1416 events
include multi-accident sequences
varied environment
captured by CCTV
\begin{table*}[]
\centering
%\begin{adjustbox}{angle=90}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
Paper:  [REF](year)                   & \cite{shirazi2016looking}(2016) & \cite{sivaraman2013looking}(2013) &\cite{khan2017uav} (2017) & \cite{zheng2014traffic}(2014) & \cite{wali2015comparative}(2015) &\cite{morris2013understanding}(2013) & \cite{mukhtar2015vehicle}(2015)  & \cite{janai2017computer}(2017) & \cite{nguyen2018deep}(2018)& \cite{badue2020self}(2020) &\cite{yurtsever2020survey} (2020) & \textbf{Ours}\\ \hline
Human-driven Vehicle       & H    & H    & H    & H    & H    & H    & H       & L  & H & L    & L    & H    \\ \hline
Safety Assessment Analysis & H    & L    & L    & H    & L    & M    & L        & L & L  & L    & L    & M    \\ \hline
Video-based Method         & H    & H    & H    & L    & H    & H    & H        & H & L  & M    & M    & H    \\ \hline
Deep Learning Method       & L    & M    & M    & L    & L    & L    & L        & H & H & M    & H    & H    \\ \hline
Perspective                & E    & E    & E    & E    & I    & E    & I        & I & E  & I    & I    & E    \\ \hline

relations to AVs       & L    & L    & L    & L    & L    & L    & L        & H & L & H   & H    & H    \\ \hline
relations to insurance       & X    & X    & X    & X    & X    & X    & X        & X & X & X    & X    & L    \\ \hline
relations to  psychology        & X    & X    & X    & X    & X    & X    & X        & X & X & X    & X    & M    \\ \hline
relations to  Crowd-sourcing        & X    & X    & X    & X    & X    & X    & X        & X & X & X    & X    & L    \\ \hline
Network Analysis        & X    &H   & M    & M    & X    & H    & X       & H & H &M    & M    & H    \\ \hline
\end{tabular}%
}
%\end{adjustbox}
\caption{Summary of related review papers. 'H', 'M', and 'L' denote the different extent of content, respectively 'high', 'moderate', and 'low'. 'X' means that the topic is not covered. 'E' denotes the external observers' perspective, while 'I' denotes the internal nodes' perspective.}  
\label{tab:surveys}
\end{table*}


\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline \rowcolor{gray}
\textbf{Paper: [REF](year)} &
  \cite{shirazi2016looking}(2016) &
  \cite{sivaraman2013looking}(2013) &
  \cite{khan2017uav} (2017) &
  \cite{zheng2014traffic}(2014) &
  \cite{wali2015comparative}(2015) &
  \cite{morris2013understanding}(2013) &
  \cite{mukhtar2015vehicle}(2015) &
  \cite{janai2017computer}(2017) &
  \cite{nguyen2018deep}(2018) &
  \cite{badue2020self}(2020) &
  \cite{yurtsever2020survey} (2020) &
  \cite{wang2019enhancing}(2019) &
  \cite{grigorescu2020survey}(2020) &
  \cite{mozaffari2020deep}2020 &
  \textbf{Ours} \\ \hline
\begin{tabular}[c]{@{}c@{}}Human-driven \\ Vehicle\end{tabular}         & H & H & H & H & H & H & H & L & H & L & L & H & L & L & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Safety Assessment\\  Analysis\end{tabular}   & H & L & L & H & L & M & L & L & L & L & L & L & M & L & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Video-based\\  Method\end{tabular}           & H & H & H & L & H & H & H & H & L & M & M & M & H & M & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Deep Learning \\ Method\end{tabular}         & X & X& X & X & L & X & L & H & H & H & H & H & H & H & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Perspective\\ ~\end{tabular}                 & E & E & E & E & I & E & I & I & E & I & I & E & I & E & E \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to\\  AVs\end{tabular}             & L & L & L & L & L & L & L & H & L & H & H & M & H & H & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to \\ insurance\end{tabular}       & X & X & X & X & X & X & X & X & X & X & X & X & X & X & L \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to \\ psychology\end{tabular}      & X & X & X & X & X & X & X & X & X & X & X & X & X & X & M \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to  \\ Crowd-sourcing\end{tabular} & X & X & X & X & X & X & X & X & X & X & X & X & X & X & L \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to\\ Edge Computing\end{tabular}   & X & X & X & X & X & X & X & X & X & X & X & X & X & X & M \\ \hline
\begin{tabular}[c]{@{}c@{}}Network\\ Analysis\end{tabular}                                                        & X & H & M & M & X & H & X & H & H & M & M & H & X& M & H \\ \hline
\end{tabular}%
}
\caption{Summary of related review papers. 'H', 'M', and 'L' denote the different extent of content, respectively 'high', 'moderate', and 'low'. 'X' means that the topic is not covered. 'E' denotes the external observers' perspective, while 'I' denotes the internal nodes' perspective. \arr{keep this for our reference and make another copy only with checkmark and dash or "X" sign, for 2 reasons: 1-to make it more clear, and 2-it is hard to evaluate H/M/L for others paper...If they cover it at a reasonable level put "checkmark" otherwise "X" or "-"}}
\label{tab:surveys}
\end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline \rowcolor{gray}
\textbf{Paper: [REF](year)} &
  \cite{shirazi2016looking}(2016) &
  \cite{sivaraman2013looking}(2013) &
  \cite{khan2017uav} (2017) &
  \cite{zheng2014traffic}(2014) &
  \cite{wali2015comparative}(2015) &
  \cite{morris2013understanding}(2013) &
  \cite{mukhtar2015vehicle}(2015) &
  \cite{janai2017computer}(2017) &
  \cite{nguyen2018deep}(2018) &
  \cite{badue2020self}(2020) &
  \cite{yurtsever2020survey} (2020) &
  \cite{wang2019enhancing}(2019) &
  \cite{grigorescu2020survey}(2020) &
  \cite{mozaffari2020deep}2020 &
  \textbf{Ours} \\ \hline
\begin{tabular}[c]{@{}c@{}}Human-driven \\ Vehicle\end{tabular}         & H & H & H & H & H & H & H & L & H & L & L & H & L & L & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Safety Assessment\\  Analysis\end{tabular}   & H & L & L & H & L & M & L & L & L & L & L & L & M & L & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Video-based\\  Method\end{tabular}           & H & H & H & L & H & H & H & H & L & M & M & M & H & M & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Deep Learning \\ Method\end{tabular}         & X & X& X & X & L & X & L & H & H & H & H & H & H & H & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Perspective\\ ~\end{tabular}                 & E & E & E & E & I & E & I & I & E & I & I & E & I & E & E \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to\\  AVs\end{tabular}             & L & L & L & L & L & L & L & H & L & H & H & M & H & H & H \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to \\ insurance\end{tabular}       & X & X & X & X & X & X & X & X & X & X & X & X & X & X & L \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to \\ psychology\end{tabular}      & X & X & X & X & X & X & X & X & X & X & X & X & X & X & M \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to  \\ Crowd-sourcing\end{tabular} & X & X & X & X & X & X & X & X & X & X & X & X & X & X & L \\ \hline
\begin{tabular}[c]{@{}c@{}}Relations to\\ Edge Computing\end{tabular}   & X & X & X & X & X & X & X & X & X & X & X & X & X & X & M \\ \hline
\begin{tabular}[c]{@{}c@{}}Network\\ Analysis\end{tabular}                                                        & X & H & M & M & X & H & X & H & H & M & M & H & X& M & H \\ \hline
\end{tabular}%
}
\caption{Summary of related review papers. 'H', 'M', and 'L' denote the different extent of content, respectively 'high', 'moderate', and 'low'. 'X' means that the topic is not covered. 'E' denotes the external observers' perspective, while 'I' denotes the internal nodes' perspective. \arr{keep this for our reference and make another copy only with checkmark and dash or "X" sign, for 2 reasons: 1-to make it more clear, and 2-it is hard to evaluate H/M/L for others paper...If they cover it at a reasonable level put "checkmark" otherwise "X" or "-"}}
\label{tab:surveys}
\end{table*}
\begin{table*}[]
\centering
\caption{Summary of related review papers. 
%'H', 'M', and 'L' denote the different extent of content, respectively 'high', 'moderate', and 'low'. 'X' means that the topic is not covered. 'E' denotes the external observers' perspective, while 'I' denotes the internal nodes' perspective. \arr{keep this for our reference and make another copy only with checkmark and dash or "X" sign, for 2 reasons: 1-to make it more clear, and 2-it is hard to evaluate H/M/L for others paper...If they cover it at a reasonable level put "checkmark" otherwise "X" or "-"}\xc{Updated for the latest chose surveys. The text content still needs to update. Additionally, it seems we removed edge computing in this version, which means we need to remove the row for edge computing.}
\arr{Good job. I like this Table, and it can be the instrumental in getting this paper accepted if we convince the reviewer that it is accurate and complete. A few more comments: a) it should be consistent with text, b) it is ok to include some older References and if we need we can include 2 tables one on top of another, c) if we include more review papers we can have "o" with note that this topic is covered but is outdated, d) it might be questionable that for many topics like "Related to Insurance", "crowd-sourcing", and "Edge computing", is not covered by any of the previous papers, it might be better for only 2 of these unique aspects (not all of them) you include a paper focused only on this matter, like finding a paper that reviews edge computing from traffic data. e) Bring back the Edge computing from the Access, if it is removed it must be a mistake, f) you can also include some new aspects: like "sensors", "data collection methods", "public tools and datasets", "roadside infrastructures", g) if you include Human-driven vehicles, better to add another row for "Autonomous vehicles" right after it (perhaps you can just move relation to AVs to 2nd row".}
}
\label{tab:surveys}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline\rowcolor{gray}
\textbf{Paper:   {[}REF{]}} &
  REF: \cite{hu2020review} &  
  REF: \cite{mozaffari2020deep} &  
  REF: \cite{grigorescu2020survey} & 
  REF: \cite{yurtsever2020survey} &   
  REF: \cite{janai2017computer} &
  REF: \cite{badue2020self} &
  REF: \cite{kumaran2019anomaly} &
  REF: \cite{wang2019enhancing} &
  REF: \cite{nguyen2018deep} &
  REF: \textbf{Ours} \\ 
\textbf{(year)} &
  (2020) &  
  (2020) &  
  (2020) &
  (2020) &   
  (2020) &
  (2020) &
  (2019) &
  (2019) &
  (2018) &
  \textbf{ } \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Human-driven\\      Vehicle\end{tabular}}          & $\surd$ & $\surd$ &    &    &    &    & $\surd$ & $\surd$ & $\surd$ & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Safety   Assessment\\      Analysis\end{tabular}}  & $\surd$ & $\surd$ & $\surd$ &    &    &    & $\surd$   &    &    & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Video-based\\      Method\end{tabular}}            & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Deep   Learning\\      Method\end{tabular}}        & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Relations   to\\      Avs\end{tabular}}            & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ &    &    & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Relations   to\\      insurance\end{tabular}}      &    &    &    &    &    &    &    &    &    & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Relations   to\\      psychology\end{tabular}}     &    &    &    &    &    &    &    &    &    & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Relations   to\\      Crowd-sourcing\end{tabular}} &    &    &    &    &    &    &    &    &    & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Relations   to\\      Edge Computing\end{tabular}} &    &    &    &    &    &    &    &    &    & $\surd$ \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Network\\      Analysis\end{tabular}}              & $\surd$ & $\surd$ &    &    &    &    & $\surd$ & $\surd$ & $\surd$ & $\surd$ \\ \hline
\end{tabular}%
}
\end{table*}


\begin{table*}[]
\begin{center}
\begin{tabular}{|l|l|l|}
\hline\rowcolor{gray}
\textbf{Task}                                                         & \textbf{DataSet}            & \textbf{Description }              \\ \hline Object Classification
                                     & Cifar-10/100       & Natural image             \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                       & MNIST              & Hand-writen digits        \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                       & ImageNet           & Natural image             \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                       & Fasion-MNIST       & Fasion items              \\ \hline
Scene Classification                      & UIUC-Sports        & Sports events             \\ \cline{2-3} 
                                                             & Place365           & Indoor and outdoor scenes \\ \cline{2-3} 
                                                             & ADE20k             & Indoor and outdoor scenes \\ \hline
Fine-grained Classification                 & CUB200             & Birds                     \\ \cline{2-3} 
                                                             & Stanford dogs/cats & Dogs/Cats                 \\ \cline{2-3} 
                                                             & Oxford flowers     & Flowers                   \\ \hline
\end{tabular}
\end{center}
\caption{Differences datasets for classification tasks, which can be used for initial performance analysis of DL-based classification methods, even in the context of traffic analysis.} 
%\arr{This is good but not relevant to our paper. Develop tables for datasets or methods relevant to classification tasks in traffic analysis. In general our goal is not reviewing DL methods but reviewing their use, applicability, and role in Traffic [safety] analysis. A table with a header like "method[REF]  - DL Method -  application  accuracy", and in DL method you put the method name like GoogleNet and in the application you put something like vehicle type classification}\xc{I think we can remove the table. Traffic-related scene classification is often solved by segmentation methods. And most of the works(On Table.\ref{tab:objectdetection}, except\cite{soin2017moving,peppa2018urban,6778050} ) we mentioned on the object detection section also do car type classification. We can mention it on this section.}}
\label{tab:Classifaction Datasets}
\end{table*}

\begin{table*}[]
\centering
\caption{Summary of related review papers. 
%\arr{Good job. I like this Table, and it can be the instrumental in getting this paper accepted if we convince the reviewer that it is accurate and complete. A few more comments: a) it should be consistent with text, b) it is ok to include some older References and if we need we can include 2 tables one on top of another, c) if we include more review papers we can have "o" with note that this topic is covered but is outdated, d) it might be questionable that for many topics like "Related to Insurance", "crowd-sourcing", and "Edge computing", is not covered by any of the previous papers, it might be better for only 2 of these unique aspects (not all of them) you include a paper focused only on this matter, like finding a paper that reviews edge computing from traffic data. e) Bring back the Edge computing from the Access, if it is removed it must be a mistake, f) you can also include some new aspects: like "sensors", "data collection methods", "public tools and datasets", "roadside infrastructures", g) if you include Human-driven vehicles, better to add another row for "Autonomous vehicles" right after it (perhaps you can just move relation to AVs to 2nd row".}
\xc{Updated. The paper with '*' means although this paper is related but outdated.} \arr{This new table is good. Split miscellaneous points as we discussed, 2) use \checkmark and L\checkmark if a topic is covered in less details. I means instead of using "*" for limited content per paper it is better to use it per topic and you already have this information from the previous TABLe!!!. }}
\label{tab:surveys}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline\rowcolor{gray}
\textbf{Paper}                                                                                                                                                      & \cite{hu2020review}Hu et al.& \cite{mozaffari2020deep}Mozaffari et al. & \cite{grigorescu2020survey}Grigorescu et al. & \cite{yurtsever2020survey}Yurtsever et al. & \cite{janai2017computer}Janai et al. & \cite{badue2020self}Badue et al. & \cite{kumaran2019anomaly}kumaran et al. & \cite{wang2019enhancing}Wang et al. & \cite{nguyen2018deep}Nguyen et al.& *\cite{shirazi2016looking}shirazi et al.& *\cite{mukhtar2015vehicle}Mukhtar et al. & *\cite{morris2013understanding} Morris et al.& Ours \\ \hline
\textbf{Year}                                                                                                                                                       & 2020                      & 2020                           & 2020                              & 2020                             & 2020                           & 2020                       & 2019                            & 2019                           & 2018                        & 2016                            & 2015                      & 2013                           &      \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Human-driven\\      Vehicle\end{tabular}}                                                                                        & $\surd$                        & $\surd$                             &                                   &                                  &                                &                            & $\surd$                              & $\surd$                             & $\surd$                          & $\surd$                              & $\surd$                        & $\surd$                             & $\surd$   \\ \hline
\textbf{Avs}                                                                                                                                                        & $\surd$                        & $\surd$                             & $\surd$                                & $\surd$                               & $\surd$                             & $\surd$                         & $\surd$                              &                                &                             &                                 &                           &                                & $\surd$   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Safety   Assessment\\      Analysis\end{tabular}}                                                                                & $\surd$                        & $\surd$                             & $\surd$                                &                                  &                                &                            & $\surd$                              &                                &                             & $\surd$                              &                           & $\surd$                             & $\surd$   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Video-based\\      Method\end{tabular}}                                                                                          & $\surd$                        & $\surd$                             & $\surd$                                & $\surd$                               & $\surd$                             & $\surd$                         & $\surd$                              & $\surd$                             & $\surd$                          & $\surd$                              & $\surd$                        & $\surd$                             & $\surd$   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Deep   Learning\\      Method\end{tabular}}                                                                                      & $\surd$                        & $\surd$                             & $\surd$                                & $\surd$                               & $\surd$                             & $\surd$                         & $\surd$                              & $\surd$                             & $\surd$                          &                                 &                           &                                & $\surd$   \\ \hline
\textbf{Sensors}                                                                                                                                                    & $\surd$                        &                                & $\surd$                                & $\surd$                               & $\surd$                             & $\surd$                         &                                 &                                &                             & $\surd$                              & $\surd$                        &                                &      \\ \hline
\textbf{Datasets}                                                                                                                                                   &                           &                                & $\surd$                                & $\surd$                               & $\surd$                             &                            & $\surd$                              &                                &                             & $\surd$                              &                           & $\surd$                             &      \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Network\\      Analysis\end{tabular}}                                                                                            & $\surd$                        & $\surd$                             &                                   &                                  &                                &                            & $\surd$                              & $\surd$                             & $\surd$                          &                                 &                           & $\surd$                             & $\surd$   \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Miscellaneous\\       Points\\      (Insurance, Psychology, \\      Crowd-sourcing,\\ Vehicular Edge Computing, \\      etc.,)\end{tabular}} &                           &                                &                                   &                                  &                                &                            &                                 &                                &                             &                                 &                           &                                & $\surd$   \\ \hline
\end{tabular}%
}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{List of sample problems to assess the overall safety of a highway segment. The short codes include MOT: multi-object tracking, OD: object detection, IS: instance segmentation, TE: trajectory extraction, SS: semantic segmentation, EP: environment prior, C: classification. The tasks with '*' meaning that these tasks can be solved by obtaining the relationships (distance, velocity) among vehicles and determining a threshold from the relationships. \arr{use consistent format like "Traffic Blocked--> Traffic blocked".} \arr{Good job, as we dicussed you can add more detailed steps and use '*' for steps that can be included or can be useful but is not necessary like denoising, video stabilization, super resolution, trajectory smoothing,etc. }}
\label{tab:problem}
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{|l|l|c|}
\hline\rowcolor{gray}
\textbf{Task}                                & \textbf{Processing Steps} & \textbf{Examples}                         \\ \hline
Vehicle Stopped on Shoulder            & EP-OD/MOT                   & \cite{xu2018dual}                                       \\ \hline
Car Accident                           & OD/MOT                      & \cite{tian2019automatic,nguyen2020anomaly}              \\ \hline
Emergency Vehicle on The Road          & Fine-grained OD             & \cite{nayak2019vision}                                  \\ \hline
Careless/evasive Lane Change           & MOT-TE-C                    & \cite{chen2017dangerous,ramyar2016identification}       \\ \hline
Debris in Roadway                      & EP-OT/SS                    & \cite{ohgushi2020road,hua2019small,deepika2017obstacle} \\ \hline
Traffic Blocked (Slowed-down)          & MOT-TE-(SE)                 & \cite{kaltsa2018multiple,wang2019abnormal}              \\ \hline
Sharp Braking                                 & MOT-TE                    & \cite{jiang2015analysis} \\ \hline
Passing Red Traffic Light              & OD(for sign may needed)-MOT & \cite{wonghabut2018traffic}                             \\ \hline
Traffic Composition                           & OD/MOT                    & \cite{dai2019video}      \\ \hline
*Vehicle Driving Obviously Excessively   Slow & MOT-TE                    &   -                                        \\ \hline
*Vehicle Driving Obviously Excessively   Fast & MOT-TE                    &   -                                        \\ \hline
Vehicle Driving in The Prohibited Area & EP-MOT-TE                   & \cite{nowosielski2016automatic}                         \\ \hline
Invalid Car in HOV                            & EP-OD/MOT                 &  -                                         \\ \hline
Improper (Careless) Entering the Road  & EP-MOT-C                    & \cite{datondji2016survey}                               \\ \hline
Improper (Careless) Exiting the Road   & EP-MOT-C                    & \cite{datondji2016survey}                               \\ \hline
Zigzag Driving                                & MOT-TE-C                  & \cite{chen2017dangerous} \\ \hline
*Distance Violation to Front Vehicle          & MOT-C                     &  -                                         \\ \hline
*Distance Violation to Side Vehicle           & MOT-C                     &  -                                         \\ \hline
Violation of the Lines                 & ET-MOT-TE                   & \cite{nowosielski2016automatic}                         \\ \hline
Pedestrian on The Road                        & OD/MOT                    &  -                                         \\ \hline
Bike/Motorcycle on The Road                   & OD/MOT                    &  -                                         \\ \hline
Trailer {[}Oversized Car{]} on The Road       & OD/MOT                    &  -                                         \\ \hline
\end{tabular}%
}
\end{table*}

\begin{table*}
\centering
\caption{Summary of related review papers. The paper with '*' means although this paper is related but outdated. $L\surd$ denotes a topic is covered in fewer details. }
\label{tab:surveys}\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccccccc} 
\toprule 
 \textbf{Paper}                                                                                                     & \cite{hu2020review}Hu et al.& \cite{mozaffari2020deep}Mozaffari et al. & \cite{grigorescu2020survey}Grigorescu et al. & \cite{yurtsever2020survey}Yurtsever et al. & \cite{janai2017computer}Janai et al. & \cite{badue2020self}Badue et al. & \cite{kumaran2019anomaly}kumaran et al. & \cite{wang2019enhancing}Wang et al. & \cite{nguyen2018deep}Nguyen et al.& *\cite{shirazi2016looking}shirazi et al.& *\cite{mukhtar2015vehicle}Mukhtar et al. & *\cite{morris2013understanding} Morris et al.& Ours         \\ 
\midrule 
\textbf{Year}                                                                          & 2020                  & 2020                  & 2020                  & 2020                  & 2020                  & 2020                  & 2019                  & 2019                  & 2018                  & 2016                  & 2015                  & 2013                  &                              \\ 

\begin{tabular}[c]{@{}c@{}}\textbf{Human-driven}\\\textbf{ Vehicle}\end{tabular}       & $\surd$               & $\surd$               &                       & $\surd$               &                       &                       & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$                      \\ 

\textbf{Avs}                                                                           & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$               &                       & $L\surd$              &                       &                       &                       & $\surd$                      \\ 

\begin{tabular}[c]{@{}c@{}}\textbf{Safety Assessment}\\\textbf{ Analysis}\end{tabular} & $\surd$               & $\surd$               & $\surd$               & $\surd$               &                       &                       & $\surd$               &                       &                       & $\surd$               &                       & $\surd$               & $\surd$                      \\ 

\begin{tabular}[c]{@{}c@{}}\textbf{CV-based}\\\textbf{ Method}\end{tabular}            & $\surd$               & $L\surd$              & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $L\surd$              & $\surd$               & $\surd$               & $\surd$               & $\surd$                      \\ 

\begin{tabular}[c]{@{}c@{}}\textbf{Deep Learning}\\\textbf{ Method}\end{tabular}       & $L\surd$              & $\surd$               & $\surd$               & $\surd$               & $\surd$               & $L\surd$              & $\surd$               & $\surd$               & $L\surd$              &                       &                       &                       & $\surd$                      \\ 

\textbf{Sensors}                                                                       & $\surd$               &                       & $\surd$               & $\surd$               & $\surd$               & $\surd$               &                       &                       &                       & $\surd$               & $\surd$               &                       &         $\surd$                     \\ 

\textbf{Datasets}                                                                      &                       &                       & $\surd$               & $\surd$               & $\surd$               &                       & $\surd$               &                       &                       & $\surd$               &                       & $\surd$               &  $\surd$                            \\ 

\begin{tabular}[c]{@{}c@{}}\textbf{Network}\\\textbf{ Analysis}\end{tabular}           & $\surd$               & $\surd$               &                       &                       &                       &                       & $\surd$               & $\surd$               & $\surd$               &                       &                       & $\surd$               & $\surd$                      \\ 

\begin{tabular}[c]{@{}c@{}}\textbf{Vehicular }\\\textbf{Edge Computing}\end{tabular}   &                       &                       &                       &                       &                       &                       &                       &                       &                       &                       &                       &                       & $\surd$                      \\ 

%\textbf{\textbf{Psychology}} %              
\begin{tabular}[c]{@{}c@{}}\textbf{Behavioral \&}\\\textbf{Driver Cognition}\end{tabular}
& \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & {$\surd$}  \\
\bottomrule
\end{tabular}}
\end{table*}

==> figures/table.tex <==

\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
Method &
  Dataset &
  Performance(mAP) &
  Features \\ \hline
\multicolumn{4}{|l|}{\textit{One-stage}} \\ \hline
SDS (2014)\cite{hariharan2014simultaneous} &
  \begin{tabular}[c]{@{}l@{}}PASCAL VOC 2011\\ PASCAL VOC 2012\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}52.6\%\\ 51.6\%\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}MCG\cite{arbelaez2014multiscale} to generate proposal;\\ Define Instance Segmentation.\end{tabular} \\ \hline
DeepMask (2015)\cite{pinheiro2015learning} &
  \begin{tabular}[c]{@{}l@{}}PASCAL VOC 2007\\ MS COCO\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}improves Fast R-CNN  to 69.9\%@1.2s/image\\ @1.6s/image\end{tabular} &
  Bottom-up proposals generation. \\ \hline
SharpMask (2016)\cite{pinheiro2016learning} &
  MS COCO 2015 &
  25.1\%(AP), 45.8\%(AP^{50}), 24.8\%(AP^{75}) &
  \begin{tabular}[c]{@{}l@{}}Add top-down refinement network\\  to DeepMask.\end{tabular} \\ \hline
MNC (2016) \cite{dai2016MNC}&
  \begin{tabular}[c]{@{}l@{}}PASCAL VOC 2012\\ MS COCO 2015\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}63.5\% on validation set (mAP@0.5)\\ 29.7\% on test-dev set(mAP@0.5)\\ @360 ms/image\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}New Cascaded multi-task architecture;\\ End to End trainable;\\ No external modules.\end{tabular} \\ \hline
Mask R-CNN (2017)\cite{he2017mask} &
  MS COCO &
  \begin{tabular}[c]{@{}l@{}}37.1\%(AP), 60\%(AP^{50}), 39.4\%(AP^{75})\\ @200ms/frame\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}The extension version of Faster R-CNN;\\ \textit{RoIAlign} can better retain spatial information\end{tabular} \\ \hline
FCIS (2017)\cite{li2017fully} &
  \begin{tabular}[c]{@{}l@{}}PASCAL VOC 2012\\ MS COCO 2016\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}65.7\% (mAP@0.5) and 52.1\% (mAP@0.7) \\ 59.9\%(mAP@0.5) \\ @0.24s/image\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}The extension version of InstanceFCN\\ End to end trainable;\\ Can detect and segment objects jointly \\ and simultaneously; \\ Propose position-sensitive inside/outside \\ score maps.\end{tabular} \\ \hline
\multicolumn{4}{|l|}{\textit{Two-stage}} \\ \hline
InstanceFCN(2016)\cite{dai2016instance} &
  PASCAL VOC 2012 &
  61.5\% (mAP@0.5) and 43.0\% (mAP@0.7) &
  \begin{tabular}[c]{@{}l@{}}Propose instance-sensitive score maps;\\ Apply \textit{hole algorithm}\cite{chen2014semantic} to VGGNet;\\ Use  Local coherence to simplify the \\ complexity.\end{tabular} \\ \hline
YOLACT (2019)s\cite{bolya2019yolact} &
  \begin{tabular}[c]{@{}l@{}}MS COCO 2017\\ PASCAL VOC 2012\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}29.9\%(AP)@33fps\\ 72.3\%(AP^{50}), 56.2\%(AP^{70})@47.6fps\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Divide the tasks into non-local prototype \\ masks generation and instance-wise \\ mask coefficients prediction\end{tabular} \\ \hline
YOLACT++(2020)s\cite{bolya2019yolact++} &
  \begin{tabular}[c]{@{}l@{}}MS COCO 2017\\ PASCAL VOC 2012\end{tabular} &
  33.5(AP)@34.1fps &
  \begin{tabular}[c]{@{}l@{}}Add re-scoring branch;\\ Add DCN to speed up;\\ Try different anchor aspect ratio and scales\end{tabular} \\ \hline
SOLO (2019)\cite{wang2019solo} &
  MS COCO &
  \begin{tabular}[c]{@{}l@{}}37.1(AP)@10.4fps\\ 34.2(AP)@22.5fps (light-weight)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Propose instance category;\\ Only needs to perform two pixel-level \\ classification problem; \\ Global mask representation\end{tabular} \\ \hline
SOLOv2 (2020)\cite{wang2020solov2} &
  MS COCO &
  \begin{tabular}[c]{@{}l@{}}38.8(AP)@18fps\\ 37.1\%(AP)@31.3fps (light-weight)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Improve SOLO by mask learning and\\  \textit{matrix NMS}.\end{tabular} \\ \hline
TensorMask (2019)\cite{chen2019tensormask} &
  MS COCO &
  37.1\% (AP)@0.38s/image &
  \begin{tabular}[c]{@{}l@{}}Represent masks by multi-scale \\ structured high-dimensional(4D) tensors;\\ Scale-adaptive sizes are implemented\\  by Bipyramid structure.\end{tabular} \\ \hline
PolarMask (2020) \cite{xie2020polarmask}&
  MS COCO &
  32.1\% (AP)@12.3fps &
  \begin{tabular}[c]{@{}l@{}}Introduces contour representation\\  in the Polar coordinates;\\ The complexity is close to a \\ single-shot objector.\end{tabular} \\ \hline
BlendMask (2020)\cite{chen2020blendmask} &
  MS COCO &
  \begin{tabular}[c]{@{}l@{}}41.3\%(AP)@116ms/image\\ 34.5\%(AP)@39.7ms/image (real-time setting)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Combine benefits from both top-down \\ and bottom-up methods.\end{tabular} \\ \hline
CondInst (2020)\cite{tian2020conditional} &
  MS COCO &
  35.4\%(AP)@49ms/image &
  \begin{tabular}[c]{@{}l@{}}No need for RoI cropping and \\ feature alignment;\\ mask FCN network parameters are \\ dynamically-generated;\\ Mask prediction heads are compact.\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Differences between some state-of-the-art methods. The data of 'Performance' is provided by its corresponding papers. Since test it by different GPU conditions, the numbers are for reference only.}
\label{tab:Instance segementation}
\end{table*}

==> safety.tex <==
\section{Safety Metrics } \label{sec:safety-metrics}
%\xc{Jeffrey reorganize this section. His comments are in the following}
\begin{comment}


An essential objective of driving safety analysis is extracting \textit{safety metrics}, which are quantifiable measures extracted from traffic videos (or other data sources) that determine the relative risk of an event that may lead to a crash. Here, we review key safety metrics that have been broadly used for driving safety analysis. It is notable that many algorithms developed for AVs utilize safety metrics for safe navigation decisions and avoiding crashes; however, we consider both self-driving and human-driven vehicles.
%the amount of risk into running to a crash between involving vehicles

A recent paper \cite{mahmud2017application} summarizes safety metrics according to different basis (temporal, distance, and deceleration). A more recent paper provides a more updated list of safety metrics for ADS-equipped vehicles \cite{wishart2020driving}. Two important aspects are considered in this review. First, we propose additional safety metrics for network-level analysis \ar{\cite{wishart2020driving}?}\xc{This work stills focus on only involved vehicles, and doesn't propose any metric for network-level analysis}. Secondly, safety metrics are typically calculated by processing the visual information from the AV's perspective, while we also consider extracting safety features from an external observer's point of view. For example, we consider integrative processing of roadside and aerial traffic videos.  


First, let us review the widely used basic safety metrics of (i) temporal-based indicators: Time to Collision (TTC), Extended Time to Collision (Time Exposed Time-to-Collision(TET), Time Integrated Time-to-Collision(TIT)\cite{minderhoud2001extended}), Modified TTC (MTTC), Crash Index (CI), Time-to-Accident (TA), Time Headway (H), and Post-Encroachment Time (PET); (ii) distance-based indicators: Potential Index for Collision with Urgent Deceleration (PICUD), Proportion of stopping Distance (PSD), Margin to Collision (MTC), Difference of Space Distance and Stopping Distance (DSS), Time Integrated DSS (TIDSS), and Unsafe Density (UD); (iii) deceleration-based indicators: Deceleration Rate to Avoid a Crash (DRAC), Crash Potential Index(CPI), and Criticality Index Function (CIF). 

Our main references include \cite{gettman2003surrogate}, \cite{mahmud2017application} and \cite{wishart2020driving}. 

We also mention the approach an observer system takes to monitor video and extract safety metrics. The observer system also called \textbf{system} in the rest of this paper for convenience, is a terrestrial or aerial monitoring system that collects traffic video for processing from an external observer's point of view. 
A list of these metrics, along with their brief descriptions, is presented in Table \ref{tab:metrics}.

\end{comment}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}


%\begin{figure}[htbp]
%\begin{center}
%\centerline{\includegraphics[width=0.8\columnwidth]{figures/human-driven metrics.png}}
%\caption{Related metrics on a conflict point.Source from \cite{gettman2003surrogate}}
%\label{fig:safety metircs}
%\end{center}
%\end{figure}






%\section{Operational Safety Metrics}\label{Jeffrey comment}
An essential objective of driving safety analysis is extracting \textit{operational safety metrics}, which are quantifiable measures extracted from traffic videos (or other data sources) that determine the relative risk of an event that may lead to a crash. 

In this section, we review key safety metrics that have been broadly used for driving safety analysis. 
%A recent paper \cite{mahmud2017application} summarizes safety metrics according to different basis (temporal, distance, and deceleration). A more recent paper provides a more updated list of safety metrics for ADS-equipped vehicles \cite{wishart2020driving}. 
%Razi added
Three new aspects are considered in our review review. First, we propose additional safety metrics for network-level analysis. Secondly, we consider both AVs and human-driven vehicles, in contrast to some work that focus only on one class of vehicles. Thirdly, we consider extracting and processing safety metrics from an external observer's point of view, such as a roadside infrastructure, or an aerial traffic monitoring system.  
A recent paper \cite{mahmud2017application} summarizes safety metrics according to different basis (temporal, distance, and deceleration):
\begin{enumerate}[i]
  \item \textbf{Temporal-based indicators:} Time to Collision (TTC), Extended Time to Collision (Time Exposed Time-to-Collision(TET), Time Integrated Time-to-Collision(TIT)\cite{minderhoud2001extended}), Modified TTC (MTTC), Crash Index (CI), Time-to-Accident (TA), Time Headway (H), and Post-Encroachment Time (PET). 
  \item \textbf{Distance-based indicators:} Potential Index for Collision with Urgent Deceleration (PICUD), Proportion of stopping Distance (PSD), Margin to Collision (MTC), Difference of Space Distance and Stopping Distance (DSS), Time Integrated DSS (TIDSS), and Unsafe Density (UD);
  \item \textbf{Deceleration-based indicators:} Deceleration Rate to Avoid a Crash (DRAC), Crash Potential Index(CPI), and Criticality Index Function (CIF).
\end{enumerate}

A more recent paper \cite{wishart2020driving} by the safety metric team of the Institute of Automated Mobility (IAM), whose project leader is the co-author of our paper, provides a comprehensive set of operational safety metrics following an extensive literature review. The objective was to develop a set of metrics for both human-driven and AVs that includes existing, adapted, and novel metrics. In a follow-up paper\cite{elli2021evaluation}, the IAM proposed a taxonomy for operational safety metrics that is explored and expanded upon here. The IAM work is also a component of an Information Report being developed by the SAE Verification and Validation (V\&V) Task Force under the On-Road Automated Driving (ORAD) Committee\cite{OSM2020}. The taxonomy will be introduced first, and then selected operational safety metrics will be discussed (including the metrics from \cite{mahmud2017application} listed above).

\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=0.9\columnwidth]{figures/taxonomy_2.jpg}}
\caption{Operational safety metrics taxonomy proposed by the IAM.}
\label{fig:taxonomy}
\end{center}
\end{figure}





The expanded taxonomy introduced here is shown in Figure.\ref{fig:taxonomy}. The highest taxonomic rank in the proposed taxonomy hierarchy consists of three types that are based, essentially, on the data source, which includes the level of access required of ADS data. This access to proprietary data could be challenging, depending on the implementation of the operational safety metric; it should be noted that “lighter” metrics require more cooperation with the AV developer. The three types are (example metrics are given for each, and are described in more detail later in the section):
\begin{enumerate}
\item \textbf{Black Box Metric:} A metric that allows measurement of data that can be obtained without requiring any access to ADS data. This could be from an on-board or off-board source. ADS data may enhance the accuracy and precision of the measurement(s).
EXAMPLE: Proper Response Action (PRA).

\item \textbf{Grey Box Metric:} A metric that allows measurement of data that can only be obtained with limited access to ADS data.
EXAMPLE: ADS DDT Execution (ADE).

\item \textbf{White Box Metric:} A metric that allows measurement of data that can only be obtained with significant access to ADS data.
EXAMPLE: Perception Precision (PP).
\end{enumerate}

The second rank in the taxonomic hierarchy is the classification rank, which consists of the following (again, an example metric that is described later in the section is included):
\begin{enumerate}
\item\textbf{Safety Envelope Metric:} A metric that allows for measurement of the subject vehicle’s maintenance of a safe boundary around itself. This includes situations that may not be within the subject vehicle’s control.
		EXAMPLE: Rear End Collision Incident (RECI).
\item\textbf{Behavioral Metric:} A metric that allows for measurement of an improper behavior of the subject vehicle.
EXAMPLE: Aggressive Driving (AD).
	
\item\textbf{Component Metric:} A metric that allows for measurement of the proper function of ADS components.
EXAMPLE: Event Data Recorder Compliance (EDRC).
	
\item\textbf{Sensing Metric:} A metric that allows for measurement of the ability of the ADS sensors to receive adequate information from the AV environment.
EXAMPLE: Camera Resolution (CR).
	
\item\textbf{Perception Metric:} A metric that allows for measurement of the ability of the ADS to interpret information about the AV environment obtained by the ADS sensors.
EXAMPLE: Human Traffic Control Detection Error Rate (HTCDER).
	
\item\textbf{Planning Metric:} A metric that allows for measurement of the ability of the ADS to plan an appropriate route through the AV environment.
EXAMPLE: Object Avoidance Plan Error (OAPE).
	
\item\textbf{Control Metric:} A metric that allows for measurement of the ability of the AV to execute the planned route devised by the ADS.
EXAMPLE: Actuation Error (AE).

\end{enumerate}

It is important to note that not all classification rank types link to data source rank types in the current version. For example, the Component Metric is not linked to the Black Box Metric because data at the component level is deemed to be more access to (potentially proprietary) data than is allowed for the Black Box Metric.

The metrics currently being considered for inclusion in the SAE J3237 Information Report\footnote{This SAE standards document is currently in development and the operational safety metrics list could be modified, expanded, or contracted. In particular, additional White Box metrics are currently being considered.} include in Table \ref{tab:taxonomy}. The IAM has focused on Black Box Metrics and Grey Box Metrics as part of the comprehensive set introduced in \cite{mahmud2017application}.\\
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{0.8\textwidth}{!}{
\centering%
\begin{tabular}{|l|c|c|}
\hline\rowcolor{gray} 
\multicolumn{1}{|c|}{\textbf{Metric Name}}               & \textbf{\begin{tabular}[c]{@{}c@{}}Data \\ Source \\ Taxonomy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Classification\\  Taxonomy\end{tabular}} \\ \hline
Minimum Safe Distance Violation (MSDV)                   & Black                                                                       & Safety Envelope                                                             \\
Proper Response Action (PRA)                             & Black                                                                       & Safety Envelope                                                             \\
Minimum Safe Distance Factor (MSDF)                      & Black                                                                       & Safety Envelope                                                             \\
Time-to-Collision (TTC)                                  & Black                                                                       & Safety Envelope                                                             \\
Modified Time-to-Collision (MTTC)                        & Black                                                                       & Safety Envelope                                                             \\
Time Headway (TH)                                        & Black                                                                       & Safety Envelope                                                             \\
Instantaneous Safety Metric (ISM)                        & Black                                                                       & Safety Envelope                                                             \\
Collision Avoidance Capability (CAC)                     & Black                                                                       & Safety Envelope                                                             \\
Minimum Safe Distance Infringement (MSDI)                & Black                                                                       & Safety Envelope                                                             \\
Post-Encroachment Time (PET)                             & Black                                                                       & Safety Envelope                                                             \\
Not-at-Fault Collision Incident (NAFCI)                  & Black                                                                       & Safety Envelope                                                             \\
Rear-End Collision Incident (RECI)                       & Black                                                                       & Safety Envelope                                                             \\
Deceleration Rate to Avoid the Crash (DRAC)              & Black                                                                       & Safety Envelope                                                             \\
Difference of Space Distance and Stopping Distance (DSS) & Black                                                                       & Safety Envelope                                                             \\
Maximum Speed (MaxS)                                     & Black                                                                       & Behavioral                                                                  \\
Delta Velocity ($\Delta$V)                                      & Black                                                                       & Behavioral                                                                  \\
Traffic Law Violation (TLV)                        & Black                                                                       & Behavioral                                                                  \\
Evasive Action (EA)                                      & Black                                                                       & Behavioral                                                                  \\
Aggressive Driving (AD)                                  & Black                                                                       & Behavioral                                                                  \\
Collision Incident (CI)                                  & Black                                                                       & Behavioral                                                                  \\ \hline
ADS DDT Execution (ADE)                                  & Grey                                                                        & Control                                                                     \\
Achieved Behavioral Competency (ABC)                     & Grey                                                                        & Planning                                                                  \\
Human Traffic Control Perception Error Rate (HTCDER)     & Grey                                                                        & Perception                                                                  \\
Human Traffic Control Violation Rate (HTCVR)             & Grey                                                                        & Behavioral                                                                  \\
Minimum Safe Distance Calculation Error (MSDCE)          & Grey                                                                        & Perception                                                                  \\
Safety-Related Component Failure Perception (SRCFD)      & Grey                                                                        & Component                                                                   \\
Event Data Recorder Compliance (EDRC)                    & Grey                                                                        & Component                                                                   \\ \hline
Perception Precision (PP)                                & White                                                                       & Perception                                                                  \\
Perception Perception Rate (PDR)                         & White                                                                       & Perception                                                                  \\
Perception Weighted Harmonic Mean (PWHM)                 & White                                                                       & Perception                                                                  \\
Perception False Positive Rate (PFPR)                    & White                                                                       & Perception                                                                  \\
Perception False Negative Rate (PFNR)                    & White                                                                       & Perception                                                                  \\
Anomaly Perception Behavior (ADB)                        & White                                                                       & Perception                                                                  \\
Multiple Object Perception Error Rate (MODER)            & White                                                                       & Perception                                                                  \\
Localization Error (LE)                                  & White                                                                       & Perception                                                                  \\
Multiple Object Tracking Precision (MOTP)                & White                                                                       & Perception                                                                  \\
Data Conflict Perception Rate (DCDR)                     & White                                                                       & Perception                                                                  \\
Intersection over Union (IoU)                            & White                                                                       & Perception                                                                  \\
Actuation Error (AE)                                     & White                                                                       & Control                                                                   \\
Software Execution Error (SEE)                           & White                                                                       & Component                                                                   \\
Object Avoidance Plan Error (OAPE)                       & White                                                                       & Planning       \\\hline                                                            
\end{tabular}%
}
\caption{Current SAE J3237 Information Report operational safety metrics.}
\label{tab:taxonomy}
\end{table*}
\indent We also mention the approach an observer system takes to monitor video and extract safety metrics. The observer system also called system in the rest of this paper for convenience, is a terrestrial or aerial monitoring system that collects traffic video for processing from an external observer’s point of view. A list of these metrics, along with their brief descriptions, is presented in Table \ref{tab:metrics}. 

Our main references include \cite{gettman2003surrogate}, \cite{mahmud2017application} and \cite{wishart2020driving}. 
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline\rowcolor{gray} 
\textbf{Metric}     & \textbf{Definition} & \textbf{Features}                                                                                                                         \\ \hline
MaxS       & $\max v$         & A simple but effective measure of the severity of a collision.                                                                   \\ \hline
$\Delta v$    & $\Delta v$          & An effective indicator of the severity of a collision.                                                                           \\ \hline
TTC &
  $TTC =\frac{X_L-X_F}{v_F-v_L}$ &
  \begin{tabular}[c]{@{}l@{}}Provides more information than PET; assumes that involved vehicles are at a constant speed;\\ cannot reflect the severity.\end{tabular} \\ \hline
PET &
  $PET =t_2-t_1$ &
  \begin{tabular}[c]{@{}l@{}}Can be easily captured and computed; suitable for assessing intersecting conflicts; \\ only suitable for the cases of transversal trajectories;\\ cannot reflect the severity.\end{tabular} \\ \hline
Initial DR & $DR_{t=0}$          & A basic indicator; cannot consider the following vehicle's acceleration/deceleration.                                                        \\ \hline
DRAC       &$TTC =\frac{(v_F-v_L)^2}{X_L-X_F}$         & \begin{tabular}[c]{@{}l@{}}No need to directly observe the deceleration rate; \\ does not work for lateral movement\end{tabular}      \\ \hline
CPI        & $CPI_i=\frac{\sum_{t=t_i}^{tf_i}P(DRAC_{i,t})\geq MADR\Delta t\cdot b}{T_i}$          & Considers more factors such as traffic and road conditions compared to DRAC;                                                         \\ \hline
PSD        &\begin{tabular}[c]{@{}l@{}}$PSD =\frac{RD}{MSD}$;\\ $ PSD =\frac{v^2}{2MADR} $ \end{tabular}      & \begin{tabular}[c]{@{}l@{}}Works for a conflict with a single vehicle involved; \\ \rarely used for specific safety problems.\end{tabular} \\ \hline
UD &
  $UD=\frac{\sum_{S=1}^{S_t}\sum_{V=1}^{V_t}unsafety_{V,S}\cdot d}{TL}$ &
  \begin{tabular}[c]{@{}l@{}} Delivers more accurate information than typical micro-simulation outputs;\\ allows comparison between simulation scenarios or links;\\ some parameters are difficult to capture automatically;\\ only applicable to identical trajectories.\end{tabular} \\ \hline
  
  MSDV &
  \begin{tabular}[c]{@{}l@{}}Indicate the subject vehicle violate safety boundary of another.\\ Safety boundary: $d_{min}^{long,same}$(Eq.\ref{eq:d_long_same}) $d_{min}^{long,opp}$(Eq.\ref{eq:d_long_opp}) and $d_{min}^{lat}$(Eq.\ref{eq:d_lat})\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Provides how to calculate the quantified risky distances;\\ a basis of many assessment methods.\end{tabular} \\ \hline
PRA &
  \begin{tabular}[c]{@{}l@{}}An action to recover when\\ $d_{min}^{long},d_{min}^{lat}$ and the safe range of $a^{lat}$,$a^{long}$ are violated\end{tabular} &
  Adds more information beyond MSDV. \\ \hline
MSDF &
  \begin{tabular}[c]{@{}l@{}}$MSDF^{lat} = \frac{d^{lat}}{d^{lat}_{min}}$\\ $MSDF^{long} = \frac{d^{long}}{d^{long}_{min}}$\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Can indicate the degree of defensive driving style;\\ a higher $MSDF$ may not means higher safety.\end{tabular} \\ \hline
MSDCE &
  $MSDCE = \sqrt{\frac{\vert d^{long}_{gt,min} - d^{long}_{min}\vert }{d^{long}_{gt,min}}+\frac{\vert d^{lat}_{gt,min} - d^{lat}_{min}\vert }{d^{lat}_{gt,min}}}$ &
  Indicate the ADS ability to determine the safety distances. \\ \hline
CI &
  \begin{tabular}[c]{@{}l@{}}Indicate the subject vehicle is involved in a collision.\\ Active when $d^{lat}$ and $d^{long}$ are equal to 0.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Capture instances of collisions as a metric;\\ the severity of the collision can be defined by KABCO scale\cite{herbel2010highway}:\\
  K(Fatal Injury), A(Incapacitating Injury), B (Non-Incapacitating Injury),\\ C(Possible Injury), O(No Injury).\end{tabular} \\ \hline
TLV &
  Indicate the subject vehicle that violates a traffic law &
  \begin{tabular}[c]{@{}l@{}}Emphasizes that an ADS vehicle must follow existing laws;\\ exceptions are made, for example, when road closures \\ require temporary violations of driving exclusively inside a traffic lane.\end{tabular} \\ \hline
ABC &
  Indicate the subject vehicle can execute a specific behavior correctly. &
  \begin{tabular}[c]{@{}l@{}}Indicate the safety of ADS;\\ included in the preliminary list of metrics.\end{tabular} \\ \hline
ADSA &
  Indicate the ADS is active when executing behaviors. &
  \begin{tabular}[c]{@{}l@{}}Indicate the safety of ADS;\\ included in the preliminary list of metrics;has some dispute in California\cite{hawkins2019california}.\end{tabular} \\ \hline
HTCDER &
  $HTCDER = \frac{GTI-CDI}{CDI}$ &
  \begin{tabular}[c]{@{}l@{}}One of HTC measurements;\\ manually instructions by officers should still be considered.\end{tabular} \\ \hline
HTCVR &
  $HTCVR = \frac{CDI-CCI}{CDI}$ &
  \begin{tabular}[c]{@{}l@{}}One of HTC measurements;\\ manually instructions by officers should still be considered.\end{tabular} \\ \hline
  
AD &
  \begin{tabular}[c]{@{}l@{}}Indicate the maneuvers (longitudinal/lateral accelerations) \\ of a subject vehicle exceeds specified thresholds.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}The thresholds vary by jurisdiction and culture;\\ AD is only involved the subject vehicle;\\ implies the inherent and potential risks of natural driving behaviors;\\ should be included when evaluating ADS.\end{tabular} \\ \hline  
  
  
\end{tabular}%
}
\caption{%Some broadly-used safety metrics along with their key properties.\xc{
Summary of operational safety metrics along with their key properties.}
\label{tab:metrics}
\end{table*}


\subsection{Summary of Basic Operational Safety Metrics}

~~~\textbf{Maximum Speed (MaxS)}, when associated with a collision, denotes the maximum speed of the involved vehicles before the crash starts until the full stop (e.g., between time points $t_1$ and $t_4$ in Fig.\ref{fig:safety metircs} 
%\arr{update all time epochs according to the new figures: we have no t5 in the new figure}). 
MaxS is a simple but effective measure directly related to the severity of the collision.


\textbf{Differential Speed ($\Delta s$)} is defined as the relative speed between the involved vehicles. It occurs at $t_2$ in Fig.\ref{fig:safety metircs}.
The system needs to calculate the speed of the involved vehicles (using methods like DL-based object tracking with or without explicitly extracting the motion trajectories) to determine MaxS and $Delta s$.
\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=0.9\columnwidth]{figures/mymetric2.png}}
\caption{The space-speed pair diagram of a rear-end collision. $t_1$ is the time epoch the leading vehicle begins to decelerate (encroachment begin). $t_2$ is the epoch the following vehicle begins to decelerate. $t_1$-$t_2$ is the reaction time of the driver of the following vehicle. $t_3$ is the projected arrival moment of the following vehicle (under no deceleration). $t_4$ is the actual collision moment.}
\label{fig:safety metircs}
\end{center}
\end{figure}

\textbf{Time to Collision (TTC)} is a commonly used surrogate measure to define the time of an upcoming rear-end collision between two vehicles, if they continue their current speed ($t_2$-$t_3$  in Fig. \ref{fig:safety metircs}). The system needs to observe the relative position and calculate the relative velocity of the two involved vehicles. 
TTC is computed as:
\begin{align}
\label{eq:TTC}
    TTC =\frac{X_L-X_F}{v_F-v_L},
\end{align}
where $X_i$ denotes the position, $v_i$ denotes the velocity, and the indexes $L$ and $F$, respectively, denote the leading and following vehicles. The collision occurs only if $v_F\geq v_L$. Usually, we have $v_L \geq 0$ assuming that the cars move in the same direction. $v_L \leq 0$ represents a vehicle approaching from the front. The severity of an encounter can be determined by the minimum TTC (TTCmin). 
Although very useful in investigating crashes, this metric has some limitations. First, TTC assumes that involved vehicles are moving at constant speeds, which ignores the potential dangers caused by acceleration or deceleration. Secondly, it assumes that the cars drive in the same direction and not appropriate for side crashes. 




\textbf{Post-Encroachment Time (PET)} is defined as the time span between the encroached vehicle leaving and the other vehicle with the right-of-way arriving at the conflict point. The system needs to observe the relative time of the involved vehicles and estimate the conflict point. 
PET in Fig.\ref{fig:PET} is computed as:
\begin{align}
\label{eq:PET}
    PET =t_b-t_a,  
\end{align}
where $t_a$ and $t_b$ represent the arrival time of the two involved vehicles. 
PET can be easily captured and computed by the system. However, it is suitable for intersection conflicts with transversal trajectories, but it does not fully reflect the severity of the crash. 

\begin{figure}[]
\begin{center}
\centerline{\includegraphics[width=1\columnwidth]{figures/PET1.png}}
\caption{The schematic diagram of PET.}
\label{fig:PET}
\end{center}
\end{figure}



\textbf{Initial Deceleration Rate (Initial DR)} quantifies the avoidance behavior taken by a vehicle to avoid a collision. More specifically, Initial DR (the second derivative of Curve B at time point $t2$ in Fig.\ref{fig:safety metircs}) is defined as the deceleration rate $a_0$ at the beginning of the decelerating state. Deceleration rate is an appreciated variable to assess the potential severity of a conflict. Other variants of this metric family include Deceleration Rate to Avoid a Crash (DRAC), Crash Potential Index (CPI), and Criticality Index Function (CIF). 

\textbf{Deceleration Rate to Avoid a Crash (DRAC)} is defined as the minimum deceleration rate of the following vehicle to avoid a crash to the leading vehicle. 
To characterize this metric, the observer system should keep track of the relative positions and the relative velocities of the two vehicles. Note that DRAC fails to evaluate lateral movements and is applicable only to scenarios where both cars are on the same lane. Mathematically, DRAC is defined as 
\begin{align}
\label{eq:DRAC}
    DRAC =\frac{(v_F-v_L)^2}{X_L-X_F}. 
\end{align}


\textbf{Crash Potential Index (CPI)} is defined as the probability of DRAC exceeding the Maximum Available Deceleration Rate (MADR) at any moment. 
%\arr{Clarify: at any moment? or at the current moment?}\xc{Like the equation shown, the moment means the observation time step. CPI is considered the total time interval }. 
MADR depends on the type of the vehicle as well as the environmental conditions. The system needs to calculate MADR of the target vehicles and instantaneous track time-variant deceleration to obtain the %for safety analysis and 
crash likelihood. CPI is defined as 
\begin{align}
    CPI_i=\frac{\sum_{t=t_i}^{tf_i}P(DRAC_{i,t})\geq MADR ~\Delta t\cdot b}{T_i},
\end{align}
where $t_i$ and $tf_i$ are the initial and final time intervals of vehicle $i$, respectively, $T_i$ denotes the total travel time of vehicle $i$, $\Delta t$ is the observation time step, and $b$ is a binary state variable with $b=1$ for active state and $b=0$ for inactive state. Compared with DRAC, CPI considers more factors such as the traffic and road conditions, but it is not yet suitable for assessing lateral movements.




%Wrong notation: \textbf{Proportion of Stopping Distance (PSD)} is defined as the ratio of the remaining distance (RD) from the current position to the potential collision point to the acceptable minimum stopping distance (MSD). 
\textbf{Proportion of Stopping Distance (PSD)} is defined as the ratio of the Remaining Distance (RD) from the current position to the potential collision point to the acceptable Minimum Stopping Distance (MSD).
It can be stated as
\begin{align}
\label{eq:PSD}
    PSD =\frac{RD}{MSD}.
\end{align}



%Noting that here, MSD is under the assumption of maximum deceleration, we can write MSD as:
If MSD is considered under maximum deceleration, then PSD becomes:
\begin{align}
\label{eq:MSD}
    PSD =\frac{v^2}{2 MADR}.
\end{align}

PSD is an easily observable indicator and is one of the few metrics that can be used for a conflict involving a single vehicle (e.g., crashing into a stationary obstacle like a tree). PSD is defined for evasive actions and usable only for specific safety problems.




\textbf{Unsafe Density (UD)} is defined as the severity of the potential crash when the leading vehicle is within the achievable maximum DR. This metric is introduced in \cite{torday2003indicator}. When multiple cars involved, this metric considers all cars in a link, while the similar metric of UnSafety (UNS) considers only two of the cars from the link to calculate the $UNS$ of car $v$ at time step $s$, denoted by $UNS_{v,s}$. 

According to \cite{torday2003indicator}, the severity of a read-end crash is proportional to $\Delta v$, and $v_F$. %, and but $R_d$ can be obtained, so multiply the ratio $R_d$. 
More specifically, UNS is defined as:
\begin{align}
    UNS = \Delta v\cdot v_F\cdot R_d,
\end{align}
where $R_d$ denotes the ratio between the deceleration of the leading vehicle and its maximum deceleration capacity, namely
\begin{equation}
    R_d=
\begin{cases}
b/b_{max}& \text{b<0}\\
0& \text{else}
\end{cases}.
\end{equation}
Then, UD can be written as:
\begin{align}
    UD=\frac{\sum_{S=1}^{S_t}\sum_{V=1}^{V_t} UNS_{V,S}\cdot d}{TL},
\end{align}
where $S_t$ denotes the number of simulation steps within the aggregation period, $V_t$ denotes the number of vehicles in the link, $d$ denotes the time span between the two simulation steps, $T$ denotes the aggregation period, and $L$ denotes the section length for which the metrics are evaluated. 

UD provides more accurate information than typical micro-simulation outputs and allows comparison between the simulation scenarios or links. In a transportation network, each intersection is considered as a node, and the traffic flow between the nodes is represented by a link. 
%For limitation, some parameters of UD are difficult to be captured automatically, and it is only applicable for identical trajectory.
The two limitations of the UD parameter include (i) the difficulty of quantifying its constituent parameters and (ii) its applicability only to identical trajectories, namely when two cars move in the same direction, and the type of the potential crash is rear-end collision.

\subsection{Operational safety metric for ADS proposed by the IAM} 
%revised by Razi
Here, we review part of the recently proposed metrics by the IAM \cite{wishart2020driving}. These metrics are developed by a team whose leader is a co-author of this paper. 

\textbf{Minimum Safe Distance Violation (MSDV)} is defined to indicate that the subject vehicle violates the safety envelope of another entity (often is another vehicle). When the subject vehicle (subscript 1) is following behind another entity (subscript 2) and both of them are moving in the same direction. The longitudinal boundary can be defined as:
\begin{align}\label{eq:d_long_same}
    d_{min}^{long,same} &= v_1^{long}\rho_1+\frac{1}{2}a_{1,max,acc}^{long}\rho_1^2\\\nonumber
    &+ \frac{(v_1^{long}+a_{1,max,acc}^{long}\rho_1)^2}{2a_{2,min,dec}^{long}}\\\nonumber
    &-\frac{(v_2^{long})^2}{2a_{2,max,dec}^{long}},
\end{align}
where $v_i^{long/lat}$ denotes the current longitudinal/lateral velocity of  vehicle $i$, $a_{i,max/min,acc/dec}^{long/lat}$ denotes the longitudinal/lateral maximum/minimum acceleration/deceleration of vehicle $i$, and $\rho_i$ denotes the response time of vehicle $i$. 
When two involved vehicles are moving in opposite directions towards each other, the longitudinal boundary can be defined as: 
\begin{align}\label{eq:d_long_opp}
    d_{min}^{long,opp} =& v_1^{long}\rho_1+\frac{1}{2}a_{1,max,acc}^{long}\rho_1^2\\ \nonumber
    +& \frac{(v_1^{long}+a_{1,max,acc}^{long}\rho_1)^2}{2a_{1,min,dec}^{long}}\\ \nonumber
    +& \vert v_2^{long}\vert\rho_2+\frac{1}{2}a_{2,max,acc}^{long}\rho_2^2\\\nonumber
    +& \frac{(\vert v_2^{long}\vert+a_{2,max,acc}^{long}\rho_2)^2}{2a_{2,min,dec}^{long}}
\end{align}
The lateral boundary can be defined as:
\begin{align}\label{eq:d_lat}
    d_{min}^{lat} = \mu+ & v_1^{lat}\rho_1+\frac{1}{2}a_{1,max,acc}^{lat}\rho_1^2\\\nonumber
    +& \frac{(v_1^{lat}+a_{1,max,acc}^{lat}\rho_1)^2}{2a_{1,min,dec}^{lat}} \\\nonumber
    - & [v_2^{lat}\rho_2-\frac{1}{2}a^{lat}_{2,max,acc}\rho_2^2\\\nonumber
    -& \frac{(v_2^{lat}-\rho_2 a_{2,max,acc}^{lat})^2}{2a_{2,min,dec}^{lat}} ],
\end{align}
where $\mu$ is the lateral fluctuation margin. 
Noting that if the calculated result of $d_{min}^{long,same}$ or $d_{min}^{lat}$ is negative, it should be rounded up to 0. 
While the two boundaries are violated by the subject vehicle, MSDV is active ($MSDV=1$), meaning that %the binary status of the metric is equal to 1), which means 
an avoidable accident may occur. This metric characterizes the quantified risky distances as the basis of many assessment methods.

\textbf{Proper Response Action (PRA)} is defined to indicate a proper action taken by the subject vehicle to recover itself when safety boundaries ($d_{min}^{long},d_{min}^{lat}$ and the safe range of $a^{lat}$,$a^{long}$) are violated. It adds more information beyond MSDV to evaluate the driving safety of the subject vehicle.  

\textbf{Minimum Safe Distance Factor (MSDF)} is defined as the ratio between the current distance[s] to the calculated safe boundaries from the surrounding entity.
It can be found as:
\begin{align}
    &MSDF^{lat}& = \frac{d^{lat}}{d^{lat}_{min}}, &  MSDF^{long}& = \frac{d^{long}}{d^{long}_{min}},
\end{align}
where $d^{lat}$ and $d^{long}$ denote the measured distances. $MSDF\geq 1$ indicates the degree of defensive driving style. Note that a higher $MSDF$ may not mean a higher safety, necessarily.

\textbf{Minimum Safe Distance Calculation Error (MSDCE)} is defined as the difference between the calculated results by ADS from the ground truth. It can be formulated as:
\begin{align}
    MSDCE = \sqrt{\frac{\vert d^{long}_{gt,min} - d^{long}_{min}\vert }{d^{long}_{gt,min}}+\frac{\vert d^{lat}_{gt,min} - d^{lat}_{min}\vert }{d^{lat}_{gt,min}}}
\end{align}

This metric is derived from the MSDV, which indicates the ADS ability to determine the safety distances.

\textbf{Collision Incident (CI)} is defined to indicate the subject vehicle is involved in a collision determined by the reasonably related data. CI is active when $d^{lat}$ and $d^{long}$ are equal to 0. Also, the severity of the collision can be defined by KABCO scale\cite{herbel2010highway} with K(Fatal Injury), A(Incapacitating Injury), B (Non-Incapacitating Injury), C(Possible Injury), O(No Injury). 

\textbf{Traffic Law Violation (TLV)} is defined to indicate the subject vehicle that violates a traffic law which would result in an infraction or citation. Violating these laws sets TLV active. This metric emphasizes that an ADS-vehicle must follow existing laws, and an active TLV may lead to severe safety issues. It should be noted that exceptions to a TLV are made, for example, when road closures require temporary violations of driving exclusively inside a traffic lane.

\textbf{Achieved Behavioral Competency (ABC)} is defined to indicate the subject vehicle can execute a specific behavior correctly. This metric indicates the safety of ADS and is included in the preliminary list of ADS vehicles' metrics.

\textbf{ADS Active (ADSA)} is defined to indicate that the ADS is active when executing behaviors. This metric represents the safety of ADS and is included in the preliminary list of ADS vehicles' metrics. The metric has some dispute in California\cite{hawkins2019california}.

\textbf{Human Traffic Control Detection Error Rate (HTCDER)} is defined as the capability to detect instructions from a Human Traffic Control (HTC) actor correctly. It is calculated as:
\begin{align}
    HTCDER = \frac{GTI-CDI}{CDI},
\end{align}
where $GTI$ is the number of ground truth instructions, and $CDI$ is the number of correctly detected instructions. This metric is one of the HTC measurements to evaluate the safety of the subject vehicle. Note that the manual instructions by officers should still be considered in this metric.

\textbf{Human Traffic Control Violation Rate (HTCVR)} is defined as the capability of a subject vehicle to follow the received instructions successfully. It is formulated as:
\begin{align}
    HTCVR = \frac{CDI-CCI}{CDI},
\end{align}
where $CCI$ is the number of correctly compiled instructions. %This metric is another HTC measurement and has similar cases to HTCDER. 

\textbf{Aggressive Driving (AD)} is defined to indicate the maneuvers (longitudinal/lateral accelerations) of a subject vehicle exceeding specified thresholds. When exceeding ($a\geq a_T$), the metric is set active. The thresholds vary by jurisdiction and culture. This metric involves only the subject vehicle and implies the inherent and potential risks of natural driving behaviors. When evaluating the safety of ADS, this metric should be included. 


\subsection{Proposed Metrics for Network-level Analysis}

It is clear from the discussion above that most of the metrics are defined for scenarios where only two vehicles are involved. This represents a micro-scale perspective to the safety problem while ignoring the network-level metrics that may contribute to the overall traffic safety. For instance, the composition of traffic (e.g., the ratio of trucks to all vehicles) can contribute to the frequency and severity of collisions. In this paper, we take this approach and offer a set of new metrics that can be used for the overall and long-term safety assessment of traffic flow, especially on %cities and 
highways. These are sample metrics, and we do not claim they are comprehensive by any means. Indeed, we believe that this area needs further investigation. The summary of these metrics is provided in Table.\ref{tab:newmetric}. 


\textbf{Individual Velocity Variation Rate (IVVR)} is defined as the variation of velocities for each vehicle in a specific zone or time interval. We define it as
\begin{align}
    IVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{max}-v_i^{min}|}{v_i^{av}}
\end{align}
where $v_i^{max},v_i^{min},v_i^{av}$ are the minimum, maximum, and average velocities of vehicle $i$. The higher values of this metric means that on average each vehicle changes its speed more often by accelerating and decelerating. This can be due to the road profile, density of intersections and exits, or road conditions. 


\textbf{Overall Velocity Variation Rate (OVVR)} is defined as the variation of average velocities among vehicles in a specific zone or time interval. OVVR is defined as 
\begin{align}
    OVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{av}-v^{av}|}{v^{av}},
\end{align}
where $v_i^{av}$ is the average velocity of vehicle $i$, and $v^{av}=\sum_{i=1}^N{v_i^{av}}/N$ is the average velocity of all vehicles. Similar to IVVR, this metric can be associated with crash rate in specific highway sections.

\textbf{Over Speeding Rate (OSR)} is defined as the rate of over-speeding by vehicles as follows:
\begin{align}
    OSR =\frac{1}{N}\sum_{i=1}^{N} I(v_i^{max} > v_L),
\end{align}

\begin{align}
    OSR_i =\frac{1}{N}\sum_{i=1}^{N} I(v_i^{max}/v_L > Threshold_i),
\end{align}
%\xc{Modified OSR $OSR_i =\frac{1}{N}\sum_{i=1}^{N} I(v_i^{max}/v_L > Threshold_i)$. 
%where $Threshold_i>1$ (e.g.,  Levl 1:$Threshold_1=1.1$, Level2:$Threshold_2=1.2$ ... ) indicates the different level of over-speeding }
where $Threshold_i$ is used to capture different levels of over-speeding.
Here, $v_L$ is the speed limit, and $I(x>y)$ is the indicator function with $I(x>y)=1$ for $x>y$ and $I(x>y)=0$ otherwise.  
Speed limits are typically set based on a standardized set of guidelines and national manuals, taking into account road geometry features such as the radii of curves, sight distance, and weather conditions. A high OSR, when associated with a high crash rate, may indicate the need for taking more warning and prevention measures to avoid over-speeding, noting that over-speeding can be an important contributor to crashes. On the other hand, high OSR, when it does not correlate with a high accident rate, can indicate the need for revising the set speed limits without compromising traffic safety. 

The aforementioned traffic metrics can be characterized by processing the roadside cameras or by crowd-sourcing and accumulating information provided by vehicles' dash cameras.

\textbf{Traffic Composition Indicator (TCI)} is defined to gauge the diversity of vehicle types in specific road sections.  
For instance, it is known that a higher density of trucks on roads can correlate with the frequency and severity of road accidents; hence trucks are prohibited in some road sections in highly-populated areas \cite{meyers1981comparison}. This can be due to trucks' larger deceleration inertia, more frequent break failures, and lower maneuverability levels. In general, if vehicles classified into classes $c=1,2,3,\dots,C$, then the traffic composition can be defined as
\begin{align}
    TCI = \frac{\big(\sum_{c=1}^C N_c)^2}{C\sum_{c=1}^C N_c^2},\\
\end{align}
where $N_c$ is the number of vehicles in class $c$, and the metric is defined similarly to the Jain fairness index. This metric ranges from $1/C$ for the most unbalanced composition to $1$ for an equal number of vehicles from each type. If one is interested in evaluating the rate of a specific class like trucks to all vehicles, the following metric can be used:
\begin{align}
     f_c = \frac{N_c}{\sum_{i=1}^C N_i}.
\end{align}

When classifying cars into two classes $c=1$ for trucks and $c=2$ for non-trucks, these two metrics are related as 
\begin{align}
     TCI = \frac{1}{2(1-2 f_1 f_2)}.
\end{align}

Lower $TCI$ values mean that most cars are of the same type with lower risks. This metric can be estimated by processing roadside videos but requires high-complexity learning methods for vehicle detection and classification. 
 
\textbf{Normalized Traffic Density (NTC)} is defined as the density of vehicles on road sections as 
%  \begin{align}
%      NTC = \frac{N_v}{N_l*L},
%  \end{align}
 
  \begin{align}
     NTC = \frac{\sum l_i/\bar{l}}{N_l*L},
 \end{align}
%\xc{$NTC = \frac{\sum l_i/\bar{l}}{N_l*L},
where  $l_i$ is the length of a vehicle, $\bar{l}$ is the average of all vehicles' length. We normalize the vehicle by its length to capture the effect of vehicle's size. %later we cn check, I am not sure it is necessary to make it this complex?

Here, 
%$N_v$ is the number of vehicles, 
$N_l$ is the number of lanes, and $L$ is the length of the road section. This parameter can be easily captured by video processing and vehicle recognition. Higher NTC values are expected to be associated with higher crash rates, and may raise the request for traffic load balance strategies.  
 
\textbf{Traffic Recovery Time (TRT)} is defined as the time required for traffic flow recovery after accidents. 
The system of vehicular flow can be considered as a non-equilibrium system of interacting particles \cite{sugiyama2008traffic}, and the instability of a flow-free state is induced by the collective effects of the increase of fluctuations. 
It is known that any traffic event can suddenly lead to a jamming state, and TRT reflects the time span from an event epoch to the status change to free flow. This time is expected to be much shorter than the interval between the consecutive events for flow stability. TRT can be defined as:
\begin{align}
    TRT = \frac{1}{N_e}\sum_{i=1}^{N_e} |t_r(i)-t_b(i)|,
\end{align}
where $N_e$ is the number of events in the monitoring interval, and $t_b(i)$ and $t_r(i)$, respectively, denote the event start epoch, and the flow recovery epoch for event $i$. These parameters can be easily captured by roadside videos or fusing information obtained from dash cameras. 
%\arr{update the table accordingly}

The summary of the proposed network-level safety metrics is presented in Table \ref{tab:newmetric}. We believe that this list is not comprehensive by any means and can initiate efforts to develop a more comprehensive list of network-level safety metrics. 




\begin{comment}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[htbp]

\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
Metric &
  Defination &
  Features \\ \hline
IVVR &
  $IVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{max}-v_i^{min}|}{v_i^{av}}$ &
  \begin{tabular}[c]{@{}l@{}} Reflects the instability of traffic flow by car speed variations and crash rate;\\ Can partially offer network re-design suggestions;\end{tabular} \\ \hline
OVVR &
  $OVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{av}-v^{av}|}{v^{av}}$ &
  \begin{tabular}[c]{@{}l@{}}Overall speed variation of vehicles; \\Defined similar to IVVR for overall traffic speed variation;\\ Not easily affected by outliers; \end{tabular}\\ \hline
OSR &
  $OSR =\frac{1}{N}\sum_{i=1}^{N} I(v_i^{max} > v_L)$ &
  \begin{tabular}[c]{@{}l@{}}Indication of speed limit violations; Can offer suggestions for network design;\end{tabular} \\ \hline
TCI &
  \begin{tabular}[c]{@{}l@{}}$TCI = \frac{\big(\sum_{c=1}^C N_c)^2}{C\sum_{c=1}^C N_c^2}$\\ $f_c = \frac{N_c}{\sum_{c=1}^C N_c}$\\ $TCI = \frac{1}{2(1-2 f_1 f_2)}$, two classes\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Flow composition indicator;\\ Can be associated with elevated crash risks\end{tabular} \\ \hline
NTC &
  $NTC = \frac{\sum l_i/\bar{l}}{N_l*L}$ &
  \begin{tabular}[c]{@{}l@{}} Reflects traffic density;\\ Can be associated with elevated crash risks\end{tabular} \\ \hline
TRT &
  $TRT = \frac{1}{N_e}\sum_{i=1}^{N_e} |t_r(i)-t_b(i)|$ &
  \begin{tabular}[c]{@{}l@{}}
  A simple and reasonable way to evaluate severity of the accidents;\\
  Can also take traffic stability into consideration\end{tabular}\\ \hline
\end{tabular}%
}
\caption{A set of proposed network-level safety metrics. }
\label{tab:newmetric}
\end{table}

\end{comment}


\begin{table*}[htbp]

\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline\rowcolor{gray} 
\textbf{Metric} &
  \textbf{Definition} &
  \textbf{Features} \\ \hline
IVVR &
  $IVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{max}-v_i^{min}|}{v_i^{av}}$ &
  \begin{tabular}[c]{@{}l@{}} Reflects the instability of traffic flow by car speed variations and crash rate;\\ Can partially offer network re-design suggestions\end{tabular} \\ \hline
OVVR &
  $OVVR =\frac{1}{N}\sum_{i=1}^{N} \frac{|v_i^{av}-v^{av}|}{v^{av}}$ &
  \begin{tabular}[c]{@{}l@{}}Overall speed variation of vehicles; \\Defined similar to IVVR for overall traffic speed variation;\\ Not easily affected by outliers \end{tabular}\\ \hline
OSR &
  $ OSR_i =\frac{1}{N}\sum_{i=1}^{N} I(v_i^{max}/v_L > Threshold_i)$ &
  \begin{tabular}[c]{@{}l@{}}Indication of speed limit violations; Can offer suggestions for network design\end{tabular} \\ \hline
TCI &
  \begin{tabular}[c]{@{}l@{}}$TCI = \frac{\big(\sum_{c=1}^C N_c)^2}{C\sum_{c=1}^C N_c^2}$\\ $f_c = \frac{N_c}{\sum_{c=1}^C N_c}$\\ $TCI = \frac{1}{2(1-2 f_1 f_2)}$, two classes\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Flow composition indicator;\\ Can be associated with elevated crash risks\end{tabular} \\ \hline
NTC &
  $NTC = \frac{\sum l_i/\bar{l}}{N_l*L}$ &
  \begin{tabular}[c]{@{}l@{}}Consider vehicle shape;\\ Reflects traffic density;\\ Can be associated with elevated crash risks\end{tabular} \\ \hline
TRT &
  $TRT = \frac{1}{N_e}\sum_{i=1}^{N_e} |t_r(i)-t_b(i)|$ &
  \begin{tabular}[c]{@{}l@{}}
  A simple and reasonable way to evaluate severity of the accidents;\\
  Can also take traffic stability into consideration\end{tabular}\\ \hline
\end{tabular}%
}
\caption{A set of proposed network-level safety metrics.} %\xc{modified}}
\label{tab:newmetric}
\end{table*}
%TRT:\ar{of what? potential accidents.} \arr{Is not it more related to the overall stability of traffic in case of crashes? because it does not say what is the risk, rather it says how long it takes to recover and be back to normal conditions after an accident.}
%\xc{TRT: What I think is TRT is more related to the effect brought by crashes, which can be explained by both severity and traffic stability}





==> table.tex <==

\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
Method &
  Dataset &
  Performance(mAP) &
  Features \\ \hline
\multicolumn{4}{|l|}{\textit{One-stage}} \\ \hline
SDS (2014)\cite{hariharan2014simultaneous} &
  \begin{tabular}[c]{@{}l@{}}PASCAL VOC 2011\\ PASCAL VOC 2012\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}52.6\%\\ 51.6\%\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}MCG\cite{arbelaez2014multiscale} to generate proposal;\\ Define Instance Segmentation.\end{tabular} \\ \hline
DeepMask (2015)\cite{pinheiro2015learning} &
  \begin{tabular}[c]{@{}l@{}}PASCAL VOC 2007\\ MS COCO\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}improves Fast R-CNN  to 69.9\%@1.2s/image\\ @1.6s/image\end{tabular} &
  Bottom-up proposals generation. \\ \hline
SharpMask (2016)\cite{pinheiro2016learning} &
  MS COCO 2015 &
  25.1\%(AP), 45.8\%(AP^{50}), 24.8\%(AP^{75}) &
  \begin{tabular}[c]{@{}l@{}}Add top-down refinement network\\  to DeepMask.\end{tabular} \\ \hline
MNC (2016) \cite{dai2016MNC}&
  \begin{tabular}[c]{@{}l@{}}PASCAL VOC 2012\\ MS COCO 2015\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}63.5\% on validation set (mAP@0.5)\\ 29.7\% on test-dev set(mAP@0.5)\\ @360 ms/image\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}New Cascaded multi-task architecture;\\ End to End trainable;\\ No external modules.\end{tabular} \\ \hline
Mask R-CNN (2017)\cite{he2017mask} &
  MS COCO &
  \begin{tabular}[c]{@{}l@{}}37.1\%(AP), 60\%(AP^{50}), 39.4\%(AP^{75})\\ @200ms/frame\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}The extension version of Faster R-CNN;\\ \textit{RoIAlign} can better retain spatial information\end{tabular} \\ \hline
FCIS (2017)\cite{li2017fully} &
  \begin{tabular}[c]{@{}l@{}}PASCAL VOC 2012\\ MS COCO 2016\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}65.7\% (mAP@0.5) and 52.1\% (mAP@0.7) \\ 59.9\%(mAP@0.5) \\ @0.24s/image\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}The extension version of InstanceFCN\\ End to end trainable;\\ Can detect and segment objects jointly \\ and simultaneously; \\ Propose position-sensitive inside/outside \\ score maps.\end{tabular} \\ \hline
\multicolumn{4}{|l|}{\textit{Two-stage}} \\ \hline
InstanceFCN(2016)\cite{dai2016instance} &
  PASCAL VOC 2012 &
  61.5\% (mAP@0.5) and 43.0\% (mAP@0.7) &
  \begin{tabular}[c]{@{}l@{}}Propose instance-sensitive score maps;\\ Apply \textit{hole algorithm}\cite{chen2014semantic} to VGGNet;\\ Use  Local coherence to simplify the \\ complexity.\end{tabular} \\ \hline
YOLACT (2019)s\cite{bolya2019yolact} &
  \begin{tabular}[c]{@{}l@{}}MS COCO 2017\\ PASCAL VOC 2012\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}29.9\%(AP)@33fps\\ 72.3\%(AP^{50}), 56.2\%(AP^{70})@47.6fps\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Divide the tasks into non-local prototype \\ masks generation and instance-wise \\ mask coefficients prediction\end{tabular} \\ \hline
YOLACT++(2020)s\cite{bolya2019yolact++} &
  \begin{tabular}[c]{@{}l@{}}MS COCO 2017\\ PASCAL VOC 2012\end{tabular} &
  33.5(AP)@34.1fps &
  \begin{tabular}[c]{@{}l@{}}Add re-scoring branch;\\ Add DCN to speed up;\\ Try different anchor aspect ratio and scales\end{tabular} \\ \hline
SOLO (2019)\cite{wang2019solo} &
  MS COCO &
  \begin{tabular}[c]{@{}l@{}}37.1(AP)@10.4fps\\ 34.2(AP)@22.5fps (light-weight)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Propose instance category;\\ Only needs to perform two pixel-level \\ classification problem; \\ Global mask representation\end{tabular} \\ \hline
SOLOv2 (2020)\cite{wang2020solov2} &
  MS COCO &
  \begin{tabular}[c]{@{}l@{}}38.8(AP)@18fps\\ 37.1\%(AP)@31.3fps (light-weight)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Improve SOLO by mask learning and\\  \textit{matrix NMS}.\end{tabular} \\ \hline
TensorMask (2019)\cite{chen2019tensormask} &
  MS COCO &
  37.1\% (AP)@0.38s/image &
  \begin{tabular}[c]{@{}l@{}}Represent masks by multi-scale \\ structured high-dimensional(4D) tensors;\\ Scale-adaptive sizes are implemented\\  by Bipyramid structure.\end{tabular} \\ \hline
PolarMask (2020) \cite{xie2020polarmask}&
  MS COCO &
  32.1\% (AP)@12.3fps &
  \begin{tabular}[c]{@{}l@{}}Introduces contour representation\\  in the Polar coordinates;\\ The complexity is close to a \\ single-shot objector.\end{tabular} \\ \hline
BlendMask (2020)\cite{chen2020blendmask} &
  MS COCO &
  \begin{tabular}[c]{@{}l@{}}41.3\%(AP)@116ms/image\\ 34.5\%(AP)@39.7ms/image (real-time setting)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Combine benefits from both top-down \\ and bottom-up methods.\end{tabular} \\ \hline
CondInst (2020)\cite{tian2020conditional} &
  MS COCO &
  35.4\%(AP)@49ms/image &
  \begin{tabular}[c]{@{}l@{}}No need for RoI cropping and \\ feature alignment;\\ mask FCN network parameters are \\ dynamically-generated;\\ Mask prediction heads are compact.\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Differences between some state-of-the-art methods. The data of 'Performance' is provided by its corresponding papers. Since test it by different GPU conditions, the numbers are for reference only.}
\label{tab:Instance segementation}
\end{table*}
